Base Station Certificate and Multi-Factor Authentication for Cellular Radio Control Communication Security

Current cellular networking remains vulnerable to malicious fake base stations due to the lack of base station authentication mechanism or even a key to enable authentication. We design and build a base station certificate (certifying the base station's public key and location) and a multi-factor authentication (making use of the certificate and the information transmitted in the online radio control communications) to secure the authenticity and message integrity of the base station control communications. We advance beyond the state-of-the-art research by introducing greater authentication factors (and analyzing their individual security properties and benefits), and by using blockchain to deliver the base station digital certificate offline (enabling greater key length or security strength and computational or networking efficiency). We design the certificate construction, delivery, and the multi-factor authentication use on the user equipment. The user verification involves multiple factors verified through the ledger database, the location sensing (GPS in our implementation), and the cryptographic signature verification of the cellular control communication (SIB1 broadcasting). We analyze our scheme's security, performance, and the fit to the existing standardized networking protocols. Our work involves the implementation of building on X.509 certificate (adapted), smart contract-based blockchain, 5G-standardized RRC control communications, and software-defined radios. Our analyses show that our scheme effectively defends against more security threats and can enable stronger security, i.e., ECDSA with greater key lengths. Furthermore, our scheme enables computing and energy to be more than three times efficient than the previous research on the mobile user equipment.

==> Sections/Apndx_Our_Scheme.tex <==
\section{Multi-Factor Authentication Algorithm}
\label{apndx:algorithm}
\begin{algorithm}[t!]
\small
    \caption{Multi-factor authentication at user equipment using $ID,K,L,t$ \syc{lower priority}}
    \label{alg:algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Parameter}{Parameter}
    \Input{         $\mathcal{C}$.$ID_{i}$, $\mathcal{C}$.$K_i$, $\mathcal{C}$.$L_i$, \hfill \hfill \hfill /* \textit{Blockchain ledger} */ \\
                    \mbox{SIB1}, $ID_i$, $n$, $t$, $S_k$, \hfill \hfill \hfill /* \textit{Online communication} */ \\
                    $\bar{L}$, $\bar{t}$ \hfill \hfill \hfill /* \textit{User equipment sensing} */
                    }
    \Output{$A$ \hfill \hfill /* \textit{Authenticated? True (1), False (0)} */}
    \Parameter {$\tau_t$,$\tau_d$}
    $ A = 0$ \\
    \If{$\mathcal{C}.ID_i$ == $ID$} 
    {
       $K_i$, $L_i$ = get($ID$,$\mathcal{C}$.$K_i$, $\mathcal{C}$.$L_i$)  \\

       \If{distance($L_i$, $\bar{L}$) $\leq \tau_d$}
       {    
           % $\Delta t$ = $\bar{t} - t$ \\
       \If{($\bar{t} - t$)$ \leq \tau_t$}
            {   
                \If{$V_{K_i}$(\mbox{SIB1},$n$,$t$,$S_k$) == 1}
                {
                    \textnormal{\textbf{return}}  $ A = 1$ \hfill  \\
                }
            }
        }
    }

\end{algorithm}
\sou{Newly drafted}

The user equipment uses multiple factors ($ID, L, t, K$) from multiple sources (offline/online communication, local sensing) to yield multi-factor authentication. Algorithm~\ref{alg:algorithm} illustrates the multi-factor authentication including the sources of factors and the sequential verification. Upon successful sequential verification ensures the authenticity of the base station. 

In the offline, the blockchain ledger delivers the database, $\mathcal{C}$, containing the digital certificates of the legitimate base stations validated by the core network. Each digital certificate within $\mathcal{C}$ has base station ID, $ID$, base station public key, $K$, and the base station location, $L$. We use these three factors for authentication and we present the parameters as $\mathcal{C}.{ID}_i$, $\mathcal{C}.{K}_i$, $\mathcal{C}.{L}_i$ for any base station $i$. During online communication, i.e. SIB1 broadcast message transmission, the user equipment received SIB1, cell ID, $ID$, nonce, $n$, timestamp, $t$ and digital signature, $S_k$. During multi-factor authentication, the user equipment also senses its location, $\bar{L}$ and SIB1 reception timestamp, $\bar{t}$. The user equipment also selects two control threshold parameters $\tau_d$ and $\tau_t$ for $L$ verification and $t$ verification. All of these factors are being used in the sequential authentication verification of our scheme. The output of the sequential verification is represented by $A$ which is a boolean, where $A=0$ for not authenticated and $A=1$ is for authenticated.

At the beginning of the algorithm, the user equipment sets $A=0$, i.e. the base station is not authenticated. Then it proceeds for $ID$ verification by looking up the base station ID in the blockchain ledger, $\mathcal{C}$. If the user equipment finds a base station certificate using the cell ID ($ID$) received during the online communication then the $ID$ verification is successful and it proceeds to the $L$ verification. However, before $L$ verification, the user equipment gets the base station location, $L$, and public key, $K$ from the ledger for later verification. In $L$ verification, the user equipment measures the distance (e.g. euclidean distance) between $L$ and $\bar{L}$. If the distance is less than or equal to the threshold $\tau_d$ then the $L$ verification is successful and it proceeds to $t$ verification. In $t$ verification, the user equipment uses the timestamp, $t$, and its measured timestamp, $\bar{t}$. If $\bar{t}-t$ is less than or equal to $\tau_t$ then the $t$ verification is considered successful. Upon successful $t$ verification, the user equipment proceeds for SIB1 message verification by verifying the digital signature. In SIB1 verification, it uses $K$ received offline and $S_k$ received online. If the digital signature verification $V_{K_i}$(SIB1,$n$,$t$,$S_k$) results in $1$ then the SIB1 verification is successful. Upon successful SIB1 verification, the final algorithm output yields $A=1$, i.e. the base station is authenticated. If the verification fails at any step in the sequence then the authentication results in $A=0$, i.e. base station not authenticated.


==> Sections/Blockchain_OS.tex <==
\section{Blockchain in Our scheme}
\label{apndx:blockchain_os}
Because the service provider infrastructure (core network and base stations) are public entities and do not require anonymity or privacy and because the public keys can be public/known for the security of the public-key digital signature, we use a permissioned but public blockchain where the 
blockchain ledger gets written only by the core network while it can be read/stored/accessed by all the entities in the cellular networking. Therefore, our blockchain forgoes the heavily distributed consensus protocol, e.g., computation-heavy proof-of-work (PoW), to determine which data gets uploaded and by whom. (Technically, our blockchain implementation in Section~\ref{subsec:offline_results} uses PoW consensus but with a difficulty of 0, i.e., all hash function computation for mining is valid.) Also, in contrast to the cryptocurrency blockchain, we do not have the incentivization or competition issues because the service provider infrastructure and its beneficiaries/clients are all aligned in their incentives to provide connectivity and secure cellular connections against the rogue base stations. 

==> Sections/Discussion_and_Future_work.tex <==
\section{Discussions of Future Work}
\label{sec:discussion}
% \souc{brainstorming what others can be included here}
% \syc{All of these would point to Future Work, because limitations, extensions, applications to other scenarios imply future work. I changed the title to better reflect this. Also, I recommend changing the subsection title below to be more descriptive about the future work direction than just "Future Work"; I suggest "Securing other base station control communications."}

% \syc{I would also re-order the subsections based on the importance and strength of these directions.}

\noindent \textbf{Securing more radio control communications}
\syc{lower priority. But if in the appendix, summarize and include in the Conclusion} 
% \subsubsection{Securing more radio control communications}
In this work, we propose base station authentication using SIB1 message. There are other system information messages in cellular networking which carry important system parameters such as mobility information, public warning messages, cellular vehicular-to-everything networking, etc. The base station broadcasts these messages in clear text and without any integrity protection. The adversary can exploit these vulnerabilities to launch attacks. However, authenticating other SIB messages using the digital signature may cause scalability issues and pose challenge to design practical solution. We explore designing a scalable and pragmatic solution to protect other system information messages as a future work. %how the attacker can exploit vulnerabilities of other system information messages and how can we protect them %\syc{let's revise the following part of the sentence to ". " It's more appropriate for future work directions, as it is identifying what needs to be addressed as opposed to jumping ahead with our current solution plan.} more efficiently without using digital signatures. 

\noindent \textbf{Transition to Post-Quantum Cryptography}
%\subsubsection{Transition to Post-Quantum Cryptography}
The state-of-the-art and this research work adopt classical public key cryptography to thwart malicious or rouge base station attacks. According to Shor's algorithm~\cite{shor1994algorithms}, classical public key cryptography (based on integer factorization and discrete logarithmic problems) is vulnerable to quantum computers which motivates the transition of the scheme toward post-quantum cryptography (PQC). The National Institute of Standardization and Technology (NIST) has standardized three PQC digital signature ciphers namely, Dilithium, Falcon, and SPHINCS+. However, transitioning from classical to post-quantum cryptography poses challenges to integrate into existing radio control communication due to their larger key and digital signature size (e.g. signature length of SPHINCS+-256s is 29792 bytes with a public key of 128 bytes and Falcon-512 has 666 bytes of signature length with 897 bytes of public key). The byte size limitation of the SIB1 message restricts the seamless incorporation of PQC digital signature algorithms into our scheme. For instance, the Falcon-512 algorithm with a signature length of 666 bytes, exceeds the capacity of the SIB1 message. Consequently, increasing the packet size of SIB1 is a prerequisite to include PQC in base station authentication. In that case, our scheme is more friendly for PQC algorithms integration because we distribute the public key offline using blockchain and therefore the SIB1 packet size needs to extend only to fit the digital signature.

\noindent \textbf{Adopt our scheme in Standardization and in Practice}
%\subsubsection{Adopt our scheme in Standardization and in Practice}
We build our scheme on top the standard 3GPP 5G NR protocol and it is also backward compatible with LTE because broadcasting RRC messages are identical in both 5G-NR and LTE. We only add four additional data fields in the SIB1 message on top of the standardized packet to authenticate the base station in the radio control communication while respecting the RRC layer protocol standards. In the RRC procedure, the base station needs to generate a digital signature before broadcasting the SIB1 message and the UE needs to verify the SIB1 message using the base station certificate before passing the containing information to the upper layer for further processing. For our offline phase adoption, we propose the Authentication Server Function (AUSF) of the core network take part in writing certificates in the blockchain. Access and Mobility Function (AMF) can act as an intermediary node between the base station and the AUSF during certificate signing.

% \subsubsection{Roaming scenario}
% Our design scheme can be adapted to the roaming scenario by adding certificates of the visited network into the blockchain. When the user wants to access cellular services outside of its subscribed network (home network) coverage using another network (visited network) then the user needs to download the blockchain ledger of that visited network. In this case, the problem is that the user does not have the anchoring public key of the visited network (as installed subscribed network public key in USIM card). We can solve this problem by adding the visited network certificates containing the public keys signed by the home network into the blockchain. Hence, to handle the roaming scenario, the core of the home network signs certificates of the visited network (public key of the core of the visited network) and distributes that with the base station certificates. When the user wants to use the visited network it first gets the public key of the visited network from its existing blockchain and then downloads the blockchain of the visited network to authenticate visited network base stations.

\noindent \textbf{Mobility of User and Base Station}
%\subsubsection{Mobility of User and Base Station}
In this research, we limit our scope where the user can be mobile and base stations are stationary as compared to flying/drone base stations which are mobile. The location information in the base station certificates are static GPS location of the stationary base station. Further exploration is required to incorporate location information of flying base stations into our scheme in the future. 


% \syc{Add discussions about Post-Quantum Transition. For example, how would applying our scheme using the post-quantum digital signature ciphers look like? What would be the challenges? The selected PQC ciphers are: Dilithium, Falcon, and SPHINCS+. Simeon and Manohar know about these.}

% \syc{Add discussions about Transition to Standardization and Practice.}

==> Sections/Hardware.tex <==
\section{Hardware Specification}
\label{apndx:hardware}
\begin{table}[]
\caption{Hardware specifications for the devices used.} %Device specifications of our experimental setup}
\centering
\tiny
%\renewcommand{\arraystretch}{1.4}
\label{device_specs}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllll}
\hline
Simulating       & Processor (brand, model \& clock speed)          & Memory\\ \hline
Core Network & Ryzen Threadripper 3960x @ 4.5 GHz   & 64 GB  \\ \hline
Base Station & AMD Ryzen 7 5700U @ 4.3 GHz & 16 GB \\\hline
User Equipment         & Intel 12th N95 @ 3.4 GHz        & 8 GB  \\\hline
3rd Party Node   & Intel Core i7-10750H @ 2.6 GHz       & 16 GB \\ \hline
\end{tabular}
}
\vspace{-5px}
\end{table}



For the frontend radio communications between the UE and the base station, we use two USRP B210 software-defined radio (SDR) hardware and the two nodes are $d$ distance apart. For the backend processor for processing the digital communications, the hardware and processor specifications of the machines that we use for the simulated nodes are in Table~\ref{device_specs}. The highest-rated processor/CPU (AMD Ryzen Threadripper 3960x) is used to simulate the core network and the second highest-rated processor (AMD Ryzen 7 5700U) simulates the base station. The UE hardware (Intel 12th Gen N95 mini PC) is also comparable to that of the 5G smartphone computing capabilities. 

==> Sections/Improvements.tex <==
\section{\sou{Scope for Improvements}}
\sou{
This section is just for tracking the improvements that we discussed. \\
Reviews of IEEE CNS submission: \\
Strengths: \\
1. Base station authentication is an important factor for defeating rogue base stations. \\
2. The implementation efforts try to almost resemble a realworld scenario. \\
3. The proposed solution is technically sound. \\
\\
Scope of Improvement:\\
1. Stronger motivation for using blockchain based key distribution over PKI\\
2. Strong and clear threat model\\
3. Include security analysis and discussion\\
4. Paper re-organization/writing for more clarity and readability\\
\\
Our course of action: \\
1. Introduce base station certificate which contains ID, BS public key, and location information. - Done for online part (updated: 06 Oct-2023) \\
2. Threat model will be revised such that each certificate field will address one of the threats. (public key $\rightarrow$ authentication and integrity and location information $\rightarrow$ replay/location spoofing attack protection). \\
3. Implement fake base station attacks.- Yet to figure out how hackRF can be used with srsRAN (updated 06 Oct -2023)\\
4. Include a contrast between our scheme and 5G-AKA. Why we need our scheme? Does 5G-AKA has any mechanism that can do the same task as our scheme does?
 \\
5. A new section/subsection regarding blockchain application in 5G/Mobile devices to address one of the feedback of CNS review (usage of blockchain is not practical)
}





\begin{tabular}{|c|c|c|c|||c|c|}
\hline
\textbf{Threat type} & \textbf{Vulnerability} & \textbf{Threat vectors} & \textbf{Threat impact} & \textbf{STA Research defense} & \textbf{Our scheme defense} \\ \hline
\multirow{3}{*}{New Base Station Threat} & Unprotected control comm. messages & Transmit fabricated base station ID and RRC message & Authentication failure and connect to the attacker &  Base station authentication\tnote{$\circ$}  &  Base station authentication\tnote{$\circ$} (\S\ref{sec:our_scheme}) \\ \cline{2-6} 
 & & Distribute fabricated public key & Authentication failure and connect to the attacker & Public key distribution along with the message\tnote{$\circ$} & Blockchain based certificate distribution\tnote{$\circ$} (\S\ref{subsec:our_scheme_blockchain})\\ \hline
\multirow{4}{*}{Base Station Spoofing} & Unprotected system information messages & Transmit fabricated base station ID~\cite{rupprecht2018security} & Force the UE to connect with the fake base station & Base station authentication\tnote{$\circ$} & Base station authentication\tnote{$\circ$} (\S\ref{sec:our_scheme})  \\ \cline{2-6} 
 & Unprotected system information messages & Handover exploitation~\cite{bitsikas2022you} & Denial of service, UE battery drain, cell outage &  Base station authentication\tnote{$\triangle$} & Base station authentication\tnote{$\triangle$} (\S\ref{sec:our_scheme}) \\ \cline{2-6} 
 & Unprotected system information messages & Dispatch false public warning/alert messages~\cite{bitsikas2021don} & Authentication failure and false alarms (such as emergency alarms) & Base station authentication\tnote{$\triangle$} & Base station authentication\tnote{$\triangle$} (\S\ref{sec:our_scheme}) \\ \cline{2-6} 
  & Unprotected system information messages & Bidding down attack~\cite{2023karakoc} & Downgrade service from 5G to 4G to 3G to 2G & Base station authentication\tnote{$\triangle$} & Base station authentication\tnote{$\triangle$} (\S\ref{sec:our_scheme}) \\ \cline{2-6} 
 & Packets without time and location information \souc{?} & Wormhole attack~\cite{hu2006wormhole} & Bypass the cryptographic authentication & $X$ & Location-based authentication$^\circ$ (\S\ref{sec:online_bs}) \\ \hline
% \multirow{2}{*}{Control Communication Injection} & Unencrypted/Unprotected control messages & Man-in-the-Middle attack~\cite{shaik2019new} & UE capability identification, Traffic monitoring &  Base station authentication & Base station authentication (\S\ref{sec:our_scheme}) \\ \cline{2-5} 
%  & Unencrypted/Unprotected control messages & Protocol bidding down ~\cite{shaik2019new} & Downgrade service to 2G/3G/4G, device power drain, &  Base station authentication & Base station authentication (\S\ref{sec:our_scheme}) \\ \hline
\end{tabular}

\begin{tablenotes}
        \item [$\circ$] Complete defense 
        \item [$\triangle$] Partial defense 
        \item [$X$] No defense
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
\label{tab:threat_analysis}
\end{table*}

==> Sections/Old_Tex_Files/03252024__Introduction.tex <==
\section{Introduction}
%\sou{Distribution will be replaced by Delivery throughout}
% \souc{Wording issues: \syc{As a secondary factor, i.e., tie-breaker, try Google search for seeing which word is more popular} \\
% 1. Mobile user/user? \syc{User equipment? We would start more broadly than just 4G/5G so it may be good to imply 4G/5G from the start} \\
% 2. Fake base station or malicious or rouge base station? 
% 3. Replay/Relay attack or only relay or only replay?
% 4. Location spoofing or wormhole? \\
% 5. Certificate construction or generation?}
% \souc{First Round}\\
% \souc{How cellular networking is important}\\
\sou{The novelty of our research: \\
1. Base Station certificate construction with ID, Public key, and location information that prevents malicious base station threats (section 4: Threat analysis) \\
2. Offline delivery of BS certificates using blockchain. Why? Because (a) offline enables usage of greater cryptographic key length i.e. higher security while the online certificate delivery is limited due to byte length constraint (b) Takes three times less signature verification which consumes three times less energy than online delivery \\
The multi-pronged authentication is the outcome of our research novelty. Hence, we validate our research novelty with multi-pronged authentication.}

Mobile and wireless users use cellular networking, e.g., 4G and 5G, for connectivity and Internet access. Cellular networking has exceeded Wi-Fi in accessing the Internet and web since November 2016. %\syc{Please update the following sentence with more recent:} \souc{updated as of October}
As of \sour{february 2024}, the cellular traffic is \sour{1.58} times greater in use/traffic worldwide and up to 6 times greater in the developing regions~\cite{mbdtus}. %, the reliance on cellular networking even increases up to 5 times~\cite{mbdtus}.  
%this is become 3-5 times greater for countries in developing regions, e.g., Somalia, Eritrea, Niger, Nigeria, Afghanistan, etc. \syc{Arijet: Please fill them in, provide the sources, and cite them for these blanks.}\as{addressed} \syc{Arijet: Please find this number for developing regions. I expect the number to be very high (almost no WiFi but complete reliance on cell) in some regions.} \as{addressed}. % \as{Worldwide (Mobile:57.18\% and Desktop:40.8\%) - 1.41 times, Africa (Mobile:72.05\% and Desktop:26.8\%) - 2.68 times, Somalia (Mobile:75.04\% and Desktop:23.58\%) -3.18 times, Eritrea (Mobile:77.03\% and Desktop:22.09\%) - 3.48 times, Niger (Mobile:83.33\% and Desktop:16.41\%) - 5.07 times, Afghanistan (Mobile:76.04\% and Desktop:23.32\%)- 3.26 times, Nigeria (Mobile:80.82\% and Desktop:18.5\%) - 4.36 times}  
To access the remote servers, the mobile users rely on the cellular base station which is the first hop in the communication path and acts as a bridge gateway between the wireless link (from/to the mobile user) and the wired connections (from/to the cloud server via routers and switches). 

%\souc{Malicious base station attack and reason} \\
The malicious or rogue base station has been a well-known security issue in the wireless security community. The malicious base station threats include breaching the user privacy against its location and credentials, redirection of the networking (e.g., fake destination and web server), protocol downgrading and manipulation (e.g., de-registration and authentication-and-key-agreement or AKA bypass), %DoS, downgrading (AKA bypass and de-registration)
dispatching false alert messages, %~\cite{bitsikas2022you,lee2019your}} \syc{Do not add citations here; we intentionally refer to the section to avoid this} 
and complete control of the availability and wireless link for DoS, among others. %(Section~\ref{subsec:related_malicious_bs}). 
The malicious base station threat research works are discussed in greater details in Section~\ref{sec:related_work}. 
%
The vulnerability stems from the lack of key establishment and authentication of the base stations\footnote{The 3GPP 5G provider infrastructure does support keys and authentication but the subject entities are at the backend beyond the base station, i.e., 5G authentication and key agreement (AKA) with the core network and 5G authentication and key management for applications (AKMA) with the destination application servers. %\syc{Please confirm this for 5G AKMA} \souc{5G-AKA is the primary authentication protocol for mutual authenticaiton between UE and the network. The 5G-AKMA is a frame work that utilizes the 5G-AKA to establish keys between UE and the application server (which is defintely after establishing 5G-AKA). Hence in this case 5G-AKA is appropriate.} \syc{Thanks. I reflected that.}
For example, 5G AKA
establishes the public key for the backend core network, e.g., via hardcoding on the sim card, and there is security set up between the core network and the user equipment~\cite{3gppsap}. However, the intermediary base station does not have a key of its own to build autonomous security control.}, which prevents a mobile user from distinguishing between authorized vs. rogue/malicious base station. 
% %While the backend \emph{core network} (multiple hops away from the mobile user) provides the security control and secure communications based on cryptography with the mobile user, the base station acts as a security-oblivious bridge gateway, e.g., does not block or control the communications for security. The users also remain vulnerable to connect with a malicious or rogue base station because they cannot distinguish between legitimate vs. non-authorized base station. % with malicious intent including mobile-user privacy breach
% %\syc{3GPP is undergoing to introduce public keys for base stations. Let's mention that.} 
% % 3GPP is currently undergoing the process to introduce public keys for base stations; however, the process is at an early stage in establishing the requirements of such keys~\cite{3gppfbs}%\syc{Cite the 3GPP lit. here}
% % The current 5G networking therefore has no defense against malicious base station, for example, there are software-defined radio (SDR) tutorials to set up rogue and malicious base stations against 5G phones~\cite{sdrhacking1}. %\syc{Arijet: help cite those sources}\as{addressed}
%
% %(In contrast, in 5G, the backend core network establishes public key and uses it to secure the connection security. The base station is security-oblivious and only serves as a bridge gateway between wireless and wired communications without any autonomous security control or establishing its own key.) % is set up between the user and the backend core network after the base station's operation for serving as the bridge gateway between wireless and wired communications without security.)
% %(The security is set up between the user and the backend core network after the base station's operation for serving as the bridge gateway between wireless and wired communications without security.)
% \souc{It seems we directly jumped into the public key cryptography. Should we say something why symmetric cryptography is not useful here? May be in 1 or 2 lines?} \syc{It may be distracting. It is known that symmetric keys are often the result of public-key crypto, e.g., Diffie-Hellman Key Exchange. Is there a reason that you want to include symmetric cryptography here?} \\
% %\syc{Need to revise/write the rest of the Intro from here:}
% %\souc{Base Station authentication and public key} \\
% Authenticating a base station requires a key (providing an advantage for the legitimate authorized parties over the unauthorized parties) and the cryptographic schemes building on the key secrecy (the cipher and the cryptographic protection are broken if the unauthorized attacker knows the key). While the mutual authentication between the user and core network % both the user authenticating the core network and the core network authenticating the user 
% use such keyed cryptographic scheme, \sou{the user does not authenticate the base station in the current mobile cellular networking (5G and the previous generations)}. In fact, the current 5G networking implementation and practice does not utilize the base station's public key at all, although 
There have been recent proposals in research~\cite{singla2021look,hussain2019insecure} and standardization/development~\cite{3gppfbs} to introduce and use the base station's public key. 
In 3GPP standardization, such proposals are at the early stages of establishing the requirements for the base station keys~\cite{3gppfbs}. 
The lack of key disables the authentication and the integrity protection of the control communication exchanged between the user equipment and base station; such control communication resolves the medium access control (MAC) and radio resource control (RRC) to set up the wireless channel before involving the backend core network. 

To secure the base station authenticity and its communication integrity, we design and build our scheme spanning across the processes of the certificate construction, the certificate/key delivery, and the key application for digital signature. 
For certificate construction, we design and build the base station certificate building on the X.509 certificate, which generally binds the public key and its subject ID to certify the subject's public key. However, we newly add the geographical location information of the stationary terrestrial base station and bind both the base station ID and its location to the public key so that the user equipment can cross-check with its own location to verify the location authenticity. %against \syc{change the term if using different one:} remote replay threat. % which enables security against \syc{After the threat section drafting and establishing the terms, add the threats which gets defended by the location inclusion on the certificate}. 
For certificate/key delivery, we use permissioned blockchain so that only the core network can write on the blockchain and distribute the base station's public keys. 
The base station's public key is then used for digital signature for message authenticity of the control communications between the user equipment and base station. 
The base station certificate generation (key establishment) and its blockchain-based delivery (key delivery) occur \emph{offline} before the user equipment encounters the base station. 
The base station's digitally signing the radio control communications and the user equipment using the public key to verify (digital signature and verification) occur \emph{online} when the user encounters the base station and communicates with it for the connectivity service. During online, the message authenticity protection for the control communications are critical as the \emph{control communications} are the communication exchanges to set up the communication channels for the following data communications or connectivity service, e.g., radio channel frequency and medium access control with the base station and the user-equipment authentication and security mode with the core network. 

%\sou{The upper one describes the overview of our scheme while the latter one describes how our scheme advances recent research. However, there is a gap between these two paragraphs. we need to give a rationale for choosing each component of our scheme that addresses the challenges of recent research. Firstly, Why do we include ID, location, and public key in the digital certificate? Secondly, what is the motivation for using blockchain here? The answer is, online transmission of base station certificates is prohibited by the byte size limitation (372 bytes) of recent research works. Hence, we need blockchain as an alternative solution to address this problem. We replace PKI for delivery of certificates we use blockchain. Thirdly, although it should come first, what is our reason for using base station public key instead of a symmetric key? The reason is the inherent deficiencies of symmetric key cryptography: non-repudiation, non public verifiability of keys, and most of all delivery of symmetric key because in current practice the user equipment has no information of the base station at all before it receives the first RRC message.}

\syc{misplaced}
\sour{Our rationale for using blockchain in offline communication for base station certificate delivery comes from the inherent byte size constraint of 5G radio control communication imposed by the physical layer. The base station can adopt Public Key Infrastructure (PKI) and send digital certificates to the user equipment in the first radio control broadcast message but according to the 3GPP standard, the physical layer limits message size up to 372 bytes~\cite{3gppphy} making it difficult to fit the base station certificates within the first radio control message. Moreover, in the PKI-based certificate delivery, the user equipment needs to verify the multiple certificates using the network public key installed within before authenticating the base station. The offline blockchain-based certificate delivery addresses both of the pitfalls with no byte length limitations while the secure delivery of base station certificates with its inherent property and the user equipment can authenticate the base station with lower computational time and with lower energy consumption.}

\syc{trying to do too much}
We advance beyond %both the state-of-the-art practice (no authenticity and integrity protection) and 
the state-of-the-art to enable greater security and for efficiency. The state-of-the-art, the most prominent and related to our work~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}, do not make use of the base station's location and \sour{adopt PKI to} append the public key within the base station's control communication, e.g., when delivering the \sour{first broadcast} message in 5G RRC. %, and use that to authenticate the base station and its following control communications
%~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}. %The related research works are generally covered in Section~\ref{rw}, but the most prominent and related works  
Our novel location information addition on the base station certificate enables the defense against wormhole attacks %\syc{wormhole?} 
that can launch fabricated radio control message broadcasting, handover exploitation, dispatching false alert messages, and bidding down attacks. %\syc{Fill these in. After the threat section drafting and establishing the terms, add the threats which gets defended by the location inclusion on the certificate}. 
Our blockchain application provides a secure record/database of the registered base stations and their public keys/certificates and delivers them offline, which makes the online control communications shorter and enables the use of the cryptographic cipher with greater security/key length. Offline Base station certificate dissemination through blockchain also enables three times less energy consumption at the user equipment for signature verification than state-of-the-art.
%\syc{Newly added:}
Such base station certificate construction and delivery enables a multi-pronged approach for authenticating the base station and its radio-control communication message; the ID is used to check if the base station is registered and stored in the blockchain database; the location verifies the base station's location integrity; and the digital signature defends against malicious injections. 

%\syc{Anything else we do better than the state-of-the-art research?}\souc{Another benefit is 3 times less power consumption due to offline base station certificate delivery}
%\sou{We used SIB1, wormhole attack throughout without explaining what this is.}
%\syc{TO MYSELF: 11152023: It may be better to try to incorporate the followings in the earlier paragraphs: offline vs. online, systems approach, comprehensive threat analyses. I'll work on this.}
We take a systems approach for our research to highlight our contributions across multiple process steps for authenticating the base station's ID and control communication. %, which involve both the offline and online processes. 
We conduct a comprehensive analyses of the vulnerability and the threat to better identify how our scheme defends against the threats based on malicious or rogue base station. 
%
Our research also involves prototype implementation for validation and experimentation and builds on the existing standardized technologies. 
For the offline processes, %For the \emph{offline} process (occurring before the user equipment encounters the base station), 
we build on the X.509 certificate and use the blockchain to deliver the base station's public key and location. Blockchain automatically delivers and synchronize the latest the public key information when the core network introduces/adds the subject base station to the connectivity-provision infrastructure, and we use Ethereum smart contract in our implementation. 
For the online processes, %For the \emph{online} process (when the user equipment is in communications with the base station to access the connectivity provided), 
we build on the 3GPP 5G NR protocol and more precisely the SIB1 message broadcasting transmissions in the 5G radio resource control (RRC). In our scheme, the base station digitally signs the SIB1 message in the 5G radio resource control. In turn, the user equipment, having received the base station's certificate and public key previously in offline, verifies the digitally signed SIB1 message. We implement, validate, and test our scheme using software-defined radios (SDR) and the open-source 4G/5G srsRAN software. 

Our research contributions include: 
\begin{itemize}[noitemsep,topsep=0pt]
\item The comprehensive vulnerability and threat analyses to identify those against which our scheme is effective %(covering the threats which get defended by our scheme), 
\item The new base station certificate construction including the terrestrial base station's location to defend against wormhole attacks
\item The blockchain-based delivery of the base station certificate to provide a secure record of registered base stations and to enable the offline delivery of the base station's certificate (ID, location, and certificate)
\item The multi-pronged use of the base station certificate (including the ID, location, and public key for digital signature) to secure the message authentication of the base station's RRC control communication message 
%\item The use of the public key for digital signature to secure the message authentication of the base station's RRC control communication message 
\item The concrete implementation of our schemes, enabling validation and experimentation
\item The comparative vulnerabilities/threats, security, and performance analyses of our scheme against the state-of-the-art to demonstrate the strengths of our scheme 
\end{itemize} 

% The rest of the paper is organized as follows. We state the threat model that motivates our research and describe our contribution in section~\ref{sec:motivation}. We provide relevant background in section~\ref{sec:background} to support the comprehensive threat and defense analyses in section~\ref{sec:threat_analyses}. We describe our scheme in section~\ref{sec:our_scheme}, experimental setup in section~\ref{sec:experimental_setup} and experimental analyses in section~\ref{sec:experimental_analyses}. Section~\ref{sec:related_work} describes related work, and section~\ref{sec:conclusion} concludes the paper. 

%\syc{Draft the rest of the paper-organization paragraph}
%\syc{Explicitly state why the Motivations section and the Comprehensive Analyses section are separate. The Analyses section require the Background, while the earlier Motivations section does not.} 




% \syc{LET'S MOVE OR OMIT THE REST OF THE INTRODUCTION SECTION, i.e., the following paragraphs in this section. For example, the fact that blockchain carries public information and the base stations information are public should get included in the future section; this has been omitted in the new Intro before this comment. If any questinos, let's discuss.}

% %\souc{introduce the reason or challenges for public key: Want to introduce the base station certificate later paragraph: construction, distribution and usage} \\
% \sou{
% The main purpose of introducing base station authentication is to prevent users from getting connected to malicious base stations. The base stations are distributed %\souc{distributed network?} \syc{Looks fine, e.g., "the soldiers are distributed across the various strategic points."} 
% across a large geographical area and connected to the core network. The user has only the security parameters (key, security scheme, etc.) of the core network installed in the integrated card. It is a challenge to distribute the base station public key to the users because of the distribution channel to use and the trust management of the public key. The trust management problem can be solved by utilizing the pre-shared cryptographic keys between the user and the core network. For the public key distribution, the current research works choose to send the public key and the digital signature along with the message. It has two consequences: the user needs to wait until it receives the message to get all the parameters, then verify the parameters before authenticating the base station and the message size which limits the number of bytes that can fit into the message. Furthermore, the authentication alone cannot prevent attacks such as relay/replay, and location spoofing which requires additional parameters (timestamp, location information). In such cases, additional verification of these parameters and the message size limitation make the distribution problem more challenging. Hence, to authenticate the base station we need to construct a certificate to contain the security parameters, distribute the certificate, and make use of the certificate to authenticate the base station.}

% \souc{Public key distribution. Not sure how to modify the paragraph. Maybe some part of it goes in preceding paragraph: Work on this later } \\
% We securely distribute the base station's public key (to enable the security functionalities and implementations on the base station) %(which is not used in the current 5G networking and enables the security control functionalities on the base station) 
% and use the key to authenticate the base station and secure the RRC bootstrapping (when a mobile user gets turned on for use and encounters a base station). 
% While previous research exchanged the base station's public key as a part of the radio resource control (RRC) communications (appending the public key and the certificate along with the very first broadcast message for bootstrapping the radio channel control)~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}, % \syc{Arijet: Help cite. The more the better.}\as{addressed} \syc{Is "3gppfbs" standardization suggestion, as opposed to research paper?}, ~\cite{3gppfbs} is a standardization proposal but not finalized at this time. % The 1990's papers do not specify SIB1 but states "bootstrapping" message, while the more recent papers do specify SIB1
% such approach adds prohibitive overheads on the RRC communications, which is broadcasting communications designed for short control messages and limited in bandwidth. %\syc{This needs to be supported later with the physical-layer descriptions of the RRC communication and how that makes it broadcasting friendly with low bandwidth performance.} %RRC communications dedicated for setting up the wireless channels (physical layer and medium access control) is broadcasting based (a base station broadcasts the initial SIB1 to many mobile users), designed for short RRC-control messages, and limited in bandwidth (its reliable transmission rate is significantly lower than the data channel established after RRC control). %such approach has seconds of transmission overheads for the wireless communication link (not the entire path from the core network to the user). 
% %This approach also requires the public key and the certificate along with SIB1 in the RRC communications 
% The state-of-the-art research appending the base station's public key in the RRC broadcast message also limits the cryptographic cipher choice because of the size limit of such broadcasting message. 

% %\souc{Our designed scheme in high level: Revamped to accommodate the changes} \\
% We design and build a scheme to construct the base station certificate generated by the base station containing the relevant information fields, distribute the certificate among the users through blockchain after signing by the core network, and use the certificate by the user during base station authentication. The certificate construction and distribution take place offline (before the initial RRC connection \souc{or during a base station setup}) and the certificate usage takes place online during the RRC connection setup by the user. Blockchain is appropriate because the base stations' deployment and identities are publicly known and accessible as telecommunications service provider entities, e.g., a public website identifying the currently active base stations~\cite{cellmapp}, unlike mobile users requiring privacy. In our scheme, the blockchain containing the certificate of the deployed base stations is publicly accessible (i.e., can be read and stored by all relevant nodes) but permissioned (i.e., only the core network writes its blocks and records). We use blockchain because of its properties of distributed storage, automatic synchronization/broadcasting, and high integrity. After the offline key distribution, the legitimate base station digitally signs the SIB1 message, and a mobile user checks the replay/relay, location spoofing attack before verifying the signature using the base station certificates distributed via blockchain. We implement, validate, and test our scheme using software-defined radios (SDR) and the popular open-source 4G/5G software in srsRAN for the online 5G RRC communications and using Ethereum for the offline blockchain-based public key distribution.
% % We design and build a scheme that distributes the base station's public key using blockchain offline (i.e., before the initial RRC handshake). Blockchain is appropriate because the base stations' deployment and identities are publicly known and accessible as telecommunications service provider entities, e.g.,~\cite{cellmapp}, unlike mobile users requiring privacy. 
% % In our scheme, the blockchain containing the public keys of the deployed base stations is publicly accessible (i.e., can be read and stored by all relevant nodes) but permissioned (i.e., only the core network writes its blocks and records). We use blockchain because of its properties of distributed storage, automatic synchronization/broadcasting, and high integrity. After the offline key distribution, the legitimate base station digitally signs the SIB1 message, and a mobile user verifies the signature using the public key distributed via blockchain. We implement, validate, and test our scheme using software-defined radios (SDR) and the popular open-source 4G/5G software in srsRAN for the online 5G RRC communications and using Ethereum for the offline blockchain-based public key distribution.

% %\souc{Added our contributions here. Should we include why we use blockchain for distribution (motivation)? Include a high level overview which will be connected with later section\\}

% \noindent In summary, our contributions to this research work are: 
% \begin{itemize}
%     \item providing concrete attack scenarios of a fake base station that exploits the legitimate base station's system information messages
%     \item introducing security parameters including base station public key, location information, timestamp, and distance to thwart fake base station attacks
%     \item solving distribution of security parameters through base station certificates using blockchain
%     \item providing a comparative security and performance analysis of our scheme against state-of-the-art research
% \end{itemize}


% \souc{I want to include answers to the following questions:\\
% 1. How a fake base station can exploit system information messages to launch attacks? This will give us why SIB1 is perfect for authentication except it is the first message. Ans: Add a subsection in related work threats in RRC communication: include C pooper's work. \\
% 2. Why blockchain for distribution other than sharing security parameters along with SIB1? The fields/information elements in SIB1 are much more in 5G-NR than in 4G. On the other hand, the maximum allowable size for SIB1 is 372 bytes. Hence it is inconvenient to include all security parameters inside SIB1.answer: we need to establish public keys of base stations beforehand for authenticity. A user can identify the authorized BS against unauthorized by the blockchain database containing the base station certificates}
% % The rest of the paper is organized as follows. Section~\ref{rw} discusses related research. Section~\ref{sec:background} provides a brief background in 5G mobile networking which is needed to understand our research. 
% % %Section~\ref{subsec:RRC_anlaysis} motivates our work with preliminary analyses using 5G implementations. \syc{Need another section motivating the RRC overhead} 
% % Section~\ref{sec:threat_model} describes our threat model to clarify our contributions. 
% % \syc{To self: Need to include the rest of the sections: our scheme, implementation, experiment, discussion, and conclusion}

==> Sections/Old_Tex_Files/03252024_our_scheme_new.tex <==
% \begin{figure}[t!]
%     \centering
% \includegraphics[width=0.9\columnwidth]{Images/High_Level_Arrow_Diagram.pdf}
%     \caption{Overview of our scheme. %\sou{Simeon please change "distribution" with "delivery"}
%     }
%     \label{fig:arrow_diagram}
% \end{figure}

\begin{figure}[t!]
    \centering
\includegraphics[width=0.75\columnwidth]{Images/Diagram_Key_Components_Sim.pdf}
    \caption{\syc{discuss} Information delivered during offline (dashed-dotted) vs. online (solid) for our scheme. The base station certificate contains the identifier ($ID$), public key ($K$), and location information ($L$).%\sw{Dotted-dashed line, no color}\sou{Simeon please change "distribution" with "delivery" and "Usage" with "Multi-Pronged Authentication"}
}
    \label{fig:key_components}
\end{figure}

%\vspace{-2px}
\section{Our scheme}
\label{sec:our_scheme}
%\souc{key components of base station certificate: construction, distribution, usage and two phases: offline and online}
We design a base station authentication scheme that consists of two phases: offline base station certificate construction and delivery, and online multi-pronged base station authentication by using the delivered certificate. In the offline certificate construction and delivery phase, the core network validates and signs the public key of base stations and publishes the digital base station certificate via the blockchain ledger. The core network binds both of the base station's cell ID ($ID$) and the geographical location ($L$) with the key ($K$) when digitally signing for the base station certificate. A UE that wants to connect to the network receives the base station certificates on the blockchain offline before initiating a radio connection with the base station. The offline blockchain communication includes the base station's certificate (including information fields listed in Fig. ~\ref{fig:cert_contents}) and can get delivered any time before the radio connection with that base station, e.g., in any of the previous communications by the mobile user. %This phase is offline because base station's public key can be make available to the mobile user's local storage in beforehand of radio connection initiation to the network (similar to USIM installation in mobile device). 
%\syc{Revise and reflec the multi-pronged approach} 
During the online multi-pronged authentication phase, the base station digitally signs the SIB1 message, and the UE receives and verifies the SIB1 message using the ID, public key, and location information of the base station that it gets from the offline blockchain. %Blockchain based PKI plays an important role in our scheme for secure and reliable delivery of base stations public keys to the mobile users.
The security of our scheme relies on the security of the cryptographic primitives.

%\syc{Recap offline vs. online information delivery. List them here, and state that the rest of the section describes and explains them in greater details.} 
In offline, we deliver the digital certificate database of the base stations $\mathcal{C} = \{C_i\}_i$, where $\{C_i\} = \{ID_i, K_i, L_i \}$ is the individual record and $i$ is the registered base station index. 
In online, we deliver cell ID ($ID_i$), nonce ($n$), and SIB1 generation timestamp ($t$) appended into the SIB1 message of the base station $i$. Fig.~\ref{fig:key_components} illustrates these key parameters and their delivery method from the base station to the UE. This information gets used for authenticating the base station $i$, which yields the Boolean $\mathcal{A}$, where $\mathcal{A}=1$ means that the base station $i$ has been authenticated (true) vs. $\mathcal{A}=0$ not authenticated (false). 
We describe and explain these information deliveries in greater detail in the rest of the sections. 


% \begin{table}[t]
% %\small
% \tiny
% \centering
% \vspace{10 px}
% \caption{\souc{Newly added: Need simeon's help to get size}A Base Station certificate with total size 138 bytes\sw{Consider displaying similarly to Fig. 3 but for x.509} \syc{Let's just use Fig. 3 if this is only adding the B information}}
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular} { |c| c | c |}
% \hline 
% \textbf{Field Name}  & \textbf{Description} & \textbf{Size (B)} \\
% \hline
% version & Version of the certificate & 1 \\
% \hline
% serialNumber & Serial number of the certificate & 1\\
% \hline
% issuerName & Operator name & 2\\
% \hline
% \textbf{subjectUniqueID} & \textbf{Cell ID of the Base Station ($ID$)} & 4\\
% \hline
% \textbf{subjectPublicKey} & \textbf{Base Station public key ($K$)} & 56\\
% \hline
% validityPeriod & Default value (1 year) & 1\\
% \hline
% \textbf{Location} & \textbf{Location info. of the Base Station ($L$)} & 8\\
% \hline
% %\textbf{Longitude} & \textbf{Longitude of the Base Station} & 4\\
% %\hline
% digitalSignature & Signature of the issuer & 64\\
% \hline
% algorithm & Algorithm used to sign the certificate & 1\\
% \hline 
% \end{tabular}
% \label{tab:x_509 fields}
% %\vspace{-10mm}
% \end{table} 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Images/Offline_Sim.pdf}
    \caption{Offline certificate construction and delivery using blockchain (right).\vspace{-10px}}
    \label{fig:offline}
\end{figure}


\begin{figure}[t!]
    \centering
\includegraphics[width=1\columnwidth]{Images/Diagram_for_Online_V2_Sim.pdf}
    \caption{Online multi-pronged base station authentication by user equipment (UE). The blue color indicates our addition in 5G RRC, and the blockchain (left) is locally stored at UE.\vspace{-10px}} %\syc{Fig moved because the Existing 5G subsection makes use of the figure}}
    \label{fig:online}
\end{figure}


\subsection{Offline Base Station Certificate Construction}
\label{subsec:our_scheme_cert_construct}

Our base station certificate construction builds on the X.509 standardized certificate, which is popularly used for securing the Internet and web, e.g., transport layer security (TLS) and hypertext transfer protocol secure (HTTPS). However, we adapt its construction specifically for base station and to enable greater security objectives. 
Figure~\ref{fig:cert_contents} illustrates the data fields within our base station certificate where our additions beyond X.509 are highlighted in blue. One change we make is the change of formats in the ID from the IP address for Internet/web security to the base station's cell ID ($ID$). 

We add the geographical location of the stationary terrestrial base station in the base station certificate, and the core network uses both the cell ID and the location information to digitally sign and generate the certificate. %which acts as an encoded ID of the base station, in addition to the un-encoded cell ID. 
In addition to the cell ID ($ID$) and public key ($K$), our base station certificate includes the location ID ($L$). $L$ includes the longitude and latitude of the base station and is thus a two-dimensional object, i.e., $L$=$(L_1$,$L_2)$ where $L_1$, $L_2$ are the longitude and latitude coordinate respectively.  %the first coordinate $L_1$ is the longitude coordinate and $L_2$ is the latitude coordinate. %The \emph{encoding} based on the geographical location (keeping track of longitude and latitude) enables the user equipment to cross-check with its own location to verify the location authenticity (the base station and the user equipment are within the physical range of each other). 
Base station's location information is public information, unlike the user equipment's location and behavior requiring privacy, and is thus appropriate for widespread delivery. For example, in the US, the FCC keeps track of the registered base station and publishes their cell IDs and the geographical locations~\cite{fcc_cell_data}%\syc{Cite the FCC database}
, which data is also what we use in our prototype implementation later for simulating the real-world base station deployments. 
% \syc{Include a diagram showing the data fields included in the certificate, and highlight our additions with a different color}
% \sw{} Fig.~\ref{fig:x509contents}

\subsection{Offline Certificate Delivery Using Blockchain}

\syc{Previously in the Intro but commented out}
% \syc{From here:}
% \syc{trying to do too much}
% We advance beyond %both the state-of-the-art practice (no authenticity and integrity protection) and 
% the state-of-the-art to enable greater security and efficiency. The state-of-the-art, the most prominent and related to our work~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}, do not make use of the base station's location and adopt PKI to append the public key within the base station's control communication, e.g., when delivering the first broadcast message in 5G RRC. %, and use that to authenticate the base station and its following control communications
% %~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}. %The related research works are generally covered in Section~\ref{rw}, but the most prominent and related works  
% Our novel location information addition on the base station certificate enables the defense against wormhole attacks %\syc{wormhole?} 
% that can launch fabricated radio control message broadcasting, handover exploitation, dispatching false alert messages, and bidding down attacks. %\syc{Fill these in. After the threat section drafting and establishing the terms, add the threats which gets defended by the location inclusion on the certificate}. 
% Our blockchain application provides a secure record/database of the registered base stations and their public keys/certificates and delivers them offline, which makes the online control communications shorter and enables the use of the cryptographic cipher with greater security/key length. Offline Base station certificate dissemination through blockchain also enables three times less energy consumption at the user equipment for signature verification than state-of-the-art.
% %\syc{Newly added:}
% Such base station certificate construction and delivery enables a multi-pronged approach for authenticating the base station and its radio-control communication message; the ID is used to check if the base station is registered and stored in the blockchain database; the location verifies the base station's location integrity; and the digital signature defends against malicious injections. 

% \syc{misplaced}
% \sour{Our rationale for using blockchain in offline communication for base station certificate delivery comes from the inherent byte size constraint of 5G radio control communication imposed by the physical layer. The base station can adopt Public Key Infrastructure (PKI) and send digital certificates to the user equipment in the first radio control broadcast message but according to the 3GPP standard, the physical layer limits message size up to 372 bytes~\cite{3gppphy} making it difficult to fit the base station certificates within the first radio control message. Moreover, in the PKI-based certificate delivery, the user equipment needs to verify the multiple certificates using the network public key installed within before authenticating the base station. The offline blockchain-based certificate delivery addresses both of the pitfalls with no byte length limitations while the secure delivery of base station certificates with its inherent property and the user equipment can authenticate the base station with lower computational time and with lower energy consumption.}

\vspace{-2px}
\subsubsection{Blockchain Enabler} % for Distributing the Base Station Certificate}
%\souc{May be we can considering the reordering of the subsections}
\label{subsec:our_scheme_blockchain}
%- Describe how blockchain play an important role here.
%\syc{Blockchain subsection drafted. I plan to revise.}

Blockchain enables the secure and offline delivery of the base stations' certificates. Blockchain is appropriate for such delivery because, unlike UEs, the base stations are public entities and publicly advertise their presence via broadcasting SIB1. The blockchain provides the public ledger including the ID (the cell ID as described in Section~\ref{subsec:background_5G}), the public key, and the location information of the legitimately registered and deployed base stations. 
%\syc{What is the ID we use?} \sou{cell id of the base station}

The blockchain ledger includes the digital certificates that are signed by the core network and whose subjects are the base stations (as well as the core network itself in the genesis block). % (validating and linking the base station's ID and its public key). 


The ledger validates and links the ID and the public key of the core network (self-signed in the genesis block) and the base stations (signed and vouched by the core network). The core network uploads its public key and certificate before it digitally signs and generates certificates for base stations, and the genesis block includes the core network's initial public key information. % the private key corresponding to the public key in that certificate is used for digitally signing the other certificates for the Base Stations. 
Because the core network signs and generates the digital certificates (after the base station generates the key pair and sends the public key to the core network), the core network uploads the digital certificates to the blockchain. The digital certificates in the blockchain ledger are verified, stored, and shared with all the entities involved in 5G networking, including mobile users. 

We use blockchain for the delivery of the base stations' certificates because of the following enabling blockchain properties. Blockchain provides \emph{message authentication integrity} by using the cryptographic primitives of public-key digital signature and the hash function. These cryptographic primitives are robust in security (the computational hardness assumptions) and anchor modern-day digital information and networking security. Blockchain provides easy access to its ledger information and builds on \emph{distributed storage and broadcasting} so that all the nodes store the blockchain ledger (including the base stations' certificates). The distributed storage and broadcasting enable the ledger to get \emph{automatically synchronized in various channels} (e.g., ad hoc connections or from previous base station connections) during the offline times, enabling easier access to the base station certificate information before the online phase using the cellular connectivity services. %For example, a nearby mobile or sensor user can deliver the newest block (containing the new public key of a base station) for the ledger synchronization in ad hoc/peer-to-peer networking. 

Our use of the blockchain is substantially simpler and cheaper than that used in other blockchain implementations, % permissionless cryptocurrencies, 
as described in Appendix~\ref{apndx:blockchain_os}. We further experimentally validate and analyze the appropriateness of blockchain for offline base station's certificate delivery in Section~\ref{subsec:offline_results}.
%\syc{Move the rest of the paragraph to appnedix} 

 
\vspace{-2px}
\subsubsection{Certificate Delivery Using Blockchain}
\label{subsec:our_scheme_cert_distribution}
While Section~\ref{subsec:our_scheme_blockchain} explains the blockchain used for certificate delivery, we describe how the decentralized blockchain ledger interacts with the rest of the entities. Fig.~\ref{fig:offline} illustrates our scheme protocol for the offline base station certificate construction and delivery. During the installation of the new base station or when the current digital certificate expires, the base station generates its own public-private key pair ($K, k$) for each cell. Then the base station sends a certificate signing request to the core network with an ID. Hence, the base station creates separate certificate signing request for each of its cell and send them to the core network for signing. In the certificate, the base station also includes its location information before sending a signing request. Upon receiving the signing request, the core network validates and signs the certificate of each cell of the base station and writes the signed certificate into the blockchain ledger. Only the core network has the write permission for the blockchain ledger. %A mobile user that wants to connect to a network need to synchronize base station digital certificates from blockchain ledger into its local storage. Initially, 

%\syc{New paragraph added to describe the ledger as a database of registered base stations}
The blockchain ledger serves as the registered database ($\mathcal{C}$) of registered base stations for the UE. The integrity of such records (i.e., only the core network can write and insert) relies on blockchain technology, as described in Section~\ref{subsec:our_scheme_blockchain}. When the base station presents its cell ID ($ID$), if the UE does not find it in its locally stored blockchain ledger, then it determines that the base station is not registered and certified by the core network. 

The user receives the base stations' certificates ($\mathcal{C} = \{ ID_i, K_i, L_i \}_i$) containing the public key and the location information via blockchain from its previous communications, e.g., the Internet using an infrastructure network or from another user through an ad-hoc network. %for the first time before initiating radio connection to the base station. Later on, the mobile user can synchronize the ledger periodically once its connected to the network.
As a part of the blockchain's validity check, the user verifies the base station's certificate using the core network's public key. 
%
The base station relies on the core network to validate its public key because we assume the core network resides in a secure confinement of the service provider and the attacker will not have access to the core network to forge the digital certificate of the base stations or upload malicious certificates into the blockchain ledger. 
%Blockchain based PKI framework is significantly important here to distribute the public keys of base stations to mobile user using a minimal version of X.509 digital certificate. 





% Simeon version: output boolean, b, remove descriptions in the inputs/outputs/parameter % put `certificate` in math cal, unnecessary comments, right align the comments
\begin{algorithm}[t!]
\small
    \caption{Online Multi-pronged Authentication at UE}
    \label{algo:auth}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Parameter}{Parameter}
    
    %\underline{function authentication} ($n$, $t$, $\tau$, $S_k$, cell\_ID, $\bar{L}$, $\bar{t}$)\;
    %\Input{($n$, $t$, $\tau$, $S_k$, ID_i) received in online phase (SIB1) \\
    %and ($\bar{L}$, $\bar{t}$) measured at the user}
    \Input{\emph{SIB1}, $ID_i$, $n$, $t$, $S_k$, $\bar{L}$, $\bar{t}$ \hfill \hfill /* \textit{Online communication} */ }
    \Output{$\mathcal{A}$ \hfill \hfill /* \textit{Authenticated? True (1), False (0)} */}
    \Parameter {$\tau_t$,$\tau_d$}
    %/* \textit{Query certificate in blockchain ledger database using cell ID} */ \\
    \If{$\mathcal{C}.ID_i$ == $ID_i$}
    {
       %/* \textit{Get $K$, $L$ from blockchain ledger corresponding to cell ID} */ \\
       $K_i$, $L_i$ = get($ID_i$,$\mathcal{C}$.$K_i$, $\mathcal{C}$.$L_i$)  \\

      % /* \textit{Calculate distance between the base station and the user} */ \\
       $d$ = distance($L_i$, $\bar{L}$)  \\
      % /* \textit{Calculate SIB1 generation and reception time difference} */ \\
       $\Delta t$ = $\bar{t} - t$ \\
      % /* \textit{Base station authentication} */ \\
       \If{$d \leq \tau_d$ \textnormal{\textbf{\&\&}} $ \Delta t \leq \tau_t$ \textnormal{\textbf{\&\&}} $V_{K_i}$(SIB1,$n$,$t$,$S_k$) == 1}
       {
           \textnormal{\textbf{return}}  $\mathcal{A} = 1$ \hfill /* \textit{Authenticated} */ \\
       }
    }
    \textnormal{\textbf{return}} $\mathcal{A} = 0$ \hfill /* \textit{Not authenticated} */ \\
\vspace{-4px}
\end{algorithm}





% Sourav version:
% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
    
%     \underline{function authentication} ($n$,$t$,$\tau$,$S_k$, cell ID,$\bar{L}$,$\bar{t}$)\;
%     \Input{($n$,$t$,$\tau$,$S_k$, cell\_ID) received in online phase (SIB1) and ($\bar{L}$,$\bar{t}$) measured at the user}
%     \Output{$1\leftarrow$ authenticated, $0\leftarrow$ not authenticated}
%     Query certificate in blockchain ledger database using cell ID \\
%     \If{$certificate.ID=$ cell ID}
%     {
%        /* Get $K$, $L$ from blockchain ledger corresponding to cell ID */ \\
%        $K,L$ = get($certificate.K,certificate.L$)  \\

%        /* Calculate distance between the base station and the user */ \\
%        calculate $d$ = distance($L$,$\bar{L}$)  \\
%        /* Calculate SIB1 generation and reception time difference */ \\
%        $\Delta t$ = $\bar{t} - t $ \\
%        $T\leftarrow$ SIB1 freshness threshold \\
%     \If{$d \leq \tau$ \textnormal{\textbf{and}} $T \leq \Delta t$ \textnormal{\textbf{and}} $V_K$(SIB1,$n,t,\tau,S_k$)}
%          {
%             return 1;\
%          }
%     }
%     return 0\;
%     \caption{Online Base Station Authentication}
%     \label{algo:auth}
% \end{algorithm}


% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
    
%     \underline{function auth\_id} $(ID)$\;
%     \Input{$ID$ received in SIB1 (Cell ID)}
%     \Output{$(K,L)$ or Null}
%     Query certificate in blockchain ledger database using $ID$ \\
%     \eIf{$certificate.ID=ID$}
%       {
%         return $(K,L)$\;
%       }
%       {
%         return Null\;
%       }
%     \caption{Online Base Station ID Authentication}
%     \label{algo:auth_ID}
% \end{algorithm}

% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \underline {function distance} ($(L,\bar{L}$)\;
%     \Input{Base Station location: $L(L_1,L_2)$ from base station certificate as output from Algorithm \ref{algo:auth_ID} \\
%     UE location: $\bar{L}(\bar{L_1},\bar{L_2})$ retrieved by the user} 
%     \Output{$d$}
%     Calculate $d = \sqrt{(L_1-\bar{L_1})^2 + (L_2-\bar{L_2})^2}$
%     \\
%     \underline{function auth\_location} ($\tau,d)$)\;
%     \Input{calculated distance: $d$ from \underline {function distance}, distance threshold: $\tau$ from SIB1 message}
%     \Output{$1\leftarrow$ Valid, $0\leftarrow$ Invalid}

%     \eIf{$d \leq \tau$}
%       {
%         return $1$\;
%       }
%       {
%         return $0$\;
%       }
%     \caption{Online Location Authentication\sw{Make sure all variables are defined in main body as opposed to in the pseudocode, also incorrect definition of a 2D vector, $\mathbf{L} = \begin{bmatrix}
% L_1 \\
% L_2
% \end{bmatrix}$}}
%     \label{algo:auth_location}

% \end{algorithm}

% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \underline{function auth\_message $V_K$} (SIB1,$n,t,\tau,S_k$)\;
%     \Input{message: SIB1, $n,t,\tau$ Signature: $S_k$ from SIB1 Public key: K from base station certificate}
%     \Output{$1\leftarrow$ Valid, $0\leftarrow$ Invalid}
    
%     \eIf{$V_K$(SIB1,$n,t,\tau,S_k$)}
%       {
%         return $1$\;
%       }
%       {
%         return $0$\;
%       }
%     \caption{Online Message Authentication}
%     \label{algo:auth_msg}
% \end{algorithm}

\subsection{Online Multi-Pronged Base Station and Message Authentication}

\vspace{-1px}
\subsubsection{Existing 5G Protocol}
\label{subsec:our_scheme_existing_5G}
Our scheme builds on the existing 5G RRC protocol for compatibility and practicality (facilitating deployment), and this section builds on Section~\ref{subsec:background_5G} but provides greater details for the 5G RRC protocol interactions between the UE and the base station. Fig.~\ref{fig:online} shows the standard 5G control communication protocol messages in black font color. The UE uses such RRC communication protocol so this is a part of the online phase.  


%
%
%\syc{Start with why this subsection is so important for our work, e.g., compatibility. Refer to Fig.~\ref{fig:online}}\sou{Main focus of this paragraph is explaining the insights of Fig.~\ref{fig:online}. -Base station transmits SI messages periodically -Mobile user wait until next broadcast schedule to get SIBs.}\\
%In this work, we introduce base station broadcast message authentication by the mobile user in Radio Resource Control (RRC) layer of the standard 5G cellular network protocol defined by 3GPP. In Fig.~\ref{fig:online} we show the standard 5G control communication protocol messages in blue font color. \sou{Size limitation of SI messages: Physical layer TBS calculation} At first, the mobile user uses information received from Physical Downlink Shared Channel (PDSCH) signalling and Downlink Control Information (DCI) to determine the transport block size (tbs) that determines the amount of information receives by upper layer. The transport block size depends on modulation order, target code rate, redundancy version, number of resource block that is available at the mobile user using DCI signalling. We illustrate this process as physical layer signaling that takes place at the very first communication from base station to mobile user. It is important to note that according to 3GPP standard \cite{3gppphy}, the amount of information the mobile user expected to receive in system information message is determined by the transport block size (tbs) which is 2976 bits (372 bytes). 

In 5G NR RRC layer, after the initial physical layer synchronization signaling, the base station transmits system information messages with different periodicities: MIB broadcast message with a periodicity of 80 ms, SIB1 with a periodicity of 160 ms, and other SIBs with a periodicity scheduled in SIB1 (20 ms by default) \cite{3gpprrc}. It is minimum for the UE to acquire MIB and SIB1 since they contain essential radio connection-related information and the UE has to wait to get the system information message until its next broadcast schedule.

Therefore, the UE can only initiate an RRC connection request once it gets all the necessary information from system information messages and later on the complete RRC connection setup using a three-way handshake. After a successful RRC layer connection with the base station, the UE proceeds to set up a NAS layer connection with the core network. We omit the control communication between the base station and the core network in this work as it is out of the scope of our research. 

%  Prior to setup RRC connection with base station, the mobile user periodically receives a number of broadcast messages to get necessary information about the network. Master Information Block (MIB) and System Information Block Type1 (SIB1) are called Minimum SI since they are essential for the mobile user to get initial radio connection related information. The base station transmits MIB with 80ms and SIB1 with 160ms periodicity. The periodicity of other system information messages are scheduled in SIB1. 

\subsubsection{Signature Generation at Base Station}
\label{subsec:online_signature_generation}
%\sw{Make it d for distance, tau for distance threshold}
% \sou{Getting rid of nonce in our scheme, because it seems it does not server much purpose in replaying attack. Rather we send timestamp and time threshold. These timebased values will serve the same as nonce. Time itself if a nonce.}

%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%%%%%%%%
% Fig.~\ref{fig:online} depicts the online RRC communication protocol. Before broadcasting SIB1 message the base station generates a digital signature $S_k$(\emph{SIB1},$t$,$\tau_t$,$\tau_d$) on \emph{SIB1}, a timestamp ($t$), a time threshold ($\tau_t$) and a distance threshold ($\tau_d$) using its private key ($k$). The timestamp ($t$) is the SIB1 generation time at the base station and the time threshold ($\tau_t$) is the SIB1 expiration time set by the base station. We use $t$ and $\tau_t$ for replay attack protection during each SIB1 message broadcast. The distance threshold ($\tau_d$) signifies over-the-air the coverage range of the base station that we use to prevent wormhole attacks. The base station appends the digital signature along with the other parameters to the \emph{SIB1} message and broadcasts it. The final SIB1 transmission appends the following:\{\emph{SIB1},$t$,$\tau_t$,$\tau_d$,$S_k$(\emph{SIB1},$t$,$\tau_t$,$\tau_d$)\}.
%%%%%%%%%%%%%%%%%%%% Option 2 %%%%%%%%%%%%%%%%%%%%%

Fig.~\ref{fig:online} depicts the online RRC communication protocol. Before broadcasting SIB1 message the base station generates a digital signature $S_k$(\emph{SIB1},$n$,$t$) using its private key ($k$) as defined in Section~\ref{subsec:background_public_key}. % on \emph{SIB1}, a nonce ($n$), and a timestamp ($t$) using its private key ($k$). $S_k$ is defined in . 
We use the SIB1 generation timestamp ($t$) and the nonce ($n$) for replay attack protection during each SIB1 message broadcast. The base station appends the digital signature along with the other parameters to the \emph{SIB1} message and broadcasts it. The final SIB1 transmission appends the following: \{\emph{SIB1},$n$,$t$,$S_k$(\emph{SIB1},$n$,$t$)\}.

\subsubsection{Multi-pronged Authentication at UE}
\label{subsec:our_scheme_online_auth}
%\subsection{Online ID and L. Authentication at UE} % Base Station ID/Registration and Location Authentication}
%\syc{Let's draw a pseudo-code showing the online verification from the user equipment perspective. Start by stating what have been given offline vs. online because these are the inputs of the algorithm; these variables-given are in the Key Component Figure, currently Figure 4, but it would be good to use that to build the rest of the algorithm, including for the location authentication using the distance threshold $\tau$. Is the $\tau$ the distance or the distance threshold?}
The UE takes a multi-pronged approach to the base station authentication in the online phase. Algorithm~\ref{algo:auth} depicts the step-by-step procedure of the online multi-pronged base station authentication that consists of base station ID authentication, location authentication, and SIB1 message authentication. The UE receives registered base station certificates $\mathcal{C} = \{ ID_i, K_i, L_i \}_i$ via the blockchain ledger during the offline phase as described in Section~\ref{subsec:our_scheme_cert_distribution}.
%The UE receives base station ID ($ID$), public key ($K$), and location ($L$) through the blockchain ledger during the offline phase. 
During the online phase, it receives $ID_i$, $S_k$, $n$, and $t$ via the SIB1 message from a base station with index $i$ as described in Section~\ref{subsec:online_signature_generation}. The UE measures its location information ($\bar{L}$) and SIB1 reception time ($\bar{t}$) which we use for base station location authentication. In addition, the UE selects two control parameters: the time threshold ($\tau_t$), and the distance threshold ($\tau_d$) to thwart replay and wormhole attacks by location authentication. $\tau_t$ is the upper bound that the UE accepts any SIB1 message as fresh. $\tau_d$ is the upper bound of the distance between the UE and the base station that sends the SIB1 message. Our rationale for selecting the time and distance threshold at the UE is to give the UE flexibility to select base stations not only based on the higher received signal strength but also the distance from it and the freshness of the SIB1 message that it receives. The UE can make a logical decision while choosing a base station (because higher signal strength with a lower distance is more logical than higher signal strength with a greater distance). A successful multi-pronged authentication returns the Boolean $\mathcal{A}$, where $\mathcal{A} = 1$ stands for authenticated and $\mathcal{A} = 0$ stands for not authenticated.

The online multi-pronged authentication begins with authenticating the base station ID. After receiving SIB1 messages the UE extracts the $ID_i$ from the message and performs a certificate query within $\mathcal{C} = \{ ID_i, K_i, L_i \}_i$. If the UE finds a relevant base station certificate from $\mathcal{C}$ then we say it validates the ID of the base station. The base station ID validation helps the UE to determine whether the base station is registered within the operator network. A successful query returns with a base station certificate containing the public key ($K_i$) and the location ($L_i$) information of the base station. %Algorithm~\ref{algo:auth_ID} shows the pseudocode for the base station ID authentication.

Upon successful base station ID authentication, the UE uses the $L_i$ and $\bar{L}$ to authenticate the location. At first, the UE calculates the distance ($d$) between itself and the base station using their location information ($L$,$\bar{L}$). We also add a replay attack protection mechanism in location authentication. For that, it calculates the time difference ($\Delta t$) between $t$ and $\bar{t}$. Finally, the UE validates the location authentication if the two conditions are satisfied: (a) $d$ is less than or equal to $\tau_d$, and (b) $\Delta t$ is less than or equal to $\tau_t$. Upon successful location authentication, the UE proceeds to SIB1 message authentication.

% As shown in Algorithm~\ref{algo:auth_location} the UE performs location authentication using two functions: calculating the distance($d$) between its own and the base station after retrieving its own location ($\bar{L}[\bar{L_1},\bar{L_2}]$), and validating if the calculated distance is within the received distance threshold($\tau$). The UE uses the Euclidean formula to calculate the distance. If the calculated distance ($d$) is less than or equal to the distance threshold ($\tau$) then the UE authenticates the location of the base station. The UE gets base station location ($L[L_1, L_2]$) information from the base station certificate offline and distance threshold ($\tau$) from SIB1 online. 

%%%%%%%%%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%
% The location authentication prevents the wormhole attack and the replay attack. The base station sets the distance threshold ($\tau_d$) because its coverage range depends on several factors: spectrum, terrain, and transmitting power. As the frequency band increases the coverage range of a base station shrinks. The coverage area decreases in urban areas with more obstacles than in rural areas for a particular frequency band. However, increasing transmitting power expands the coverage range. Typically a 5G base station operating in millimeter wave frequency has $15$ to $600$ meters of coverage range. The base station also sets the SIB1 expiration time threshold ($\tau_t$) based on its transmission characteristics. The rigorous analysis of distance threshold and time threshold calculation is beyond the scope of this research work.

%%%%%%%%%%%%%%%%%%%%%% Option 2 %%%%%%%%%%%%%%%


%\vspace{-12px}
%\subsection{Online Message Authentication at UE} %\subsection{Online Base Station ID and Message Authentication}
%\label{subsec:our_scheme_online_auth}
%\label{sec:online_bs}
%- Describe the authentication process. \\
%- Include design diagram here.
%\syc{The online section should include the following: the authentication of the IDs (including the location authentication) and the message authentication via the digital signature. We may want to split the two subsections}\\
%\souc{Below paragraph deserves an earlier position as it describes base station generating SIB1 message with signature.}
%\sw{Using $\tau$ instead of $d/d$}

%% Moving to an ealier new section
% Fig.~\ref{fig:online} depicts the online RRC communication protocol. Before broadcasting \emph{SIB1} message the base station generates a digital signature $S_k$(\emph{SIB1},$n$,$t$,$\tau$) on \emph{SIB1}, a nonce ($n$), a timestamp ($t$) and a distance threshold ($\tau$) using its private key ($k$). The nonce ($n$) is an arbitrary value and the timestamp ($t$) is the SIB1 generation time at the base station. We use $n$ and $t$ for replay attack protection during each \emph{SIB1} message broadcast. The distance threshold ($\tau$) signifies over-the-air the coverage range of the base station that we use to prevent wormhole attacks. Finally, the base station appends the digital signature along with the other parameters to the \emph{SIB1} message and broadcasts it. The final \emph{SIB1} transmission appends the following: \{\emph{SIB1},$n$,$t$,$\tau$,$S_k$(\emph{SIB1},$n$,$t$,$\tau$)\}.


% The mobile user ensures the availability of its offline blockchain ledger within its local storage prior to initiating the RRC connection. Upon reception of \emph{SIB1}, \sou{we introduce three additional processing along with standardized \emph{SIB1} message handling: (a) get base station certificate (b) verify time and location of \emph{SIB1} (c) verify the digital signature.} At first, the mobile user looks up the \sou{base station certificate} from the blockchain ledger in its local storage using the \emph{ID} received in \emph{SIB1}. \sou{The base station certificate contains the public key ($K$) and the location ($L$) of the base station which are used for authentication and location verification. }

%\syc{Some of these would need to move to the previous section, as it focuses on the location authentication}
%\souc{From here the UE message authentication begins} \\

%%%%%%%%%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%
% Finally, during the message authentication, the UE verifies the digital signature $V_K$($S_k$(\emph{SIB1},$t$,$\tau_t$,$\tau_d$)) using the public key $K$. This validation ensures the authenticity and integrity of the contents of the SIB1 message. After successful verification of the digital signature, we say the base station is authenticated. Then, the UE proceeds to establish an RRC connection with the base station and then the NAS connection with the core network. If the base station is not authenticated then it again starts listening to system information messages from other base stations. 

% In the online phase of our scheme, we add the following four additional data fields in the SIB1 and increase the transmitted Bytes: the digital signature, the timestamp, time threshold, and the distance threshold value. In computations, we add digital signature generation at the base station. At the UE, we add base station ID authentication and certificate reading from the blockchain ledger, location authentication, and message authentication. Algorithm~\ref{algo:auth} depicts the step-by-step procedure of the online base station authentication.

%%%%%%%%%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%
%\syc{Describe and explain $\mathcal{A}$}
Finally, during the SIB1 message authentication, the UE verifies the digital signature $V_K$($S_k$(\emph{SIB1},$n$,$t$)) to validate the authenticity and integrity of the SIB1 message. Successful verification of the digital signature yields $\mathcal{A} = 1$ which means online multi-pronged authentication at UE is successful. Then, the UE proceeds to establish an RRC connection with the base station and the NAS connection with the core network afterward. If $\mathcal{A} = 0$ then UE again starts listening to system information messages from other base stations. 

In the online phase of our scheme, we add the following three additional data fields in the SIB1 and increase the transmitted Bytes: the digital signature, nonce, and timestamp. In computations, we add digital signature generation at the base station. At the UE, we add base station ID authentication and certificate reading from the blockchain ledger, location authentication, and message authentication. 

==> Sections/Old_Tex_Files/04092023_Background.tex <==
\section{Background}
\label{sec:background}
In this section, we briefly review the overall architecture and radio control communication of 5G cellular network. We also discuss related information regarding offline-online aspect of our authentication scheme.
%\syc{5G-specific message types, e.g., MIB, SIB, should be defined and described here. How they are relevant to our work also needs to be explained.}

\subsection{Radio control in 5G cellular network}
5G cellular network consists of three main components: User Equipment (UE), Next Generation Radio Access Network (NG-RAN) and the 5G core (5GC). Although, 5G core consists of important nodes (such as AMF, AUSF, SMF etc.) for different functionality, in this paper we abstracted all of these nodes as 5G Core Network(CN). NG-RAN comprises of base stations which act as a trusted intermediary node between the UE and the 5G core and are distributed across a wide geographical area for cell coverage. UE needs to establish radio connection using Radio Resource Control (RRC) with base station before it gets connected to the core network to avail the cellular services (voice, data).

A base station periodically broadcasts \textit{System Information (SI)} messages to advertise its system parameters (such as cell id, plmn id, tac, frequency info etc.) so that an UE use them during initial connection setup, mobility information or receiving public broadcast messages. These \textit{system information} messages are of two types \textit{Master Information Block (MIB)} and a number of \textit{System Information Blocks (SIBs)}. \textit{Master Information Block} and \textit{System Information Block Type1 (SIB1)} are called \textit{Minimum SI} since they are essential for the User Equipment to get initial cell access related information. The \textit{MIB} broadcast message contains a limited number of essential parameters that are needed to acquire \textit{System Information Block Type1 (SIB1)} and is transmitted with 80 ms periodicity (40 ms in LTE). \textit{SIB1} is cell-specific and transmitted with a periodicity of 160 ms that contains essential system parameters and scheduling information about other \textit{system information (SI)} messages. However, the maximum number of bit that any SIB message can transmit depends on the physical layer and it is 2976 bits (372 bytes) in 5G. During the initial radio connection, UE scans for these broadcast network messages and chooses a suitable base station cell to get connected based on \textit{system information} messages signals with higher signal strength. After acquiring these SI messages UE establish RRC connection with base station and Non-Access Stratum (NAS) connection with core network. However, there is no authentication mechanism for the UE to validate the legitimacy of the base station \textit{SI} messages before camped to it. An attacker can exploits this vulnerability and launch data privacy and security attacks on UE.

\subsection{Digital Signatures and Certificates}
In terms of message authentication (or integrity) there are two popular methods: symmetric key based message authentication code  and asymmetric key based digital signature. The drawback of message authentication code is it cannot protect the message from repudiation and a private key needs to be shared magically between communicating parties. On the other hand digital signatures use a private key to sign a message and corresponding public key to verify it. Although it is computationally costly as compared to MAC techniques yet digital signatures are more secure and convenient in several ways: convenient key distribution and management, publicly verifiable signatures and more importantly it has non-repudiation property. 

While the verifier needs the public key of signer to verify a digital signature, a trusted authority (whom the signer and verifier can trust) can signs the public key of the signer in a digital certificate and it can be share with the verifier through an authentic channel. The trusted party, in this case called the Certificate Authority (CA), plays an important role for public key distribution in the digital signature based message authentication scheme. The certificate itself must contains some mandatory information field so that the verifier can retrieve public key for a specific signer. 

%- What digital signature algorithms we are considering and why? We are going to implement ECDSA, RSA, PQC consecutively.

%- For digital signatures what type of certificate we are going to use and why? We are going to use X.509 V1 with mandatory fields.

%
%\subsection{Commit-and-Reveal Scheme}
%The commit and reveal scheme in cryptography allows the sender to a commit a message by generating hash of it and %send it to the receiver and reveal the committed message later on so that receiver can verify the hash it received %from the sender after generating the hash from the reveal message. This idea can be utilized in message integrity %protection in data communication where any sender wants to send multiple consecutive messages to the receiver. The %commit-and-reveal method is less costly as compared to digital signature since only hash functions are used.
%

\subsection{Offline and Online phases in PKI based Signature}
PKI based Digital signature schemes consists of three stages: key generation, signing and verification. Key pair (private and public) generation and distribution is a single time activity within a certain period of time. The public key can be distributed through digital certificates with a certain validity period. On the other hand, digital signature generation by sender and verification by the receiver is a multiple time activity as long as the digital certificate is valid. Thus, to reduce computation overhead and faster execution, the whole process can be divided into two phases: 1) Offline key generation and distribution 2) Online signature generation and verification. Likewise, key generation and digital certificate distribution of a base station can be done in offline prior to initiate communication to the users whereas signing and verifying can be done online during communication.

%- How we divided our scheme into online and offline parts with example.
%- Can include some references regarding offline and online aspects of PKI. How it enhanced efficiency.


==> Sections/Old_Tex_Files/04092023_Related_Work.tex <==
\section{Related work}
\label{rw}
\subsection{Fake or Malicious Base Station}
\label{subsec:related_malicious_bs}

The lack of base station authentication can facilitate an attacker to install fake base station and force legitimate users to connect to it by emitting higher signal strength than the legitimate base stations~\cite{yang2019hiding,DBLP:conf/ndss/ShaikSBAN16,hussain2018lteinspector}. This, in turn, encourages an attacker to perform several security and privacy attacks on the user. In~\cite{rupprecht2019breaking}, the authors set up a fake base station and alter the destination IP address of the DNS request of the user to launch DNS redirection attack. The authors in~\cite{kim2019touching} show that an attacker can launch AKA bypass attack to receive the user data without any encryption and remote deregistration attack to disconnect the user from the core network using fake base station. Bidding down attack~\cite{DBLP:conf/ndss/ShaikSBAN16,shaik2019new,3gppfbs} to downgrade the user to 2G/3G network and battery draining attack~\cite{shaik2019new,hussain20195greasoner} are possible by establishing a fake base station between the user and legitimate network. An attacker with a fake base station can also track a user’s location~\cite{DBLP:conf/ndss/ShaikSBAN16,hussain2018lteinspector,arapinis2012new,hussain2019privacy,hussain20195greasoner}, prevent a user from using selected/all networked services with denial-of-service attack~\cite{DBLP:conf/ndss/ShaikSBAN16,hussain2018lteinspector,shaik2018impact,chen2021bookworm,hussain20195greasoner} and launch SMS phishing attack~\cite{zhang2020lies,mulliner2011sms}. However, these attacks are feasible only after the successful connection establishment between the user and fake base station. Our base station authentication mechanism prevents these attacks by allowing only legitimate base stations to connect to the user. 
% and disregard the connection establishment messages from fake base station by a user.    

\subsection{Base Station Authentication}
\label{bsa}
\as{in this section, I assume that we will discuss in the contribution section that our scheme does not require to depend on the base station to get the public key. Hence, that point is not described here again.}
In this section, we describe and compare our work with the existing works related to the base station authentication using public key dissemination. In~\cite{hussain2019insecure}, the authors propose a Public-Key Infrastructure (PKI) based authentication scheme to secure the SIB messages between the user and base station. However, this scheme requires to verify the whole certificate chain (containing the certificate of core network entities and base station) by the user. More importantly, the user can verify both SIB1 and SIB2 message only after the reception of the SIB2 message. These two factors cause high verification overhead for base station authentication by the user. However, in our scheme, the user does not need to verify the whole certification chain and buffer the SIB1 message resulting in less verification overhead. The authors in~\cite{singla2021look} propose hierarchical identity-based signature scheme (Schnorr-HIBS) based broadcast authentication protocol for authenticating legitimate base station by securing the SIB messages between user and base station. However, this approach requires multi-party computation (includes significant overhead for offline key generation and distribution than our scheme) for generating the signature to sign the SIB1 messages and have communication overhead of 150 bytes. On the contrary, our scheme does not require multi-party computation and has less communication overhead (68-140 bytes depending on the signature algorithm used). 3GPP~\cite{3gppfbs} suggests delegating the signing process of SIB messages by digital signing network function (DSnF) in the core network instead of the base station and have more communication delay~\cite{gao2021evaluating} than our scheme. 3GPP~\cite{3gppfbs} also suggests base station authentication based on digital signatures or identity-based cryptography, however, this mechanism only applies during the cell reselection in RRC idle and inactive mode. There are also PKI-based solutions for mutual authentication between the user and base station where the user initiates the authentication process and incurs high communication overhead~\cite{yi1998optimized,zheng1996authentication}.      
 

% //////3GPP~\cite{3gppfbs} suggests base station authentication based on digital signatures or identity based cryptography. However, this mechanism is not applicable during the initial registration procedure, thus cannot secure the initial bootstrapping messages, i.e., SIB messages and only applies for the verification of legitimate base station during the RRC idle and inactive mode.      


\subsection{Fake or Malicious Base Station Detection}
% \as{This section can be merged with the previous one.}
The other defense approach (except the public-key dissemination-based base station authentication described in Section~\ref{bsa}) is to blacklist fake base stations after the detection~\cite{singla2021look}. One such technique involves utilizing measurement reports of the users to find discrepancies among the parameters (e.g., base station identifier, received signal strength etc.) in the legitimate base stations and fake base stations~\cite{3gppfbs}. Several other techniques explore using specialized smartphone applications, hardware and machine learning applications~\cite{dabrowski2014imsi,alrashede2019imsi, dabrowski2016messenger,do2016strengthening,nakarmi2021murat,steig2016network} to collect network data and detect attack presence in the network. However, these solutions do not address the root vulnerability (i.e., insecure bootstrapping messages) that enables attackers to launch fake base station attacks and can detect fake base stations only after the attack happens.  
 

% Several other techniques \cite{dabrowski2014imsi,alrashede2019imsi} explore using specialized smartphone applications and hardware to collect network statistics and detect attack presence in the network. Some works\cite{dabrowski2016messenger} propose machine learning based applications using network statistics data (detecting cipher downgrade, relayed traffic, Unknown TAI, LAI (Location Area Identity) etc.) and \cite{nakarmi2021murat} compare measurements of parameters (RSSI, PCI, RSRQ etc) from mobile phones with the same measurement mobile networks assumes that phones should have. However, these solutions do not address the root vulnerability that enable attackers to launch fake base station attacks and are provided for LTE technology.  

\subsection{Blockchain for Key Management and PKI}
\as{Do we need this subsection for globecomm since the page limit is tight? Or will we consider writing in the introduction section that there are previous works focusing (then the citations of these papers) on to secure key management and PKI  blockchain for different use cases, however, we use blockchain to secure the key management for base stations in the cellular network.} Previous works propose using blockchain to secure key management and PKI for different use cases. We use blockchain to secure the key management for base stations in the cellular network. The authors in~\cite{yakubov2018blockchain} propose blockchain-based PKI framework with hybrid X.509 certificate and smart contract for chain of trust validation. In~\cite{al2017scpki}, the authors propose smart contract-based web of trust model to verify or vouch for identity attributes and detect rogue certificates by publishing all the certificates to the network immediately. Authors in~\cite{matsumoto2017ikp} propose Instant Karma PKI (IKP) for reporting unauthorized certificates to prevent CA misbehavior using an incentive approach based on Ethereum blockchain. A blockchain based naming and storage system (Blockstack)~\cite{ali2016blockstack} solves building decentralized services, e.g., decentralized version of DNS and PKI with small CPU overhead.  

% \subsection{Malicious User}
% \as{from Dr. Chang: malicious user is not related our threat model, probably we can clarify that in the background. }
% Impact of malicious user on preventing the connection between user and base station/core network. A malicious user ...In~\cite{kim2019touching} the authors describe about blind DoS and remote de-registration attack where the attacker obtaining the temporary identifier (e.g. using silent paging attack) (\as{if define in the background, no need of explanation, otherwise need to say it is the S-TMSI}) of the user can spoof the RRC (\as{term description in the background??}) connection of the user and disconnect it from the base station/core network. Moreover, the attacker as a malicious user can send repetitive RRC connection establishment (\as{need check if we discuss this in background}) requests to the base station to prevent legitimate users from connecting to the base station by exhausting the the RRC connection capacity of the base station~\cite{kim2019touching}.     

==> Sections/Old_Tex_Files/07222024_Abstract.tex <==
\begin{abstract}
%\syc{Drafted/revised, but let's check again later}

% \syc{Construction->Delivery->multi-factored authentication}
Malicious or rogue base stations are critical and well-studied issues in telecommunication networking. %While there are digital security between the user and the backend core network, 
However, the current cellular practice in 5G remains vulnerable and there are no keys for base stations to enable the base station authentication. % when the user equipment communicates with the base station to establish the wireless channel and radio resource control. % and the R\&D community only recently proposed to introduce the base station's public key. 
To secure the base station authenticity and message integrity, we introduce and design the base station digital public-key certificate and analyze the security benefits informed by our base station vulnerability and threat analyses. 
We build our scheme to construct, deliver, and use the base station certificate. 
% We design, build, and deliver the base station digital certificate %(including both its construction and dissemination) 
% and use it %the resulting delivered certificate information 
% to secure the message authenticity of the communication-link control communication between the base station and the user equipment. 
% While we study our scheme from the base station digital certificate construction to delivery to use for multi-factored authentication, our research contributions beyond the existing research are more heavily in the base station digital certificate construction and delivery. 
For the construction, we include the information fields which individually have security benefits, including the base station location information which has not been used in other certificate applications. %, and analyze how each of the information fields of ID, location, and public key enable the authenticity and integrity against various base station threats. 
For the delivery, we use blockchain for delivering the base station certificate offline, which enables greater key length/security strength and computational efficiency than the state-of-the-art research delivering 
the public key during the base station's online control communication. %, our scheme therefore enables greater key length/security strength and computational efficiency. 
We then use the certificate to implement a multi-factored authentication using the ID, public key, and location delivered by the certificate in the 5G control communication with the user equipment. 
We take a systems approach to analyze and validate our scheme including the vulnerabilities/threats, security, performances, and fit to the existing standardized networking protocols. 
%
% While building on the related standardized technologies, % for most parts, %for practicality, %for both the digital-certificate-based key establishment and the digital-signature-based message authenticity protection. However, we 
% we make novel contributions to advance the security.
% We include the base station's location information in the certificate construction, use blockchain for the offline delivery of the certificate database, and incorporate multi-factored authentication verification during the online real-time communications between the user equipment and base station. 
% %We construct the base station certificate to include the base station's location information to defend against location spoofing and replay threats, which is novel compared to the existing certificates. Our scheme then delivers the base station digital certificate database including the registered base station records using blockchain building on its strengths of high integrity (only the core network can write on the blockchain and distribute the keys) and automatic and distributed synchronization and delivery. Both the certification construction and distribution occur offline before a user equipment (verifier) encounters the base station (prover). The base station public key authenticated by the digital certificate and the blockchain gets used in the communication-link control communication for setting the wireless communication channel including medium access control and radio recourse control. 
% Because our work spans from certificate construction to delivery to the %certificate information use for 
% multi-factored authentication, we take a systems approach for our research to analyze and validate our scheme including the vulnerabilities/threats, security, performances, and fit to the existing standardized networking protocols. We analyze the rogue base station vulnerabilities/threats (including those based on new ID, spoofing, message injections, and replay/wormhole) and compare our work with the state-of-the-art research against those threats. 
Our work involves an implementation %SDR radios and relevant softwares to implement a prototype 
building on X.509 certificate, smart contract-based blockchain, and 5G New Radio-standardized RRC %control
communications. % and systematic analyses of the changes we made from the existing technologies. 
Our %proof-of-concept 
analyses and SDR-radio-based experiments show that our scheme defends against more threats and can enable stronger security (i.e., our scheme can use ECDSA with key lengths of 256, 384, 521, 571 bits in 5G RRC communication, while only ECDSA with 224-bit key have been supported by previous research). %which could not be supported by previous research). 
We also show that our scheme design for the certificate's offline delivery and the authentication use enable the computing and energy to be more than 3.2 times efficient than the state-of-the-art research on the mobile user equipment. 

% We design and build a blockchain-based key distribution scheme and then use the key to authenticate the base station in 5G radio resource control (RRC) in which the base station transmits a digitally signed broadcast message. The blockchain delivers the base station's public key and builds on its strengths of high integrity (only the core network can write on the blockchain and distribute the keys) and automatic, distributed, and offline synchronization and delivery. %, advancing the start-of-the-art research which distributes the keys in the broadcasting and bandwidth-limited RRC chanenls at the time of the communications. 
% Our base station authentication uses the 5G RRC protocol's SIB1 message transmission (regularly broadcasted to the nearby mobile users) and enables the public-key authentication using the digital signature ciphers with greater security levels than the previous research (by offloading the base station's public key distribution in the offline blockchain). We implement and validate our scheme for both offline key distribution and online cellular communications. % (offline is before the telecommunication session and online is during). 
% Our implementations simulate the user, base station, and core network and involve radios and computers for both the online 5G communications (srsRAN and SDR) and offline key distribution (Ethereum smart contract with the third-party blockchain transmitter in both the local ad hoc and Internet-remote environments). %For such systems study and implementation, in addition to simulating the telecommunication entities (user, base station, and core network), we implement a third-party node to highlight the distributed delivery of the base station's public key (while only the core network can write, anybody can store and transmit the blockchain). %We use srsRAN and software-defined radio (SDR) for the online base station authentication and RRC communications between the user and the base station, and use Ethereum smart contract for the offline key delivery. % To highlight the automatic and robust blockchain-based key distribution, we also implement the offline key delivery (before the user becomes active for telecommunication networking) in both local and remote experiments and show how the blockchain is appropriate for base station's public key distribution. 
% Our experiments show that our scheme can support ECDSA with greater key lengths/security and that the mobile user's computing and energy consumptions are more efficient than the state-of-the-art research due to the blockchain-based offline key distribution. %because the offline key distribution enables the authentication using just one signature verification. 
% % \syc{What are the result highlights? Expand with eye-popping numbers for: blockchain is appropriate and its typical issues are non-issues here; online comm. is low in overhead in both duration and energy and the ciphers work}
% % \sou{Highlights Online: Low overhead in SIB1 message implies adopting higher elliptic curves signature algorithms, 3.50 times lower signature verification time overhead implies 3.22 times lower energy consumption at the mobile user, cryptographic operation does not incur overhead in RRC connection time}
\end{abstract}

\begin{IEEEkeywords}
Cellular Network, 5G, Blockchain, Rogue Base Station, Base Station Authentication
\end{IEEEkeywords}



%\syc{Drafted/revised, but let's check again later}



==> Sections/Old_Tex_Files/07292024_Abstract.tex <==
\begin{abstract}
%\syc{Drafted/revised, but let's check again later}

% \syc{Construction->Delivery->Multi-pronged authentication}
\syc{R.:}
\sou{Regular – 100 to 200 words}

Malicious or rogue base stations are critical %and well-studied 
issues in telecommunication networking. %While there are digital security between the user and the backend core network, 
However, the current cellular practice in 5G remains vulnerable without a base station authentication mechanism or even keys to enable the authentication. %and there are no keys for base stations to enable the base station authentication. % when the user equipment communicates with the base station to establish the wireless channel and radio resource control. % and the R\&D community only recently proposed to introduce the base station's public key. 
We secure the base station authenticity and message integrity by designing and building a multi-factor authentication scheme of the base station. Our scheme introduces the base station digital certificate (including the base station's public key, the location information, and their certifications) to enable multi-factor authentication, which verification is through multiple orthogonal channels and defends against multiple threats from a fake base station. 
We advance beyond the state-of-the-art research by introducing greater authentication information factors (and analyzing their individual security properties and benefits) and by using blockchain 
%A key enabler in our scheme is the use of blockchain 
to deliver the base station digital certificate offline (enabling greater key length/security strength and computational efficiency). 
%
We take a systems approach to design the certification construction, delivery, and use on the verifier user equipment. The user equipment verification involves multiple factors which are verified through the ledger database, the location sensing (GPS in our implementation), and the cryptographic signature verification of the 5G broadcasting message of SIB1 using the base station's public key.
%\syc{Need to tie this to SIB1 Authentication}

We analyze and validate our scheme's %including the vulnerabilities/threats, 
security, performances, and the fit to the existing standardized networking protocols. 
Our work involves an implementation %SDR radios and relevant softwares to implement a prototype 
building on X.509 certificate, smart contract-based blockchain, and 5G New Radio-standardized RRC control communications. % and systematic analyses of the changes we made from the existing technologies. 
Our %proof-of-concept 
analyses and SDR-radio-based experiments show that our scheme defends against more threats and can enable stronger security (i.e., our scheme can use ECDSA with key lengths of 256, 384, 521, 571 bits in 5G RRC communication, while only ECDSA with 224-bit key have been supported by previous research). %which could not be supported by previous research). 
%We also show that our scheme design for 
Furthermore, our certificate's offline delivery via blockchain %and the authentication use 
enables the computing and energy to be more than 3.2 times efficient than the state-of-the-art research on the mobile user equipment. 

% To secure the base station authenticity and message integrity, we introduce and design the base station digital public-key certificate and analyze the security benefits informed by our base station vulnerability and threat analyses. 
% We build our scheme to construct, deliver, and use the base station certificate. 
% % We design, build, and deliver the base station digital certificate %(including both its construction and dissemination) 
% % and use it %the resulting delivered certificate information 
% % to secure the message authenticity of the communication-link control communication between the base station and the user equipment. 
% % While we study our scheme from the base station digital certificate construction to delivery to use for multi-pronged authentication, our research contributions beyond the existing research are more heavily in the base station digital certificate construction and delivery. 
% For the construction, we include the information fields which individually have security benefits, including the base station location information which has not been used in other certificate applications. %, and analyze how each of the information fields of ID, location, and public key enable the authenticity and integrity against various base station threats. 
% For the delivery, we use blockchain for delivering the base station certificate offline, which enables greater key length/security strength and computational efficiency than the state-of-the-art research delivering 
% the public key during the base station's online control communication. %, our scheme therefore enables greater key length/security strength and computational efficiency. 
% We then use the certificate to implement a multi-pronged authentication using the ID, location, and public key delivered by the certificate in the 5G control communication with the user equipment. 
% We take a systems approach to analyze and validate our scheme including the vulnerabilities/threats, security, performances, and fit to the existing standardized networking protocols. 
% %
% % While building on the related standardized technologies, % for most parts, %for practicality, %for both the digital-certificate-based key establishment and the digital-signature-based message authenticity protection. However, we 
% % we make novel contributions to advance the security.
% % We include the base station's location information in the certificate construction, use blockchain for the offline delivery of the certificate database, and incorporate multi-pronged authentication verification during the online real-time communications between the user equipment and base station. 
% % %We construct the base station certificate to include the base station's location information to defend against location spoofing and replay threats, which is novel compared to the existing certificates. Our scheme then delivers the base station digital certificate database including the registered base station records using blockchain building on its strengths of high integrity (only the core network can write on the blockchain and distribute the keys) and automatic and distributed synchronization and delivery. Both the certification construction and distribution occur offline before a user equipment (verifier) encounters the base station (prover). The base station public key authenticated by the digital certificate and the blockchain gets used in the communication-link control communication for setting the wireless communication channel including medium access control and radio recourse control. 
% % Because our work spans from certificate construction to delivery to the %certificate information use for 
% % multi-pronged authentication, we take a systems approach for our research to analyze and validate our scheme including the vulnerabilities/threats, security, performances, and fit to the existing standardized networking protocols. We analyze the rogue base station vulnerabilities/threats (including those based on new ID, spoofing, message injections, and replay/wormhole) and compare our work with the state-of-the-art research against those threats. 
% Our work involves an implementation %SDR radios and relevant softwares to implement a prototype 
% building on X.509 certificate, smart contract-based blockchain, and 5G New Radio-standardized RRC control communications. % and systematic analyses of the changes we made from the existing technologies. 
% Our %proof-of-concept 
% analyses and SDR-radio-based experiments show that our scheme defends against more threats and can enable stronger security (i.e., our scheme can use ECDSA with key lengths of 256, 384, 521, 571 bits in 5G RRC communication, while only ECDSA with 224-bit key have been supported by previous research). %which could not be supported by previous research). 
% We also show that our scheme design for the certificate's offline delivery and the authentication use enable the computing and energy to be more than 3.2 times efficient than the state-of-the-art research on the mobile user equipment. 

% We design and build a blockchain-based key distribution scheme and then use the key to authenticate the base station in 5G radio resource control (RRC) in which the base station transmits a digitally signed broadcast message. The blockchain delivers the base station's public key and builds on its strengths of high integrity (only the core network can write on the blockchain and distribute the keys) and automatic, distributed, and offline synchronization and delivery. %, advancing the start-of-the-art research which distributes the keys in the broadcasting and bandwidth-limited RRC chanenls at the time of the communications. 
% Our base station authentication uses the 5G RRC protocol's SIB1 message transmission (regularly broadcasted to the nearby mobile users) and enables the public-key authentication using the digital signature ciphers with greater security levels than the previous research (by offloading the base station's public key distribution in the offline blockchain). We implement and validate our scheme for both offline key distribution and online cellular communications. % (offline is before the telecommunication session and online is during). 
% Our implementations simulate the user, base station, and core network and involve radios and computers for both the online 5G communications (srsRAN and SDR) and offline key distribution (Ethereum smart contract with the third-party blockchain transmitter in both the local ad hoc and Internet-remote environments). %For such systems study and implementation, in addition to simulating the telecommunication entities (user, base station, and core network), we implement a third-party node to highlight the distributed delivery of the base station's public key (while only the core network can write, anybody can store and transmit the blockchain). %We use srsRAN and software-defined radio (SDR) for the online base station authentication and RRC communications between the user and the base station, and use Ethereum smart contract for the offline key delivery. % To highlight the automatic and robust blockchain-based key distribution, we also implement the offline key delivery (before the user becomes active for telecommunication networking) in both local and remote experiments and show how the blockchain is appropriate for base station's public key distribution. 
% Our experiments show that our scheme can support ECDSA with greater key lengths/security and that the mobile user's computing and energy consumptions are more efficient than the state-of-the-art research due to the blockchain-based offline key distribution. %because the offline key distribution enables the authentication using just one signature verification. 
% % \syc{What are the result highlights? Expand with eye-popping numbers for: blockchain is appropriate and its typical issues are non-issues here; online comm. is low in overhead in both duration and energy and the ciphers work}
% % \sou{Highlights Online: Low overhead in SIB1 message implies adopting higher elliptic curves signature algorithms, 3.50 times lower signature verification time overhead implies 3.22 times lower energy consumption at the mobile user, cryptographic operation does not incur overhead in RRC connection time}
\end{abstract}

% \IEEEkeywords{\syc{Please fix} Cellular Network, 5G, Blockchain, Rogue Base Station, Base Station Authentication}










%\syc{Drafted/revised, but let's check again later}



==> Sections/Old_Tex_Files/07312024_Experimentation.tex <==
% \section{Implementation and Experimental Results}
% \label{sec:implementation_results}
\vspace{-2px}
\section{Implementation and Experimental Setup}
\label{sec:experimental_setup}

%\syc{Add the simulated entities' hardware specs, and compare with the mobile phone specs out there}\sou{addressed in ~\ref{sec:experimental_setup}}

%In this section, we discuss our experimental setup where we incorporate our scheme and the state-of-the-art research implementation within RRC. We incorporate the blockchain interactions directly into srsRAN, where the certificate storage is maintained by a local Ethereum private blockchain via smart contracts~\cite{}.

Because we implement both the offline blockchain-based key delivery and its use in the online 5G RRC communications, our implementations include both local (direct communication link) and remote setups. 
We describe and explain our offline results and then the online results. 
For our experimental results, we present the average values and the 95\% confidence intervals. 



\begin{figure}[t!]
\centering
\includegraphics[width=0.4\textwidth]{Images/setup_edit_white.pdf}
\vspace{5px}
\caption{Experimental setup with the user equipment, base station, core network, and a 3rd party node. USRP B210 SDR is used for wireless 5G communications. The 3rd party node communicates the blockchain via Wi-Fi or Bluetooth.\vspace{-5px}} % \syc{Remove the outer square}}
\label{fig:experimental_setup_image}
\end{figure}



% \vspace{-2px}
% \subsection{Implementations and Experimental Setup} \label{sec:experimental_setup}
%\syc{Include "offline" vs "online" in this high-level, brief description to better guide the rest of the section organization. There should be a clear boundary between offline vs. online (which distinction we emphasized from the beginning of the paper), for example, one subsection for offline (including the Cloud/Google stuff) and another subsection for online.}

%We divide the testbed setup and the performance measurement of our scheme into two parts according to the design: offline phase and online phase. In offline phase, we diversify the channel to demonstrate that the mobile user can download or synchronize the blockchain ledger from a local node using ad hoc network (e.g Wi-Fi/Bluetooth) or from a remote server (cloud-based) using infrastructure network (e.g. WLAN). On the other hand, in online phase, the mobile user authenticates the broadcast system information message, i.e. authenticate the base station, using the public key (shared offline phase) prior to establish active radio connection with the base station. 

%In this section, we describe our implementations and the experimental setup.

%In this section, we describe our implementations and the experimental setup. %, performance measurement and performance analysis distinctly for both offline (local and remote) and online phases of our scheme. During performance measurement, we measure blockchain scalability with respect to block size, block propagation time, computational time for offline. For online performance analysis, we measure computational overhead for cryptographic operations and its implication on energy consumption and radio connection time at the mobile user .
%\syc{Suggested text to start: "Because we implement both the offline blockchain-based key distribution and its use in the online 5G RRC communications, our implementations include both local (direct communication link) and remote setup." Finish that paragraph or two. Then, divide the setup explanations using the following divisions and include the *motivations* and *rationales* about our experimental setup. For example, why are we using multiple channels for offline BBKD?}
%Due to the statistical nature of the network measurements, we include the 95\% confidence intervals for all measurements, although some may not be visible due to lower variance.

\subsection{Entities} %\noindent \textbf{Entities and Hardware:}
We simulate the different nodes involved in 5G RRC and blockchain in our scheme. These nodes are User Equipment, Base Station, Core Network, and 3rd Party Node as depicted in Figure~\ref{fig:experimental_setup_image}. The 3rd Party Node transmits the blockchain communication to the user equipment and represents anybody it communicates through offline, %\syc{3rd Party Node does not "simulate." We just name it to be anybody the 3rd Party Node, similarly to calling it Alice or Bob}, 
for example, ad hoc node or the previous base station. We describe the hardware simulating the entities in Appendix~\ref{apndx:hardware}. 
%\input{Sections/Hardware}
%(\souc{base station does not take part in the blockchain. So should it be a base station?} \syc{any node, including the previous base station, can participate}). 
%\syc{Move the hardware part to appendix}
%In choosing the hardware specifications for the different nodes, we prioritize the CPU specification. We refer to the hardware specification in Table~\ref{device_specs} with the CPU benchmark of our machines from~\cite{cpu_benchmark}. In our experimentation, we use the highest-rated CPU (AMD Ryzen Threadripper 3960x) as the core network and the second highest-rated CPU (AMD Ryzen 7 5700U) as the base station. We rationalize our choice of selecting the device for the mobile user so that it is representative of the real-world 5G smartphone computing capabilities~\cite{iphone_benchmark,android_benchmark}. For this practical reason, an Intel 12th Gen N95 mini PC is our choice for the mobile user. We also select the memory size of each device according to the CPU to maintain the balance. For wireless communication between base station and the mobile user, we use two USRP B210 software-defined radios. We transfer the blockchain ledger to mobile user locally from another node (we call it 3rd Party node) by the Wi-Fi and Bluetooth channels. We use the same experimental setup to compare the performance of our scheme with state-of-the-art practice and state-of-the-art research.

\subsection{Online (RRC)}
%\noindent \textbf{Online (RRC):} 
For the online implementation, we use srsRAN v22.10~\cite{srsran}, an open-source 4G/5G prototyping software to incorporate our scheme. We modify the RRC protocol to implement our scheme as shown in Figure \ref{fig:online}. We use OpenSSL v1.1.1 for the digital signature and x.509 certificates, whose cryptographic operations are incorporated in both the online RRC and offline blockchain. %to incorporate the cryptographic operations of our scheme (digital signature and certificate \syc{and certificate?}) into srsRAN. 
%We implement our scheme by modifying the RRC portion of srsRAN v22.10. %\sw{remove?:}We vary the signature algorithm between six ECDSA curves with varying key sizes to show the security levels.
% \syc{Mention about the statistical/random nature of the measurements. Explicitly state that the confidence intervals for all our measurements, although some may not be visible because they are small.}
%
%We also vary the UE and the base station locations (the radio locations) to study how the location and the channel qualities affect our scheme. 
%
%Apart from demonstrating our rationale for choosing hardware and software for our testbed, we also vary the channel between the mobile user and the base station to observe the radio connection behavior of our scheme. We choose different locations for base station and mobile user to vary the channel quality (SNR) as illustrated in Fig.~\ref{fig:building_layout_image}, where channel 1 is the best quality and channel 3 is the worst quality. \sw{Needs to have line of sight and non-line of site, and distance, $d$}

\subsection{Offline (Blockchain)} %\noindent \textbf{Offline (Blockchain):}  %\noindent \textbf{Offline (Local):} 
We use Go Ethereum v1.10.15 local private blockchain (i.e., independent of the Ethereum cryptocurrency Mainnet) and Solidity v08.1 smart contract for the blockchain implementations. 
We locally store the ledger using Redis 7.0.9 caching to make the real-time online operation more efficient, as Ethereum creates a new transaction for the ledger read, which is unnecessary for our scheme. 
%
We implement offline blockchain communications using diverse communication channels in both local ad hoc and remote infrastructure-based environments. 
We vary the communication protocols to demonstrate that blockchain delivers the key irrespective of the communication protocols, c.f., Bitcoin even gets delivered via unconventional satellite networking~\cite{blockstream}, 
so we vary the communication protocols to demonstrate the diverse and robust ways that the blockchain can deliver the base station's public key.
For the ad hoc local network, the 3rd party node and the user equipment connect to Wi-Fi or Bluetooth to distribute the blockchain ledger.  % is feasible to transfer from another node irrespective of local connectivity mode. We measure the time duration for certificate delivery and Round-Trip Time (RTT) to evaluate the performance of the offline part of our scheme in the local ad hoc network scenarios. 
For the remote Internet-infrastructure-based networking, the remote server (Google Cloud servers in domestic and international locations) connects to our user equipment via TCP/IP for the blockchain/key delivery. 
% \\
% \noindent \textbf{Offline (Remote):}
% For the offline remote scenario, we use a series of geographically distributed servers to distribute the ledger and measure the blockchain download/delivery time durations. We connect the local infrastructure network to access a set of Google Cloud servers distributed geographically and sorted by the round trip time. These include Iowa, Oregon, Virginia, London, and Singapore. We host the blockchain ledger on each node and measure the corresponding time durations to deliver the blockchain certificates to our local machine, visualized in Fig.~\ref{fig:blockchaintransfertime}.
% \sw{TODO: Include the fact that any communication channel can be made, even satellite communication with blockstream~\cite{}}
% %This experiment is significant to measure the performance of blockchain ledger synchronization while the mobile user is connected to the cellular network. We measure the same parameters as the previous offline experiment and compare the results. 


\subsection{Fake Base Station Threat Implementation}
\label{subsec:implementation_threat}
We experiment and analyze the security effectiveness of our scheme in the presence of an attacker described in section~\ref{subsec:threat_model}. %In this section, we demonstrate how our design scheme prevents possible malicious base station attacks that we consider in our threat model. 
We only consider the threats against broadcast messages of legitimate base stations. We perform the threats by implementing a legitimate base station, a malicious base station, and a user equipment. While the user equipment is under the coverage of a legitimate base station, we increase the distance between the user equipment and the legitimate base station to make the user equipment out of the coverage range. Then we make the malicious base station get closer to the user equipment so that it gets higher signal strength from the malicious base station. We collect the operation log files from srsRAN for the attack scenarios and measure the system response under attack. % The detail security 
%analyses are as below: %We describe the detailed security analysis of our scheme against malicious base station attacks in the below sections.



\section{Experimental Analyses}
\label{sec:experimental_analyses}

\begin{figure}
\centering
\includegraphics[width=1\columnwidth]{Figures/horizontal_bar_plot_byte_size_distribution_made224_white.pdf}
%\vspace{-5px}
    \caption{SIB1 packet size comparison between our scheme and SOTA with different signature algorithms. The vertical line shows the SIB1 size limit of 372 Bytes.\vspace{-13px}}
    \label{fig:sib1_packet_size_i}
\end{figure}

\subsection{Security Analyses of the Scheme} 
\label{subsec:security_analysis}
%\souc{I'll update this section after finalizing the threat model and attack analysis}\\
Without our scheme to authenticate the base station, we empirically validate that the fake base station can take over the 5G RRC, as long as it has enough power to make it greater than the other legitimate base stations to the user equipment. Our threat implementation is capable of doing so (i.e., controlling its transmission power, as described in Section~\ref{subsec:implementation_threat}); Figure~\ref{fig:fbs_attack} shows the fake base station taking over the user equipment's connectivity. \syc{Add a screen-capture to show the fake base station taking over the connectivity}\sou{Added}

However, with our scheme, we empirically verify the security effectiveness against the threats of New Base Station Threat, Base Station Spoofing Threat, Connection Injection Threat, as described in this section. This empirical validation includes our scheme disabling the wormhole threat. 


\subsubsection{Enables Greater Cryptographic Strength}
\label{subsubsec:greater_security}
Our scheme utilizing the offline delivery of the certificate and public key enables more efficient communications, i.e., fewer bits to transfer in the RRC SIB message. 
As shown in Figure~\ref{fig:sib1_packet_size_i}, our scheme can support all the ECDSA ciphers with varying key lengths and security strengths, while the SIB1 size limit of 372 Bytes (as described in Section~\ref{subsec:background_5G}) prohibits the use of ECDSA with greater keys beyond ECDSA-224 in SOTA. In addition to theoretically analyzing it based on our understanding of the RRC SIB1 protocol and ECDSA, we verified this %the use of the ECDSA ciphers being enabled 
in our prototype implementation.  %
While this section focuses on the increased cryptographic security strength against brute-force attackers, we also experimentally validate and analyze the reduced computation and energy use because of the communication data efficiency in Section~\ref{subsec:results_online}. 
\vspace{-2px}
\subsubsection{New Base Station Attack} We set up a malicious base station and broadcast its fabricated system information messages to lure the user equipment to get connected to it. Our scheme prevents such attacks by base station $ID$ verification. The user equipment authenticates the base station ID when it gets the base station certificate using the ID from the blockchain ledger because the ledger contains only the registered base station certificates.  %When the UE gets the base station certificate using the ID then the base station ID is authenticated because the base station certificate is included in the blockchain ledger with the ID (cell ID) which is validated by the core network of the operator. 

\subsubsection{Base Station Spoofing Attack} In the base station spoofing attack scenario, the malicious base station fails to prove the authenticity of its SIB1 messages. We test two cases for the malicious base station: (a) it takes a legitimate SIB1 message but includes a digital signature with its private key and (b) it captures a legitimate digital signature but fabricates the SIB1 message. In both cases, $SIB1$ authentication fails because a valid digital signature can only be generated from a legitimate SIB1 message with a legitimate base station public key. The public key in the base station certificate is sufficient to thwart the base station spoofing attack. However, we authenticate the base station using only the SIB1 message, if the attacker exploits vulnerabilities of other RRC messages then our scheme cannot provide complete defense against it as we mentioned in our comprehensive threat analyses (section~\ref{subsec:threat_analyses}).




\begin{figure}
\centering
% \begin{subfigure}{0.317\columnwidth}
%     \includegraphics[width=1\textwidth]{Figures/blockchainSize.eps}
%     \vspace{5px}
%     %\vspace{6px}
%     \caption{Blockchain and certificate size when varying the number of certificates per block. %\syc{Replace "minimal" to "Certificate"}
%     }
%     \label{fig:blockchainsize}
% \end{subfigure}
% % \hfill
% % \begin{subfigure}{0.42\columnwidth}
% %     \centering
% %     \includegraphics[width=1\textwidth]{Figures/blockchainTransferTime.pdf}
% %     \caption{Blockchain transfer time over local Wi-Fi network using TCP/IP when varying number of certificates.}
% %     \label{fig:blockchaintransfertime}
% % \end{subfigure}
% \hfill
% % \begin{subfigure}{0.3199\columnwidth}
% %     \centering
% %     \includegraphics[width=1\textwidth]{Figures/certgen_certdis_contractread_contractwrite.eps}
% %     \caption{Time duration for the offline operations including certificate generation and contract interaction}
% %     \label{fig:blockchaintransfertime}
% % \end{subfigure}
% %\hfill


\begin{subfigure}{0.459\columnwidth} %0.322
    \centering
    \includegraphics[width=1\textwidth]{Figures/cloudBlockchainTransferTime_1_Sim.pdf}
    %\vspace{-1px}
    \caption{Certificate delivery time.}
    \label{fig:certDeliveryTime}
\end{subfigure}
\quad
\begin{subfigure}{0.459\columnwidth} %0.322
    \centering
    \includegraphics[width=0.96\textwidth]{Figures/cloudBlockchainTransferTime_2_Sim.pdf}
    \vspace{0.7px}
    \caption{Transmission delay in RTT.}
    \label{fig:pingRoundTripTime}
\end{subfigure}
% \begin{subfigure}{0.48\columnwidth} %0.335
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/bbkdbscalability.pdf}
%     \vspace{28px}
%     \caption{Blockchain scalability in the certificate rate and the block arrival rate.}
%     \label{fig:bbkdbscalability}
% \end{subfigure}
%\quad
% \begin{subfigure}{0.47\columnwidth} %0.322
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/cloudBlockchainTransferTime.eps}
%     \vspace{-15px}
%     \caption{Blockchain propagation time-varying channels and the source/transmitter locations.}
%     \label{fig:blockchaintransfertime}
% \end{subfigure}
% \begin{subfigure}
%     \includegraphics[width=0.25\textwidth]{Figures/bbkdbscalabilitylinearr}
%     \caption{Blockchain Scalability (Linear Scale) (revised) \syc{Arijet: Let's keep this one. Comment out the others (so we can see them if needed). Increase the font sizes in general (we would make this plot much smaller than this in the paper). No need for legend. Change the vertical axes to "Certificate Rate" and "Block Arrival Rate (Bps)" and the horizontal axis to "Average Base Station Lifespan, \textit{y} (years)". Please make all these changes and update the plot.}\as{updated}}
% \label{fig:blochchain_scalability_linearr}
% \end{subfigure}
\caption{Offline blockchain-based certificate delivery performances when varying the certificate database source locations (Local vs. Cloud) and the communication protocols (Wi-Fi vs. Bluetooth). %\syc{Significance of these results?} 
\vspace{-13px}}
\label{fig:sizes}
\end{figure}





% then the UE cannot verify it because We use blockchain for base station certificates hence the attacker base station cannot forge its public keys into the blockchain. Again, if the fake base station  then the UE also invalidates the SIB1 message because the legitimate base station generates the digital signature using a legitimate SIB1 whereas the malicious base station sends a fabricated SIB1. The public key in the base station certificate is sufficient to thwart base station spoofing attack. However, we are only authenticating the base station using only SIB1 message, if the attacker exploits vulnerabilities of other system information messages our scheme cannot provide complete defense against it as we mentioned in our comprehensive threat analyses (section~\ref{subsec:threat_analyses}).





\subsubsection{Communication Injection Attack}
As illustrated in Figure~\ref{fig:attacK_wormhole} we implement the wormhole attack by capturing a legitimate SIB1 message with the corresponding digital signature at one location and broadcasting it in another location. Although the scheme would verify the message authenticity, the $L$ verification fails because the distance between the base station and the user equipment is greater than the distance threshold. In such a case, the user equipment invalidates the SIB1. The location information in the base station certificates and the distance threshold selected by the user equipment prevent such attacks. A wormhole attack is valid because the public warning message intended for one location can be sent to another location by the attacker and our scheme successfully prevents the attack.

% We can bypass the message authenticity and replay attack time threshold. To thwart this attack we use the location information of the base station in the base station certificate and the base station sends the threshold distance. The user invalidates the SIB1 message because the distance between the base station and the user is greater than the threshold defined in the SIB1 message. Although the user receives the SIB1 message from the malicious base station, but the remote legitimate base station generates the SIB1 message.  Such an attack is valid because the public warning message intended for one location can be sent to another location by the attacker and our scheme successfully prevents the attack.

Furthermore, the attacker can capture a legitimate SIB1 message with the corresponding digital signature and replay the message to the benign user equipment as illustrated in Figure~\ref{fig:attacK_replay}. In such a scenario our scheme applies $t$ verification. The user equipment invalidates the SIB1 message if the time difference between the SIB1 generation time by the base station and the SIB1 reception time by the user equipment is greater than the time threshold. However, if the attacker replays the message within the threshold then it eventually helps the legitimate base station to broadcast the message to the user equipment because the purpose of the SIB1 message is to help the user equipment determine the network access parameters. 
% For example, if the legitimate base station sends a public warning/alert message at any instance then it does not matter if the malicious base station also replays the message. However, it is a felony if the attacker base station stores the message and sends it to another time when the alert message is no longer valid.

\begin{figure}
\begin{subfigure}{0.44\columnwidth}
    \centering
    \includegraphics[width=1\textwidth]{Figures/Computations_UE_BS_Sim.pdf}
    %\vspace{2px}
    \caption{Time durations %performances %for the various components of our scheme 
    on the user equipment and base station.}
    \label{fig:online_performance_computation}
\end{subfigure}
\quad
\begin{subfigure}{0.43\columnwidth}
    \centering
    \includegraphics[width=1\textwidth]{Figures/Our_Scheme_Sign_verification_time_ALG_Sim.pdf}
    \vspace{1.2px}
    \caption{Signature verification times varying ECDSA.} % in our scheme.}
    \label{fig:sign_verification_algorithm}
\end{subfigure}
\quad
\caption{Our scheme's online performance.}
\label{fig:sizes}
\end{figure}

\vspace{-1px}
\subsection{Offline Results for Blockchain Key and Certificate Delivery}
\label{subsec:offline_results}
We implement the offline blockchain for the base station certificate delivery and run experiments to measure the blockchain size, blockchain scalability requirement (the number of certificates per second required to support the 5G applications), and the certificate delivery time. As described in Section~\ref{subsec:our_scheme_blockchain}, the core network generates the certificates (its write control is implemented in the smart contract), while the blockchain can be read and stored by other nodes including the user equipment. As discussed in Section~\ref{sec:experimental_setup}, we experiment in both local ad hoc and remote Internet-based environments and vary the communication protocols to highlight the blockchain's strength in automatic synchronization independent of the communication protocols (as discussed in Section~\ref{subsec:our_scheme_blockchain}). We also analyze the scalability requirement (which is a critical challenge identified in the general blockchain and cryptocurrency research) and compare it with other blockchain applications to establish the blockchain's appropriateness for our application in this section. 

%We measure the performance of offline part in terms of size, scalability and certificate delivery time. Additionally, we implement core network interaction to generate certificates and write it to the smart contract. We also derived the blockchain scalability from a single block size and rate of certificate generation request of a base station per year. We find our usage of blockchain in base station key distribution is more scalable than Bitcoin and Ethereum cryptocurrency.  

% \subsubsection{Blockchain Ledger Size}
% We show how the size of the blockchain ledger (stored in a distributed manner across the nodes) scales with respect to the number of certificates stored in the ledger in Fig.~\ref{fig:blockchainsize}. Per certificate, the blockchain adds additional overheads for the blockchain operations including the chaining and the integrity protection across the blocks. % When certificates stored in the blockchain, overhead is added with the certificates. 
% For one certificate with 132 Bytes, 34548 Bytes of overhead is added which is 99.62\% of ledger size (34680 Bytes). However, this blockchain overhead decreases as the number of certificates per block increases, as shown in Fig.~\ref{fig:blockchainsize}. %\syc{Let's discuss:} i.e. total size of certificates (in Bytes) increases. 
% For 100,000 certificates, the blockchain overhead size (beyond the certificate) is decreased by 8.933\% compared to 1 certificate. %as compared to 1 certificate. %this blockchain overhead decreases as number of certificates i.e. total size of certificates (in Bytes) increases. For 100,000 certificates, total the blockchain overhead size is decreased by 8.8697 percent as compared to 1 certificate.

\subsubsection{Blockchain Scalability}
%\noindent \textbf{Blockchain Scalability} \hspace{0.1in} 
In the blockchain use for base station certificate delivery, each new transaction or record gets updated when there is a change in the base station registration, including a new base station construction or a public-key revocation, which is far less frequent than the scalability requirements of other current blockchain implementations and practices such as those for financial transactions. 
\sour{Our scheme requires only 0.0266 certificate/transactions per second which is three orders of magnitude smaller than the other blockchain applications for cryptocurrency such as Ethereum and Bitcoin;} a more detailed analysis quantifying our scheme's scalability requirement is in Appendix~\ref{apndx:blockchain_scalability}.
%\syc{Move the rest of this subsection to appendix:}
%\sou{Mention blockchain scalability requirement and refer appendix}




%\sou{Moved from Appendix}

%\input{Sections/blockchain_scalability}


% the blockchain scalability capacity recommended by Ethereum smart contract, which is 20 transactions per second~\cite{ethereumtxpersecond} or $9.2 \times  10^5$ Bytes per second (using that the average transaction size is $4.6 \times  10^4$ Bytes per transaction~\cite{ethereumtransactionsize}). 
% %\syc{Simeon: Please fill in the following and cite the sources:} 
% By comparison, Bitcoin grows by $5.65 \times 10^{10}$ Bytes per year and Ethereum cryptocurrency grows by $2.31 \times 10^{11}$ Bytes per year~\cite{blockchain-charts}. 
% \syc{Arijet: Plot $1417 \cdot 3.1536 \cdot 10^7 \frac{4.189 \times 10^5}{y}$ for the transactions per second and $1417 \cdot 3.1536 \cdot 10^7 \frac{4.189 \times 10^5}{y}$ for the Bytes per second while varying $y$} \as{Will the equation be like this?: $ \frac{4.189 \times 10^5}{y \cdot 3.1536 \times 10^7}$ for the transactions per second and $ \frac{1417 \cdot 4.189 \times 10^5}{y \cdot 3.1536 \times 10^7}$ for the Bytes per second} \syc{Arijet: Please plot this and let's discuss.}\as{plotted}
% \syc{Plot it and fill in the blank:}
% % \syc{Not gonna work if we don't consider the rate:}
% % We can observe from the number of base station data (2000-2021) in US~\cite{basestationnumber} that the base station number growth rate ranges from -2.072\% to 22.30\%. We can derive an equation from Fig.~\ref{fig:blockchainsize} that blockchain\_size (bytes) = c1 $\times$ number\_of\_base\_station $+$ c2. c1 and c2 are the coefficients and c1 = 4043 (95\% confidence interval: 4038, 4047) and c2 = 6829 (95\% confidence interval: -1.890 $\times 10 ^{5}$, 1.754 $\times 10 ^{5}$). We can see that the blockchain size with the number of base stations in 2000 and 2021 in US becomes $\approx$ 0.4216 GB 1.694 GB. However, this blockchain size is for storing the public keys of all the base stations in US. Observing the base station number growth rate from previous years~\cite{basestationnumber} we can assume that the blockchain size  . For a single mobile operator, it is significantly less than this number (considering there are three major mobile operators with the capability of setting up base stations). 

%1693566970
%\sw{Fig 5c: compare to RTT/pingtime in text}
%\syc{2.63s for block-update for disseminating one base station's public key and ID; 62.3s for downloading a ledger with $10^5$ public keys/IDs. Refer back to Section~\ref{subsec:background_5G} to derive the 420k/4 which is approximately 100k.} 
%\syc{Simeon: Give that block propagation delays for Bitcoin. Give us the number for the average peer connections including the inbound connections, and cite our paper which has more details.} % 
%\sw{Bitcoin average peer connections, the block propagation time of 23.28 seconds (cite our paper). Explain 32 peers (cite our paper, and/or Wenjun paper)}
%\syc{Simeon: Create a blockchain which has 420,000}
%\syc{Update the Storage Size (B) vs. Number of Certificates with greater information. At least, please include the certificate size (B).}


\begin{figure}
% \begin{subfigure}{0.275\columnwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/RRC_OS_STAP.pdf}
%     \vspace{3px}
%     \caption{RRC connection setup time duration}
%     \label{fig:online_performance_rrc_connection}
% \end{subfigure}
%\hfill
\begin{subfigure}{0.421\columnwidth}
    \centering
    \includegraphics[width=1\textwidth]{Figures/three_verify_comparison_Sim.pdf}
    %\vspace{0.1px}
    %\vspace{12.7px}
    \caption{Signature verification time durations at user equipment.} % for the cipher operations only.}
    \label{fig:sign_verification_comparison}
\end{subfigure}
\quad
%\vspace{-9px}
\begin{subfigure}{0.524\columnwidth}
    \centering
    \includegraphics[width=1\textwidth]{Figures/PWR_Energy_Updated_Sim.pdf}
    \vspace{6px}
    \caption{Power (measured) and energy (calculated) consumption at the user equipment.}
    \label{fig:energy}
\end{subfigure}


\caption{Our scheme vs. SOTA comparison.\vspace{-10px}} % performance of RRC handshake components}.%\sw{mis-captioned, it's online RRC}\syc{1) Why is this here? 2) Have the Wi-Fi and the setup in the experimental setup paragraph. Please be brief and have all the setup in one place (not within the subsections). I understand that we experimented with just one setting.}}
\label{fig:sizes}
\end{figure}

\subsubsection{Offline Time Overhead Performance}
We use diverse communication channels (Wi-Fi/BT) and sources (local/cloud) to demonstrate the robustness of blockchain-based certificate delivery to the user equipment. Figure~\ref{fig:certDeliveryTime} shows our experimental results for certificate delivery (34680 Bytes) from 3rd node and cloud server using ad hoc and infrastructure networks. The ad hoc network connectivity using Wi-Fi provides the fastest certificate delivery (32.22 ms) from the 3rd party node as compared to other locations and connectivity. The certificate transfer using ad hoc Bluetooth takes the longest time (1070.2 ms) which is natural due to the physical-layer design of Bluetooth providing low data rate/bandwidth. We also measure the certificate delivery from the remote cloud servers, connected to the user via the Internet (TCP/IP) and through the 3rd Party Node as the last networking hop via Wi-Fi. As shown in Figure~\ref{fig:pingRoundTripTime}, the RTT time duration increases as the remote node to initiate the blockchain transmission is located geographically farther. %It has direct correlation with the RTT time duration, as the RTT time increases the certificate delivery time increases. 
The cloud server in Iowa provides the lowest certificate delivery time (52.23 ms) and the cloud server in Singapore takes the highest time (1060.05 ms or 1.06 seconds) to deliver the certificate. 
While these measurements can be high and can reach up to about 1 second, the offline cost in the time overhead is significantly cheaper than the real-time online cost in Section~\ref{subsec:results_online}. 








%\subsection{Online Analysis for RRC Handshake} 
\vspace{-1px}
\subsection{Online Results for multi-factor Authentication} 
\label{subsec:results_online}

We compare our scheme against the SOTA described in Section~\ref{subsec:sta_r} in the computational time, energy consumption, and the RRC connection setup overheads. We also vary the user equipment locations for radio experiments and measure the signal-to-noise ratio (SNR) and its impact on the RRC connection overheads in Appendix~\ref{apndx:radio_experiments}.

\subsubsection{Our Scheme's Online Performances}
We take a systems approach to measure the performances across the online operations of our scheme. 
In Figure~\ref{fig:online_performance_computation}, we show that $ID, L, t$ verification time (0.0776) and signature verification time (4.744 ms) at the user equipment are much lower than the RRC connection establishment time duration between the user equipment and the base station (251.6 ms). The user equipment computing is only 1.89\% compared to the entire RRC networking between the user equipment and base station. Also, we add only a total of $72$ bytes of overhead in the SIB1 message using the ECDSA-224 algorithm (signature - 64B, nonce - 4B, and timestamp - 4B).

%\sou{I think we can also shift this paragraph to the appendix because it may seem obvious that digital signature verification with higher key length would require more time. Also, we argue that our scheme enables higher security, but, I think Figure 9 captured that. With this figure, we show that we also implemented that.}
Our scheme enables the use of the ECDSA ciphers with greater keys and security strengths, while the use of the ECDSA with greater keys is prohibited in SOTA as described in Section~\ref{subsubsec:greater_security}. We experimentally verify this and measure the time overheads when varying the ECDSA key lengths in Figure~\ref{fig:sign_verification_algorithm} to show that the time overheads increase as the key lengths increase. In terms of SIB1 byte length overhead with greater ECDSA key length, only the signature size contributes to SIB1 which is below the maximum SIB1 size (376 bytes).
%In terms of SIB1 byte length overhead, only the signature size contributes to the ECDSA cipher with the greater key length which is under the maximum SIB1 size (376 bytes).

\subsubsection{Our Scheme vs. SOTA}
\label{subsubsec:os_vs_sota}
We focus on our scheme implementation using ECDSA-224 when comparing our scheme vs. SOTA because SOTA does not support the other ECDSA digital signature algorithms \sour{as discussed in Section~\ref{subsubsec:greater_security}}. % except for Fig.~\ref{fig:sign_verification_algorithm} comparing the performances across the digital signature algorithms with different key lengths and security strengths.
Figure~\ref{fig:sign_verification_comparison} compares the computing overhead of the signature verification for our scheme vs. the SOTA. %, described in Section~\ref{subsec:sta_r}. 
Because the SOTA requires three signature verification on the user equipment \sour{due to certificate chaining} while our scheme only requires one, the signature verification overhead of the SOTA (19.91 ms) is 3.50 times greater than our scheme (5.68 ms). Our scheme's signature verification after incorporating it within srsRAN (5.68ms) is close to the digital signature verification without the srsRAN incorporation (5.67ms). 

The signature verification efficiency of our scheme compared to the SOTA results in the energy efficiency of our scheme, which is important for battery-equipped and energy-constrained user equipment. We take the power measurements in our experiment and then calculate the energy consumption by multiplying the average power consumption and the average time duration for the signature verification. 
As seen in Figure~\ref{fig:energy}, the SOTA takes 3.22 times more energy (531.38 milliwatt-hour versus 165.21 milliwatt-hour) than our scheme to verify the signatures, because our scheme verifies the digital signature once while the SOTA verifies three digital signatures to complete the authentication. 

 %As the key lengths increase, the cryptographic security strength against the brute-force attacker also increases, as it takes greater time for the attacker to find the private key; this attacker's time to break the scheme is currently infeasibly large assuring the security of the public key digital signature in our nowadays digital security applications. 
%\syc{I like how you compare the magnitudes here, but let's include that in the journal version.}
%\sou{Moved from Appendix}
%\input{Sections/Wireless Experiments}

%%%%%%%%%% Moved to Appendix B %%%%%%%%%%%%%
% \subsubsection{Our Scheme Varying Wireless Channels}
% We vary the wireless channel conditions between the mobile user and the base station, as shown in Fig.~\ref{fig:building_layout_image}. Channel 1 has the shortest distance of $d=5$ meters, while Channels 2 and 3 have the same distance of $d=15$ meters. Channel 2 however has a line-of-sight (LOS) channel while Channel 3 has physical barriers in walls between the mobile user and the base station (non-line-of-sight or NLOS). 

% Because shorter distance (smaller $d$) and LOS channel provide better wireless channels, Channel 1's signal-to-noise ratio (SNR) performance is better than Channel 2's, and Channel 2's is better than Channel 3's (14.2 dB vs. 9.35 dB vs. 7.11 dB). The channel conditions also affect the RRC connection setup time and the better the channel quality the lower the connection time duration. Channel 1 takes 251.58 ms for the RRC connection setup, while Channel 2 takes 300.90 ms and Channel 3 takes 304.11 ms. 







%\syc{In the future draft (and not this submission), include why we don't include Our Scheme vs. STA Practice vs. STA Research}



% In this subsection, we demonstrate the security and performance analysis of the online base station authentication phase of our scheme. We focus on illustrating the performance of our scheme as compared to state-of-the-art research in terms of computational time, energy consumption, and RRC connection setup time. 


% %\syc{Plot 1: The size (B) plot. Plot 2: The time plot (ms), showing "Key Read (User)" "Signature Verification (User)", "Signature Generation (Base Station)", and then "RRC Handshake (Protocol)". When explaining Plot 2, including the comparison between our scheme vs. STAR for signature verification; when doing the comparison, include both the actual measurement in ms and the ratio difference which is about 2x.} 

% This experiment leverages the blockchain-based key distribution by adapting a higher security level signature algorithm than the state-of-the-art research. The physical layer limitation on SIB1 packet size has a direct impact on the choice of our signature algorithm. We show the lower bound (implemented using OpenSSL) values of total SIB1 packet size with different signature algorithm in Fig.~\ref{fig:sib1_packet_size_i} for our scheme and state-of-the-art research. The implemented values of public keys and signature sizes are higher than the theoretical values due to data encoding before sending it to the network. In our scheme, we transmit only SIB1 signature in SIB1 message while distributing the base station public key during the offline phase. In contrast, the state-of-the-art research requires sending four additional data fields (core network signature, MME/AMF public key, MME/AMF signature, base station public key) which restrict their scheme to use higher level of ECDSA algorithms. We experiment with our scheme with up to ECDSA-571 whereas in state-of-the-art research it can be used only up to ECDSA-224. Fig.~\ref{fig:sign_verification_algorithm} shows the signature verification time using different Elliptic Curve Digital Signature Algorithms (ECDSA) that we adopted in our scheme. We see the signature verification time increases as we use higher public key size and ECDSA-571 gives higher security at the cost of 1.92 times more signature verification time than ECDSA-224. However, as the state-of-the-art research can support only ECDSA-224, therefore, we use the same security level algorithm for the performance analysis and comparison in the following parts of this subsection. 
% \\
% With respect to computational overhead, we measure the time duration for each additional computation that we introduce in the standard 5G RRC layer protocol. We focus on the performance of the mobile user since cryptographic operation involves higher CPU usage with associated power consumption and processing time. In Fig~\ref{fig:online_performance_time} we show that key reading time (0.04 ms) and signature verification time (5.67 ms) at the mobile user are much lower in our scheme so that it has minimal impact on RRC connection establishment time (245.66 ms). For the base station, we can consider it can generate SIB1 signature prior to broadcast each round of the system information message, hence, we can exclude base station signature generation time from our performance analysis of the system.
% \\
% While evaluating the performance of our scheme, we get it requires around 3.50 times lower signature verification time than state-of-the-art research which is expected. As shown in Fig.~\ref{fig:sign_verification_comparison}, state-of-the art research needs to verify three signatures that takes total 19.91 ms (average), whereas in our scheme it requires only 5.68 ms (average). We also measured the average signature verification time 5.67 ms of the same SIB1 message without implementing it in srsRAN (here, we say cipher only) to compare the signature verification time with srsRAN integration. We get our scheme has almost same signature verification time as cipher only verification time and state-of-the-art research requires almost 3 times of cipher only verification time. The additional signature verification time has greater impact on energy consumption of the mobile device battery. We calculate the energy consumption by taking power consumption and time duration measurement for signature verification of our scheme and state-of-the-art research. We find state-of-the-art research takes 3.22 times more energy (531.38 miliwatt-hour versus 165.21 miliwatt-hour) than our scheme to verify the signatures (refer to Fig.~\ref{fig:energy}) which is expected because it verifies 3 signatures to complete the authentication. The measured power is almost similar because the rate at which energy is consumed for each signature verification is same. Although we use a mini PC to calculate the power, however, the same ratio must hold for mobile devices as well.
% \\
% To observe the impact of cryptographic computation overhead at the mobile user on the RRC connection setup, we perform our experimentation by varying the channel quality between the mobile user and the base station. Fig~\ref{fig:SNR_vary_location} shows the channel quality in terms of Signal to Noise Ratio (SNR) for three different channels. We find that the RRC connection setup time (shown in Fig~\ref{fig:RRC_time_vary_location}) relies on channel quality and the cryptographic operation has minimal impact on it. As the base station periodically broadcast the system information messages, the mobile waits for the base station to broadcast the rest SIBs after reception and processing of SIB1 whereas the mobile user remains idle in this period. Therefore, any computation that occurs at the mobile user between the reception of SIB1 and the rest of SIBs has no impact on the RRC connection time.

==> Sections/Old_Tex_Files/07312024_Old_Our_Scheme.tex <==
\section{Our scheme}
\label{sec:our_scheme}
We design a base station authentication scheme that consists of two phases: offline key generation and distribution and online base station authentication. In offline key generation and distribution phase, the core network \syc{generate? let's discusss}, validate and sign the public key of base stations and publish the digital certificate into the blockchain ledger \syc{do we use the term "ledger"?}. A mobile user that wants to connect to the network will ensure availability of the blockchain ledger into its local storage before initiating radio connection with the base station. This phase is offline because base station's public key can be make available to the mobile user's local storage in beforehand of radio connection initiation to the network (similar to USIM installation in mobile device). During online base station authentication phase, the mobile user verifies the SIB1 message using the public key of the base station that it gets from the offline phase. Blockchain based PKI plays an important role in our scheme for secure and reliable distribution of base stations public keys to the mobile users. 

\subsection{Existing 5G Protocol}

%\syc{Start with why this subsection is so important for our work, e.g., compatibility. Refer to Fig.~\ref{fig:online}}\sou{Main focus of this paragraph is explaining the insights of Fig.~\ref{fig:online}. -Base station transmits SI messages periodically -Mobile user wait until next broadcast schedule to get SIBs.}\\
In this work, we introduce base station broadcast message authentication by the mobile user in Radio Resource Control (RRC) layer of the standard 5G cellular network protocol defined by 3GPP. In Fig.~\ref{fig:online} we show the standard 5G control communication protocol messages in blue font color. \sou{Size limitation of SI messages: Physical layer TBS calculation} At first, the mobile user uses information received from Physical Downlink Shared Channel (PDSCH) signalling and Downlink Control Information (DCI) to determine the transport block size (tbs) that determines the amount of information received by upper layer. The transport block size depends on modulation order, target code rate, redundancy version, number of resource block that is available at the mobile user using DCI signalling. We illustrate this process as frame synchronization that takes place at the very first communication from base station to mobile user. It is important to note that according to 3GPP standard \cite{3gppphy}, the amount of information the mobile user expected to receive in system information message is determined by the transport block size (tbs) which is 2976 bits (372 bytes). 

In 5G-NR RRC layer, the base station transmits system information messages with different periodicity: MIB broadcast message with a periodicity of 80 ms, SIB1 with a periodicity of 160 ms and other SIBs with a periodicity scheduled in SIB1 (20 ms by default) \cite{3gpprrc}. It is minimum for the mobile user to acquire MIB and SIB1 since they contain essential radio connection related information and the mobile user has to wait to get system information message until its next broadcast schedule.

Therefore, the mobile user can only initiate RRC connection request once it gets all necessary information from system information messages and later on complete the RRC connection setup using a three way handshake. After successful RRC layer connection with the base station, the mobile user proceed to setup NAS layer connection with the core network. We omit the control communication between base station and the core network in this work as it is out of the scope of our research. 

%  Prior to setup RRC connection with base station, the mobile user periodically receives a number of broadcast messages to get necessary information about the network. Master Information Block (MIB) and System Information Block Type1 (SIB1) are called Minimum SI since they are essential for the mobile user to get initial radio connection related information. The base station transmits MIB with 80ms and SIB1 with 160ms periodicity. The periodicity of other system information messages are scheduled in SIB1.

\subsection{Key components of our scheme}
In this section, we describe the key components of our scheme as illustrated in Fig.~\ref{fig:key_components}. We design our scheme to thwart attack scenarios described in section~\ref{subsec:attack_scenario} by introducing security parameters (identity, public key, location information, nonce, timestamp, and distance) that are being sent from the network to the user using \emph{offline} and \emph{online} phases. Table~\ref{tab:x_509 fields} shows the necessary fields of the base station certificate. The network constructs the base station certificates that include the base station's identity ($ID$), public key ($K$), and location information ($L$). Upon construction, the blockchain distributes the base station certificates from the network to the user using the offline phase after being signed by the core network. We distribute these security parameters in the offline phase because they are static for a certain period of time (validity period) and the user does not need to verify these parameters during authentication (as opposed to the recent research). The network sends some additional security parameters such as a nonce ($n$), timestamp ($t$), and distance ($d$) in the online phase because these parameters are dynamic. The user utilizes the security parameters that it receives during the online and offline phases to authenticate the base station. The user uses the $ID$ to identify the certificate of a particular base station. It uses the public key ($K$) to authenticate the base station and the location information ($L$) along with the distance ($d$) to prevent location spoofing attacks. Furthermore, the user is able to detect replay/relay attacks using the timestamp ($t$). Also, the nonce value ($n$) ensures the freshness of the digital signatures. In our scheme, the base station certificate plays a pivotal role in disseminating crucial security parameters that help the user to discriminate the legitimate base station from a malicious one.


\subsection{Blockchain For Distributing the Base Station Credentials}
\label{subsec:our_scheme_blockchain}
%- Describe how blockchain play an important role here.
%\syc{Blockchain subsection drafted. I plan to revise.}

Blockchain enables the secure and offline distribution of the base stations' public keys. Blockchain is appropriate for such distribution because, unlike the mobile users, the base stations are public entities and publicly advertise their presence via broadcasting SIB1. The blockchain provides the public ledger including the ID (the cell ID as described in Section~\ref{subsec:background_5G}) and the public key of the legitimately registered and deployed base stations. 
%\syc{What is the ID we use?} \sou{cell id of the base station}

The blockchain ledger includes the digital certificates which are signed by the core network and whose subjects are the base stations (as well as the core network itself in the genesis block). % (validating and linking the base station's ID and its public key). 
The ledger validates and links the ID and the public key of the core network (self-signed in the genesis block) and the base stations (signed and vouched by the core network). The core network uploads its own public key and certificate before it digitally signs and generates certificates for base stations, and the genesis block includes the core network's initial public-key information. % the private key corresponding to the public key in that certificate is used for digitally signing the other certificates for the Base Stations. 
Because the core network signs and generates the digital certificates (after the base station generates the key pair and sends the public key to the core network), the core network uploads the digital certificates to the blockchain. The digital certificates in the blockchain ledger are verified, stored, and shared with all the entities involved in 5G networking, including the mobile users. 

We use blockchain for the distribution of the base stations' public keys because of the following enabling blockchain properties. Blockchain provides \emph{message authentication integrity} by using the cryptographic primitives of public-key digital signature and the hash function. These cryptographic primitives are robust in security (the computational hardness assumptions) and anchor the modern day digital information and networking security. Blockchain provides easy access to its ledger information and builds on \emph{distributed storage and broadcasting} so that all the nodes store the blockchain ledger (including the base stations' digital certificates). The distributed storage and broadcasting enables that the ledger gets \emph{automatically synchronized} in various channels (e.g., ad hoc connections or from previous base station connections) during the offline times, enabling easier access to the digital certificate information before the online phase using the cellular connectivity services. %For example, a nearby mobile or sensor user can deliver the newest block (containing the new public key of a base station) for the ledger synchronization in ad hoc/peer-to-peer networking. 

Our use of the blockchain is substantially simpler and cheaper than that used in permissionless cryptocurrencies. 
Because the service provider infrastructure (core network and base stations) are public entities and do not require anonymity or privacy and because the public keys can be public/known for the security of the public-key digital signature, we use a permissioned and public blockchain where the 
blockchain ledger gets written only by the core network while it can be read/stored/accessed by all the entities in the cellular networking. Therefore, our blockchain forgoes the heavy distributed consensus protocol, e.g., computation-heavy proof-of-work (PoW), to determine which data gets uploaded and by who. Also, in contrast to the cryptocurrency blockchain, we do not have the incentivization or competition issues because the service provider infrastructure and its beneficiaries/clients are all aligned in their incentives to provide connectivity and secure cellular connections against the rogue base stations. 




\subsection{Offline Key Generation and Distribution}

Fig.\ref{fig:offline} illustrates the design diagram of the offline key generation and distribution phase of our scheme. During the installation of new base station or when the current digital certificate expired, the base station generates its own private/public key pair ($K, k$) for each cell. Then the base station sends certificate signing request to the core network with an ID ($cell\_id$ in this case). Hence, the base station creates separate certificate signing request for each of its cell and send it to the core network for signing them. Upon receiving the signing request, the core network validates and sign  the certificate of each cell of the base station and write the signed digital certificate into the blockchain ledger. The core network has the only write permission into the blockchain ledger. A mobile user that wants to connect to a network need to synchronize base station digital certificates of that network from blockchain ledger into its local storage. Initially, mobile user can download it from the internet using wifi, or collect it from another mobile user for the first time before initiating radio connection to the base station. Later on, the mobile user can synchronize the ledger periodically once its connected to the network.

Base station relies on the core network to validate its public key because we assume core network resides in a secure confinement of the service provider and attacker will not have access into the core network to forge the digital certificate of the base stations or upload malicious certificates into the blockchain ledger. Blockchain based PKI framework is significantly important here to distribute the public keys of base stations to mobile user using a minimal version of X.509 digital certificate. 

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Images/online}
    \caption{Online base station authentication by mobile user. The blue color indicates those already in 5G RRC. \syc{Fig moved because the Existing 5G subsection makes use of the figure}}
    \label{fig:online}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.28]{Images/Offline}
    \caption{Offline key generation and distribution using blockchain (right)}
    \label{fig:offline}
\end{figure}

% \begin{figure}
% \begin{subfigure}{0.38\columnwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/algsHandshakeSize.pdf}
%     \caption{Handshake size when varying the algorithms \syc{Is that the confidence interval I see? Why is this measurement random? The handshake size being random is not necessarily a bad thing (it can possibly be interesting, although it's probably trivial), but it would need to be explained.}}
%     \label{fig:handshakesize}
% \end{subfigure}
% \hfill
% \caption{!!!}
% \label{fig:sizes}
% \end{figure}

\subsection{Online Base Station Authentication}
%- Describe the authentication process. \\
%- Include design diagram here.
During Online base station authentication phase, the real time cell specific authentication of SIB1 messages happens which is illustrated in Fig. \ref{fig:online}. Our contributions over existing communication between mobile user and base station are shown in black font color in the diagram. Before broadcasting \emph{SIB1} message the base station generates a digital signature $S_k$(\emph{SIB1},$n$) on \emph{SIB1} and a nonce ($n$) using its private key ($k$).% \syc{"private key" as opposed to "private-key". Please fix throughout the paper.} \sou{fixed}
The nonce ($n$) is an arbitrary value we use for replay attack protection during each \emph{SIB1} message broadcast. Finally, the base station appends the digital signature along with the nonce to the \emph{SIB1} message and broadcast it. The final \emph{SIB1} message is: {\emph{SIB1},$n$,$S_k$(\emph{SIB1},$n$)}.

The mobile user ensures the availability of blockchain ledger into its local storage prior to network signal scanning. When the mobile user receives the \emph{SIB1}, it then, look up the public key ($K$) of the base station from the blockchain ledger in its local storage (that got from offline phase) using the \emph{ID} ($cell\_id$) received in \emph{SIB1}. It verifies the digital signature $V_K$($S_k$(\emph{SIB1},$n$)) using $K$. After successful verification of the digital signature, the mobile user proceeds to establish RRC connection with base station and NAS layer connection with core network upon successful RRC establishment.

In our scheme, regarding transmitted data byte overhead we add two additional data fields in the SIB1: the digital signature and the nonce. With respect to computations, we add, digital signature generation at base station and public key reading from blockchain ledger as well as digital signature verification at mobile user. We measure performance of our scheme as compared to State-of-the-Art research under the premise of these data size and computation overhead.


==> Sections/Old_Tex_Files/07312024_our_scheme.tex <==
% \begin{figure}[t!]
%     \centering
% \includegraphics[width=0.9\columnwidth]{Images/High_Level_Arrow_Diagram.pdf}
%     \caption{Overview of our scheme. %\sou{Simeon please change "distribution" with "delivery"}
%     }
%     \label{fig:arrow_diagram}
% \end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.75\columnwidth]{Images/Diagram_Key_Components_Sim.pdf}
    \caption{Information delivered during offline (dashed-dotted) vs. online (solid) for our scheme. The certificate database $\mathcal{C}$ including the base station public key, $k$, and its static location $l$ is shared offline, while online involves $ID,n,t$ communication.} %The base station certificate contains the identifier ($ID$), public key ($K$), and location information ($L$).%\sw{Dotted-dashed line, no color}\sou{Simeon please change "distribution" with "delivery" and "Usage" with "multi-factor Authentication"}
    \label{fig:key_components}
\end{figure}

%\vspace{-2px}

\section{Our scheme}
\label{sec:our_scheme}
%\souc{key components of base station certificate: construction, distribution, usage and two phases: offline and online}
We design our scheme from the base station digital certificate construction to delivery to its use for multi-factor authentication, as illustrated in Figure~\ref{fig:arrow_diagram}. In our scheme, the construction is offline; the delivery is offline (while the current SOTA research is online as described in Section~\ref{subsec:sta_r}); and the certificate use for multi-factor authentication is online. 

\subsection{Our Scheme Overview in Offline and Online}

We design a base station authentication scheme that consists of two phases: offline (base station certificate construction and delivery) and online (multi-factor base station authentication by using the delivered certificate). \sour{Figure~\ref{fig:key_components} shows the entities involved along with delivered information in each phase}. In the offline certificate construction and delivery phase, the core network validates and signs the public key of base stations and publishes the \sour{base station digital certificate} via the blockchain ledger. The core network binds both of the base station's cell ID ($ID$) and the geographical location ($L$) with the key ($K$) when digitally signing for the base station certificate. A user equipment that wants to connect to the network receives the base station certificates on the blockchain offline before initiating a radio connection with the base station. The offline blockchain communication includes the base station's certificate (including information fields listed in Figure ~\ref{fig:cert_contents}) and can get delivered any time before the radio connection with that base station, e.g., in any of the previous communications by the mobile user. %This phase is offline because base station's public key can be make available to the mobile user's local storage in beforehand of radio connection initiation to the network (similar to USIM installation in mobile device). 
%\syc{Revise and reflec the multi-factor approach} 
During the online multi-factor authentication phase, the base station digitally signs \sour{the first radio control communication message i.e. SIB1}, and the user equipment receives and verifies the SIB1 message using the ID, location, and public key of the base station that it gets from the offline blockchain. %Blockchain based PKI plays an important role in our scheme for secure and reliable delivery of base stations public keys to the mobile users.
The security of our scheme relies on the security of the cryptographic primitives.

%\syc{Recap offline vs. online information delivery. List them here, and state that the rest of the section describes and explains them in greater details.} 
In offline, we deliver the digital certificate database of the base stations $\mathcal{C} = \{C_i\}_i$, where each record $C_i = \{ID_i, K_i, L_i, ... \}$ is for the registered base station index $i$ and $i$ iterates across the base stations for each row. For example, the first record/row corresponds to the first registered base station $i=1$, i.e., $C_1 = \{ID_1, K_1, L_1, ... \}$. Each certificate $C_i$ can include other fields as indicated (we implement a concrete certificate based on X.509 which fields are shown in Figure~\ref{fig:cert_contents}), but $ID_i, K_i, L_i$ are the most relevant to our scheme. %\sou{need to discuss with the notation here $\{C_i\}_i$}
In online, we deliver cell ID ($ID_i$), nonce ($n$), and SIB1 generation timestamp ($t$) appended into the SIB1 message of the base station $i$. Figure~\ref{fig:key_components} illustrates the parameter deliveries between the base station and the user equipment during offline and online. % these key parameters and their delivery method from the base station to the user equipment. 
This information gets used for authenticating the base station $i$, which yields the Boolean $A$, where $A=1$ means that the base station $i$ has been authenticated (true) vs. $A=0$ not authenticated (false). 
We describe and explain these information deliveries in greater detail in the rest of the sections. 





\begin{figure}
    \centering
\includegraphics[width=\columnwidth]{Images/x.509_Contents.pdf}
    \caption{Our base station certificate information fields with the new additions are highlighted in blue. This corresponds to the individual record of a registered base station in the base station certificate database $\mathcal{C}$. %\souc{Please add BS public key}\sw{Updated with accurate information}
    %\syc{Blue-color "Cell ID" and "Location"} 
    \vspace{-5px}
    } %\syc{Fig moved because the Existing 5G subsection makes use of the figure}}
    \label{fig:cert_contents}
\end{figure}


% \begin{table}[t]
% %\small
% \tiny
% \centering
% \vspace{10 px}
% \caption{\souc{Newly added: Need simeon's help to get size}A Base Station certificate with total size 138 bytes\sw{Consider displaying similarly to Fig. 3 but for x.509} \syc{Let's just use Fig. 3 if this is only adding the B information}}
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular} { |c| c | c |}
% \hline 
% \textbf{Field Name}  & \textbf{Description} & \textbf{Size (B)} \\
% \hline
% version & Version of the certificate & 1 \\
% \hline
% serialNumber & Serial number of the certificate & 1\\
% \hline
% issuerName & Operator name & 2\\
% \hline
% \textbf{subjectUniqueID} & \textbf{Cell ID of the Base Station ($ID$)} & 4\\
% \hline
% \textbf{subjectPublicKey} & \textbf{Base Station public key ($K$)} & 56\\
% \hline
% validityPeriod & Default value (1 year) & 1\\
% \hline
% \textbf{Location} & \textbf{Location info. of the Base Station ($L$)} & 8\\
% \hline
% %\textbf{Longitude} & \textbf{Longitude of the Base Station} & 4\\
% %\hline
% digitalSignature & Signature of the issuer & 64\\
% \hline
% algorithm & Algorithm used to sign the certificate & 1\\
% \hline 
% \end{tabular}
% \label{tab:x_509 fields}
% %\vspace{-10mm}
% \end{table} 


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Images/Offline_Sim_2.pdf}
    \caption{Offline certificate construction and delivery. The certificate construction involves the base station and core network (the inner middle entities), while the delivery further involves the user equipment (left) and blockchain (right).\vspace{-10px}}
    \label{fig:offline}
\end{figure}


\subsection{Base Station Certificate Construction (Offline)}
\label{subsec:our_scheme_cert_construct}

Our base station certificate construction builds on the X.509 standardized certificate, which is popularly used for securing the Internet and web, e.g., transport layer security (TLS) and hypertext transfer protocol secure (HTTPS). However, we adapt its construction specifically for base station and to enable greater security objectives. 
Figure~\ref{fig:cert_contents} illustrates the data fields within our base station certificate where our additions beyond X.509 are highlighted in blue. One change we make is the change of formats in the ID from the IP address for Internet/web security to the base station's cell ID ($ID$). 

We add the geographical location of the stationary terrestrial base station in the base station certificate, and the core network uses both the cell ID and the location information to digitally sign and generate the certificate. %which acts as an encoded ID of the base station, in addition to the un-encoded cell ID. 
In addition to the cell ID ($ID$) and public key ($K$), our base station certificate includes the location ID ($L$). $L$ includes the longitude and latitude of the base station and is thus a two-dimensional object, i.e., $L$=$(L_1$,$L_2)$ where $L_1$, $L_2$ are the longitude and latitude coordinate respectively.  %the first coordinate $L_1$ is the longitude coordinate and $L_2$ is the latitude coordinate. %The \emph{encoding} based on the geographical location (keeping track of longitude and latitude) enables the user equipment to cross-check with its own location to verify the location authenticity (the base station and the user equipment are within the physical range of each other). 
Base station's location information is public information, unlike the user equipment's location and behavior requiring privacy, and is thus appropriate for widespread delivery. For example, in the US, the FCC keeps track of the registered base station and publishes their cell IDs and the geographical locations~\cite{fcc_cell_data}%\syc{Cite the FCC database}
, which data is also what we use in our prototype implementation later for simulating the real-world base station deployments. 
% \syc{Include a diagram showing the data fields included in the certificate, and highlight our additions with a different color}
% \sw{} Fig.~\ref{fig:x509contents}

% \syc{Construction involves signing, which is beyond just the information fields}
The certificate construction involves the base station (for key pair generation for the public key and the private key) and the core network (for signing the certificate). %, which communications are drawn in the middle two entities in Figure~\ref{fig:offline}. 
This section focuses on the certificate construction between core network and base station whose computing and communications are drawn in Figure~\ref{fig:offline} between the middle two entities. While Figure~\ref{fig:offline} illustrates our scheme protocol for both the construction and delivery, Section~\ref{subsec:our_scheme_blockchain} describes the delivery part involving blockchain and others. \sour{As shown in Figure~\ref{fig:offline}, the certificate construction process begins with the base station}. During the installation of the new base station or when the current digital certificate expires, the base station generates its own public-private key pair ($K, k$) for each cell. Then the base station sends its \sour{cell ID ($ID$)} and a certificate signing request to the core network. The base station creates separate certificate signing request for each of its cell and send them to the core network for signing, generating one certificate per $ID$ (cell ID). %In the certificate, the base station also includes its location information before sending a signing request. 
Upon receiving the signing request, the core network validates the information and constructs the certificate fields (shown in Figure~\ref{fig:cert_contents})
and digitally signs to generate the certificate signature (in the far-right field in Figure~\ref{fig:cert_contents}). % the certificate of each cell of the base station including the base station's location information $L$. 
% In Figure~\ref{fig:cert_contents}, the core network's signature result is in the far-right field, while the signature depends on the rest of the fields. 


 \begin{figure}[t!]
    \centering
\includegraphics[width=0.5\textwidth]{Images/Diagram_for_Online_V2_Sim.pdf}
    \caption{Online multi-factor authentication by user equipment, including sequential verifications (from top to bottom on the left of the diagram). The blue color indicates our addition in 5G RRC.\sou{Need to replace Algorithm 1 with Multi-factor}}% \syc{This diagram does not have t verification} \sou{revised the figure} %\syc{Fig moved because the Existing 5G subsection makes use of the figure}}
    \label{fig:online}
\end{figure}

\subsection{Certificate Delivery Using Blockchain (Offline)}

% \syc{Previously in the Intro but commented out}
% \syc{From here:}
% \syc{trying to do too much}
% We advance beyond %both the state-of-the-art practice (no authenticity and integrity protection) and 
% the state-of-the-art to enable greater security and efficiency. The state-of-the-art, the most prominent and related to our work~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}, do not make use of the base station's location and adopt PKI to append the public key within the base station's control communication, e.g., when delivering the first broadcast message in 5G RRC. %, and use that to authenticate the base station and its following control communications
% %~\cite{hussain2019insecure,singla2021look,yi1998optimized,zheng1996authentication}. %The related research works are generally covered in Section~\ref{rw}, but the most prominent and related works  
% Our novel location information addition on the base station certificate enables the defense against wormhole attacks %\syc{wormhole?} 
% that can launch fabricated radio control message broadcasting, handover exploitation, dispatching false alert messages, and bidding down attacks. %\syc{Fill these in. After the threat section drafting and establishing the terms, add the threats which gets defended by the location inclusion on the certificate}. 
% Our blockchain application provides a secure record/database of the registered base stations and their public keys/certificates and delivers them offline, which makes the online control communications shorter and enables the use of the cryptographic cipher with greater security/key length. Offline Base station certificate dissemination through blockchain also enables three times less energy consumption at the user equipment for signature verification than state-of-the-art.
% %\syc{Newly added:}
% Such base station certificate construction and delivery enables a multi-factor approach for authenticating the base station and its radio-control communication message; the ID is used to check if the base station is registered and stored in the blockchain database; the location verifies the base station's location integrity; and the digital signature defends against malicious injections. 

% \syc{misplaced}
% \sour{Our rationale for using blockchain in offline communication for base station certificate delivery comes from the inherent byte size constraint of 5G radio control communication imposed by the physical layer. The base station can adopt Public Key Infrastructure (PKI) and send digital certificates to the user equipment in the first radio control broadcast message but according to the 3GPP standard, the physical layer limits message size up to 372 bytes~\cite{3gppphy} making it difficult to fit the base station certificates within the first radio control message. Moreover, in the PKI-based certificate delivery, the user equipment needs to verify the multiple certificates using the network public key installed within before authenticating the base station. The offline blockchain-based certificate delivery addresses both of the pitfalls with no byte length limitations while the secure delivery of base station certificates with its inherent property and the user equipment can authenticate the base station with lower computational time and with lower energy consumption.}

\vspace{-2px}
\subsubsection{Blockchain Enabler, Appropriateness, and Effectiveness} % for Distributing the Base Station Certificate}
%\souc{May be we can considering the reordering of the subsections}
\label{subsec:our_scheme_blockchain}
%- Describe how blockchain play an important role here.
%\syc{Blockchain subsection drafted. I plan to revise.}

Blockchain enables the secure and offline delivery of the base stations' certificates. Blockchain is appropriate for such delivery because, unlike user equipment, the base stations are public entities and publicly advertise their presence via broadcasting SIB1. We store the public information of the base station in the blockchain and avoid the privacy-sensitive or user-equipment-specific information in the blockchain.  %, aligning with its distributed storage and distribution property. 
Our use of the blockchain is also substantially simpler and cheaper than that used in some other blockchain implementations, as we use permissioned blockchain as described in Appendix~\ref{apndx:blockchain_os}. 

%\sou{Blockchain in our scheme}

%\input{Sections/Blockchain_OS}
% The blockchain provides the certificate database $\mathcal{C}$ including the ID (the cell ID as described in Section~\ref{subsec:background_5G}), the public key, and the location information of the legitimately registered and deployed base stations. 
% %\syc{What is the ID we use?} \sou{cell id of the base station}

% The blockchain ledger includes the digital certificates that are signed by the core network and whose subjects are the base stations (as well as the core network itself in the genesis block). % (validating and linking the base station's ID and its public key). 

% The ledger validates and links the ID and the public key of the core network (self-signed in the genesis block) and the base stations (signed and vouched by the core network). The core network uploads its public key and certificate before it digitally signs and generates certificates for base stations, and the genesis block includes the core network's initial public key information. % the private key corresponding to the public key in that certificate is used for digitally signing the other certificates for the Base Stations. 
% Because the core network signs and generates the digital certificates (after the base station generates the key pair and sends the public key to the core network), the core network uploads the digital certificates to the blockchain. The digital certificates in the blockchain ledger are verified, stored, and shared with all the entities involved in 5G networking, including mobile user equipments. 

Blockchain is effective for our base station certificate delivery. Blockchain provides message authentication integrity anchored by the security-robust cryptographic hash function and public-key digital signature. 
Blockchain %also 
provides transparent access to the database/ledger thanks to its distributed storage property; in our scheme, the database includes the registered base stations and blockchain transparency enables accountability. Blockchain also provides automatic synchronization; in our scheme, it can provide the updated base station certificates offline in ad hoc connections, using other non-cellular technology, or from the previous base station connections. 
%
% We use blockchain for the delivery of the base stations' certificates because of the following enabling blockchain properties. Blockchain provides \emph{message authentication integrity} by using the cryptographic primitives of public-key digital signature and the hash function. These cryptographic primitives are robust in security (the computational hardness assumptions) and anchor modern-day digital information and networking security. Blockchain provides easy access to its ledger information and builds on \emph{distributed storage and broadcasting} so that all the nodes store the blockchain ledger (including the base stations' certificates). The distributed storage and broadcasting enable the ledger to get \emph{automatically synchronized in various channels} (e.g., ad hoc connections or from previous base station connections) during the offline times, enabling easier access to the base station certificate information before the online phase using the cellular connectivity services. %For example, a nearby mobile or sensor user can deliver the newest block (containing the new public key of a base station) for the ledger synchronization in ad hoc/peer-to-peer networking. 
%
We experimentally validate and analyze the appropriateness and effectiveness of blockchain for offline base station certificate delivery in Section~\ref{subsec:offline_results}.
%\syc{Move the rest of the paragraph to appnedix} 

%%%%%%%%%% Moved to appendix %%%%%%%%%%%%%%%%
% \begin{algorithm}[t!]
% \small
%     \caption{Multi-factor authentication at user equipment using $ID,K,L,t$}
%     \label{algo:auth}
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \SetKwInOut{Parameter}{Parameter}
%     %\SetKwComment{Comment}{/* }{ */}
%     %\underline{function authentication} ($n$, $t$, $\tau$, $S_k$, cell\_ID, $\bar{L}$, $\bar{t}$)\;
%     %\Input{($n$, $t$, $\tau$, $S_k$, ID_i) received in online phase (SIB1) \\
%     %and ($\bar{L}$, $\bar{t}$) measured at the user}
%     \Input{         $\mathcal{C}$.$ID_{i}$, $\mathcal{C}$.$K_i$, $\mathcal{C}$.$L_i$, \hfill \hfill \hfill /* \textit{Blockchain ledger} */ \\
%                     \emph{SIB1}, $ID_i$, $n$, $t$, $S_k$, \hfill \hfill \hfill /* \textit{Online communication} */ \\
%                     $\bar{L}$, $\bar{t}$ \hfill \hfill \hfill /* \textit{Online sensing} */
%                     }
%     \Output{$A$ \hfill \hfill /* \textit{Authenticated? True (1), False (0)} */}
%     \Parameter {$\tau_t$,$\tau_d$}
%     %/* \textit{Query certificate in blockchain ledger database using cell ID} */ \\
%     %/* \textit{$ID$ verification} */ \\
%     $ A = 0$ \\
%     \If{$\mathcal{C}.ID_i$ == $ID$}
%     {
%        $K_i$, $L_i$ = get($ID$,$\mathcal{C}$.$K_i$, $\mathcal{C}$.$L_i$)  \\
%       % /* \textit{Calculate distance between the base station and the user} */ \\
%        %$d$ = distance($L_i$, $\bar{L}$)
%       % /* \textit{Calculate SIB1 generation and reception time difference} */ \\
      
%        %/* \textit{$SIB1$ authentication} */ \\
%        \If{distance($L_i$, $\bar{L}$) $\leq \tau_d$}
%        {    
%            % $\Delta t$ = $\bar{t} - t$ \\
%        \If{($\bar{t} - t$)$ \leq \tau_t$}
%             {   
%                 \If{$V_{K_i}$(SIB1,$n$,$t$,$S_k$) == 1}
%                 {
%                     \textnormal{\textbf{return}}  $ A = 1$ \hfill  \\
%                 }
%             }
%         }
%     }
% %\vspace{-4px}
% \end{algorithm}


\vspace{-2px}
\subsubsection{Certificate Delivery Using Blockchain}
\label{subsec:our_scheme_cert_distribution}
% While Section~\ref{subsec:our_scheme_blockchain} explains the blockchain used for certificate delivery, we describe how the decentralized blockchain ledger interacts with the rest of the entities. 
% \syc{}
%Building on Section~\ref{subsec:our_scheme_cert_construct} constructing the certificate, 
The core network (after responding to the base station's certificate request as described in Section~\ref{subsec:our_scheme_cert_construct}) uploads the base station certificates to the blockchain, as shown in Figure~\ref{fig:offline}. 
The blockchain ledger includes the digital certificates that are signed by the core network and whose subjects are the base stations (as well as the core network itself in the genesis block to enable the writing/uploading of the certificate). % (validating and linking the base station's ID and its public key). 

% and writes the signed certificate into the blockchain ledger. Only the core network has the write permission for the blockchain ledger. %A mobile user that wants to connect to a network need to synchronize base station digital certificates from blockchain ledger into its local storage. Initially, 

%\syc{New paragraph added to describe the ledger as a database of registered base stations}
The blockchain ledger serves as the registered database ($\mathcal{C}$) of registered base stations for the user equipment. The integrity of such records (i.e., only the core network can write and insert) relies on blockchain technology, as described in Section~\ref{subsec:our_scheme_blockchain}. When the base station presents its cell ID ($ID$), if the user equipment does not find it in its locally stored blockchain ledger, then it determines that the base station is not registered and certified by the core network. 

The base station certificate ($\mathcal{C}$) gets delivered offline via blockchain. 
The user equipment uses the core network's public key stored within its USIM card to verify the authenticity of $\mathcal{C}$ and, upon verification, store $\mathcal{C}$ in its local storage. 
This process occurs offline, which is any time before the user equipment becomes active and connects to the cellular base station as described in Section~\ref{subsec:offline_vs_online}. 

% The user receives the base stations' certificates ($\mathcal{C}$) %($\mathcal{C} = \{ ID_i, K_i, L_i \}_i$) 
% containing the public key and the location information via blockchain from its previous communications, e.g., the Internet using an infrastructure network or from another user through an ad hoc network. %for the first time before initiating radio connection to the base station. Later on, the mobile user can synchronize the ledger periodically once its connected to the network. 
% As a part of the blockchain's validity check, the user equipment verifies the base station's certificate using the core network's public key. 
% %
% The base station relies on the core network to validate its public key because we assume the core network resides in a secure confinement of the service provider and the attacker will not have access to the core network to forge the digital certificate of the base stations or upload malicious certificates into the blockchain ledger. \sour{Finally after the blockchain's validity check, the user equipment stores the base station certificate database ($\mathcal{C}$) in its local storage as illustrated in Figure~\ref{fig:online} (most left).}
% %Blockchain based PKI framework is significantly important here to distribute the public keys of base stations to mobile user using a minimal version of X.509 digital certificate. 





% Simeon version: output boolean, b, remove descriptions in the inputs/outputs/parameter % put `certificate` in math cal, unnecessary comments, right align the comments










% Sourav version:
% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
    
%     \underline{function authentication} ($n$,$t$,$\tau$,$S_k$, cell ID,$\bar{L}$,$\bar{t}$)\;
%     \Input{($n$,$t$,$\tau$,$S_k$, cell\_ID) received in online phase (SIB1) and ($\bar{L}$,$\bar{t}$) measured at the user}
%     \Output{$1\leftarrow$ authenticated, $0\leftarrow$ not authenticated}
%     Query certificate in blockchain ledger database using cell ID \\
%     \If{$certificate.ID=$ cell ID}
%     {
%        /* Get $K$, $L$ from blockchain ledger corresponding to cell ID */ \\
%        $K,L$ = get($certificate.K,certificate.L$)  \\

%        /* Calculate distance between the base station and the user */ \\
%        calculate $d$ = distance($L$,$\bar{L}$)  \\
%        /* Calculate SIB1 generation and reception time difference */ \\
%        $\Delta t$ = $\bar{t} - t $ \\
%        $T\leftarrow$ SIB1 freshness threshold \\
%     \If{$d \leq \tau$ \textnormal{\textbf{and}} $T \leq \Delta t$ \textnormal{\textbf{and}} $V_K$(SIB1,$n,t,\tau,S_k$)}
%          {
%             return 1;\
%          }
%     }
%     return 0\;
%     \caption{Online Base Station Authentication}
%     \label{algo:auth}
% \end{algorithm}


% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
    
%     \underline{function auth\_id} $(ID)$\;
%     \Input{$ID$ received in SIB1 (Cell ID)}
%     \Output{$(K,L)$ or Null}
%     Query certificate in blockchain ledger database using $ID$ \\
%     \eIf{$certificate.ID=ID$}
%       {
%         return $(K,L)$\;
%       }
%       {
%         return Null\;
%       }
%     \caption{Online Base Station ID Authentication}
%     \label{algo:auth_ID}
% \end{algorithm}

% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \underline {function distance} ($(L,\bar{L}$)\;
%     \Input{Base Station location: $L(L_1,L_2)$ from base station certificate as output from Algorithm \ref{algo:auth_ID} \\
%     UE location: $\bar{L}(\bar{L_1},\bar{L_2})$ retrieved by the user} 
%     \Output{$d$}
%     Calculate $d = \sqrt{(L_1-\bar{L_1})^2 + (L_2-\bar{L_2})^2}$
%     \\
%     \underline{function auth\_location} ($\tau,d)$)\;
%     \Input{calculated distance: $d$ from \underline {function distance}, distance threshold: $\tau$ from SIB1 message}
%     \Output{$1\leftarrow$ Valid, $0\leftarrow$ Invalid}

%     \eIf{$d \leq \tau$}
%       {
%         return $1$\;
%       }
%       {
%         return $0$\;
%       }
%     \caption{Online Location Authentication\sw{Make sure all variables are defined in main body as opposed to in the pseudocode, also incorrect definition of a 2D vector, $\mathbf{L} = \begin{bmatrix}
% L_1 \\
% L_2
% \end{bmatrix}$}}
%     \label{algo:auth_location}

% \end{algorithm}

% \begin{algorithm}
% \small
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \underline{function auth\_message $V_K$} (SIB1,$n,t,\tau,S_k$)\;
%     \Input{message: SIB1, $n,t,\tau$ Signature: $S_k$ from SIB1 Public key: K from base station certificate}
%     \Output{$1\leftarrow$ Valid, $0\leftarrow$ Invalid}
    
%     \eIf{$V_K$(SIB1,$n,t,\tau,S_k$)}
%       {
%         return $1$\;
%       }
%       {
%         return $0$\;
%       }
%     \caption{Online Message Authentication}
%     \label{algo:auth_msg}
% \end{algorithm}





\subsection{Multi-Factor Authentication (Online): Setup, Factors, and Verification Sources}
\label{subsec:MFA_factors}
%\sou{A logic diagram or a flowchart for multi-factor}
\vspace{-1px}

In online when the user equipment connects to a base station, the user equipment implements \emph{multi-factor authentication} to authenticate the base station using multiple factors.
The user equipment authentication verification of the subject base station is sequential and uses the multiple factors of ID, $L$, $t$, and the digitally signed SIB1 broadcasting message. 
As these factors are verified and cross-checked with multiple sources, %from the stored ledger to the location sensing to the public-key verification.
Algorithm~\ref{algo:auth} further provides which information factors are from which source between the offline locally stored ledger, the online communications from the base station via 5G RRC, and the user-equipment sensing of the location $\bar{L}$ and time $\bar{t}$. 
% More specifically, we use the $ID$ (to determine if the base station is registered), public key $K$, and location $L$. 
% %The user equipment takes a multi-factor approach to the base station authentication in the online phase. 
We describe the multi-factor authentication within the 5G RRC communication in Figure~\ref{fig:online} and highlight our scheme in blue color, whereas the existing RRC protocol is shown in black color and described in Appendix~\ref{apndx:existing_rrc}.
Table~\ref{table:threat_analysis} also provides an overview of the mapping between the factors and the threats against which they are effective/defending in its farthest three columns. 


%%%% Moved to Appendix: Our scheme
% \subsubsection{Existing 5G Protocol}
% \label{subsec:our_scheme_existing_5G}
% Our scheme builds on the existing 5G RRC protocol for compatibility and practicality (facilitating deployment), and this section builds on Section~\ref{subsec:background_5G} but provides greater details for the 5G RRC protocol interactions between the user equipment and the base station. Figure~\ref{fig:online} shows the standard 5G radio control communication protocol messages in black font color. The user equipment uses such RRC communication protocol so this is a part of the online phase.  


%
%\syc{Start with why this subsection is so important for our work, e.g., compatibility. Refer to Fig.~\ref{fig:online}}\sou{Main focus of this paragraph is explaining the insights of Fig.~\ref{fig:online}. -Base station transmits SI messages periodically -Mobile user wait until next broadcast schedule to get SIBs.}\\
%In this work, we introduce base station broadcast message authentication by the mobile user in Radio Resource Control (RRC) layer of the standard 5G cellular network protocol defined by 3GPP. In Fig.~\ref{fig:online} we show the standard 5G control communication protocol messages in blue font color. \sou{Size limitation of SI messages: Physical layer TBS calculation} At first, the mobile user uses information received from Physical Downlink Shared Channel (PDSCH) signalling and Downlink Control Information (DCI) to determine the transport block size (tbs) that determines the amount of information receives by upper layer. The transport block size depends on modulation order, target code rate, redundancy version, number of resource block that is available at the mobile user using DCI signalling. We illustrate this process as physical layer signaling that takes place at the very first communication from base station to mobile user. It is important to note that according to 3GPP standard \cite{3gppphy}, the amount of information the mobile user expected to receive in system information message is determined by the transport block size (tbs) which is 2976 bits (372 bytes). 






% In 5G NR RRC protocol, the base station transmits system information messages with different periodicities: MIB message with a periodicity of 80 ms, SIB1 with a periodicity of 160 ms~\cite{3gpprrc}. It is minimum for the user equipment to acquire MIB and SIB1 since they contain essential radio connection-related information and the user equipment has to wait to get the system information message until its next broadcast schedule.

% Therefore, the user equipment can only initiate an RRC connection request once it gets all the necessary information from system information messages and later on the complete RRC connection setup using a three-way handshake. After a successful RRC connection with the base station, the user equipment proceeds to set up a NAS connection with the core network. We omit the control communication between the base station and the core network in this work as it is out of the scope of our research. 





%  Prior to setup RRC connection with base station, the mobile user periodically receives a number of broadcast messages to get necessary information about the network. Master Information Block (MIB) and System Information Block Type1 (SIB1) are called Minimum SI since they are essential for the mobile user to get initial radio connection related information. The base station transmits MIB with 80ms and SIB1 with 160ms periodicity. The periodicity of other system information messages are scheduled in SIB1. 

\subsubsection{Signature Generation at Base Station}
\label{subsec:online_signature_generation}
%\sw{Make it d for distance, tau for distance threshold}
% \sou{Getting rid of nonce in our scheme, because it seems it does not server much purpose in replaying attack. Rather we send timestamp and time threshold. These timebased values will serve the same as nonce. Time itself if a nonce.}

%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%%%%%%%%
% Fig.~\ref{fig:online} depicts the online RRC communication protocol. Before broadcasting SIB1 message the base station generates a digital signature $S_k$(\emph{SIB1},$t$,$\tau_t$,$\tau_d$) on \emph{SIB1}, a timestamp ($t$), a time threshold ($\tau_t$) and a distance threshold ($\tau_d$) using its private key ($k$). The timestamp ($t$) is the SIB1 generation time at the base station and the time threshold ($\tau_t$) is the SIB1 expiration time set by the base station. We use $t$ and $\tau_t$ for replay attack protection during each SIB1 message broadcast. The distance threshold ($\tau_d$) signifies over-the-air the coverage range of the base station that we use to prevent wormhole attacks. The base station appends the digital signature along with the other parameters to the \emph{SIB1} message and broadcasts it. The final SIB1 transmission appends the following:\{\emph{SIB1},$t$,$\tau_t$,$\tau_d$,$S_k$(\emph{SIB1},$t$,$\tau_t$,$\tau_d$)\}.
%%%%%%%%%%%%%%%%%%%% Option 2 %%%%%%%%%%%%%%%%%%%%%
\sour{In our scheme we use the SIB1 for the base station message authentication because it contains the essential control information of the base station and it is periodically broadcasted as described in Section~\ref{subsec:background_5G}.} Figure~\ref{fig:online} depicts the online RRC communication protocol \sour{with our scheme's addition in blue font color}. Before broadcasting SIB1 message the base station generates a digital signature $S_k$(\emph{SIB1},$n$,$t$) using its private key ($k$). % as defined in Section~\ref{subsec:background_public_key}. % on \emph{SIB1}, a nonce ($n$), and a timestamp ($t$) using its private key ($k$). $S_k$ is defined in . 
We use the SIB1 generation timestamp ($t$) and a nonce ($n$) for replay attack protection during each SIB1 message broadcast. The base station appends the digital signature along with the other parameters to the \emph{SIB1} message and broadcasts it. The final SIB1 transmission appends the following: \{\emph{SIB1},$n$,$t$,$S_k$(\emph{SIB1},$n$,$t$)\}.

% \subsubsection{Multi-Factor Authentication at User Equipment}
% \label{subsec:our_scheme_online_auth}
% %\subsection{Online ID and L. Authentication at UE} % Base Station ID/Registration and Location Authentication}
% %\syc{Let's draw a pseudo-code showing the online verification from the user equipment perspective. Start by stating what have been given offline vs. online because these are the inputs of the algorithm; these variables-given are in the Key Component Figure, currently Figure 4, but it would be good to use that to build the rest of the algorithm, including for the location authentication using the distance threshold $\tau$. Is the $\tau$ the distance or the distance threshold?}
% % \syc{What's a multi-factor approach? "The user equipment implements \emph{multi-factor authentication} to authenticate the base station using multiple credentials."}
% In online when the user equipment connects to a base station, the user equipment implements \emph{multi-factor authentication} to authenticate the base station using multiple factors.
% The user equipment authentication verification of the subject base station is sequential and uses the multiple factors of ID, $L$, $t$, and the digitally signed SIB1 broadcasting message, as depicted in Figure~\ref{fig:logic_diagram}. 
% As these factors are verified and cross-checked with multiple sources, %from the stored ledger to the location sensing to the public-key verification.
% Algorithm~\ref{algo:auth} further provides which information factors are from which source between the offline locally stored ledger, the online communications from the base station via 5G RRC, and the user-equipment sensing of the location $\bar{L}$ and time $\bar{t}$. 
% % More specifically, we use the $ID$ (to determine if the base station is registered), public key $K$, and location $L$. 
% % %The user equipment takes a multi-factor approach to the base station authentication in the online phase. 
% We describe the multi-factor authentication within the 5G RRC communication in Figure~\ref{fig:online} and highlight our scheme in blue color. %additions colored in and Algorithm~\ref{algo:auth}.
% Table~\ref{table:threat_analysis} also provides an overview of which factors provide which security protections against which threats in its farthest three columns focusing on our scheme; the rest of this section provides greater details. 

%In our scheme, the base station generates the digital signature $S_k(\mbox{SIB1},n,t)$. The base station then appends and transmits the digital signature ($S_k$), a nonce ($n$), and a timestamp ($t$) to the user equipment as a part of the SIB1 message communication. 



% In the SIB1 message, our scheme adds the data fields of the digital signature ($S_k$), a nonce ($n$), and a timestamp ($t$); these additions to the existing 5G protocol are colored blue in Figure~\ref{fig:online}. 

% we introduce only three additional data fields in the radio control communication and add three additional computations at the user equipment. The three additional data fields in the SIB1 that increase the transmitted bytes are one digital signature ($S_k$), a nonce ($n$), and a timestamp ($t$)}. In computations, we add digital signature generation at the base station. At the user equipment, we add base station ID authentication and certificate reading from the blockchain ledger, location authentication, and message authentication. 

\subsubsection{The Factors and The Verification Sources}
\label{subsec:authentication_factors}
%\noindent \textbf{The Factors and The Verification Sources:} \hspace{0.1in}
In offline, the user equipment access the base station's certificate information $\mathcal{C} = \{ ID_i, K_i, L_i \}_i$, which is stored in its local ledger as described in Section~\ref{subsec:our_scheme_cert_distribution}. 

When the user equipment wants the cellular connectivity, i.e., in online, the base station transmits its ID (the cell ID in 3GPP), SIB1, $n$, $t$ and its digital signature, $S_k(\mbox{SIB1}$). 
The user equipment receives these information and uses the base station's public key $K = K_i$ to verify it where $K_i$ is accessed through the aforementioned offline $\mathcal{C}$. Because we fix the subject base station for our authentication (i.e., we focus on the current base station which the user equipment wants to authenticate and connect to for connectivity if authenticated), we omit the subscript $i$ after accessing it online, including those for $ID_i, K_i, L_i$; if the user equipment switches to another base station, then $i$ changes. 

%
Furthermore, in online, we sense the location $\bar{L}$ and the time $\bar{t}$ to cross-check with the provided $L$ and $t$, the former from the offline ledger because the base station's location is static. 
The user equipment can control the control parameters of $\tau_d$ and $\tau_t$ for the threshold-based verifications of $L$ and $t$. 


% The user equipment receives the SIB1 and $S_k$, $n$, and $t$ and use them to authenticate the base station. %The authentication verification is described in Algorithm~\ref{algo:auth} and occurs locally within the user equipment device as drawn in the left most column in Figure~\ref{fig:online}. 
% %Algorithm~\ref{algo:auth} describes the step-by-step procedure of the authentication verification for the online multi-factor base station authentication that consists of base station ID authentication, location authentication, and SIB1 message authentication. 
% In addition to $S_k$, $n$, and $t$ received during online, the user equipment receives registered base station certificates $\mathcal{C} = \{ ID_i, K_i, L_i \}_i$ via the blockchain ledger during the offline phase and store in its local storage as described in Section~\ref{subsec:our_scheme_cert_distribution}.
% %The UE receives base station ID ($ID$), public key ($K$), and location ($L$) through the blockchain ledger during the offline phase. 
% During the online phase, it receives $ID_i$, $S_k$, $n$, and $t$ via the SIB1 message from a base station with index $i$ as described in Section~\ref{subsec:online_signature_generation}. The user equipment measures its location information ($\bar{L}$) and SIB1 reception time ($\bar{t}$) which we use for base station location authentication. In addition, the user equipment selects two control parameters: the time threshold ($\tau_t$), and the distance threshold ($\tau_d$) to thwart replay and wormhole attacks by location authentication. $\tau_t$ is the upper bound that the user equipment accepts any SIB1 message as fresh. $\tau_d$ is the upper bound of the distance between the user equipment and the base station that sends the SIB1 message. Our rationale for selecting the time and distance threshold at the user equipment is to give the user equipment flexibility to select base stations not only based on the higher received signal strength but also the distance from it and the freshness of the SIB1 message that it receives. The user equipment can make a logical decision while choosing a base station (because higher signal strength with a lower distance is more logical than higher signal strength with a greater distance). 

\subsection{Multi-Factor Authentication (Online): Sequential Authentication and Verification}
% \noindent \textbf{Sequential Multi-Factor Authentication:} \hspace{0.1in}
\sou{Need major revision to be succint}
We use the factors and the multiple sources described in Section~\ref{subsec:MFA_factors} for the sequential authentication verifications, depicted in Figure~\ref{fig:logic_diagram}. We describe the step-by-step verification process in this section and explain how each step provides the security protections. While Table~\ref{table:threat_analysis} also provides an overview of which factor/verification provides which security protections against which threats in its farthest three columns focusing on our scheme, we provide greater details in this section. 

%\syc{The following four subsubsections; please draft them}
%\sou{Drafted the five subsubsections}
\subsubsection{ID to Verify Base Station Registration}
\label{subsubsec:ID}
%First, the user equipment uses the ID enables to look up its locally stored blockchain ledger to verify that the base station is a legitimate registered base station. 
The ID verification enables the user equipment to verify whether the base station is legitimately registered by performing a lookup into its locally stored blockchain ledger $\mathcal{C}$. After receiving the SIB1 message from the base station via online communication, the user equipment extracts the $ID$ (which is the Cell ID as described in Section~\ref{subsec:background_5G}) from the message. It performs a ID lookup within $\mathcal{C} = \{ ID_i, K_i, L_i \}_i$. If the $ID$ matches an ID from $\mathcal{C}$ then the ID of the base station is verified. The base station ID verification prevents the new base station threat explained in Table~\ref{table:threat_analysis}. $\mathcal{C}$ contains only the legitimate base stations verified by the core network during offline certificate construction described in Section~\ref{subsec:our_scheme_cert_construct}, therefore, any new base station with a malicious cell ID will not be authenticated. 

The user equipment accesses the location $L$, and the public key $K$ of the base station after ID verification for the location and digital signature verification.

\subsubsection{$L$ for Spatial Integrity}
\label{subsubsec:L}
% Second it then accesses the base station's registered location information, $L$, stored in the local ledger, and cross-check with its sensed location to verify the physical location integrity. 
Upon successful ID verification, the user equipment performs $L$ verification by cross-checking the base station location, $L$, from $\mathcal{C}$, with its sensed location, $\bar{L}$. The user equipment uses a controllable threshold $\tau_d$ for $L$ verification. $L$ verification is successful if the distance between $L$ and $\bar{L}$ is less than $\tau_d$. It limits the validity of the SIB1 message within $\tau_d$ which prevents the wormhole attack because the location verification fails if the attacker transmits the SIB1 message from a distant base station to the user location. More specifically, the $L$ verification disables the attack scenarios illustrated in Figure~\ref{fig:attacK_wormhole}, because the user equipment accepts the SIB1 from the base station within its own coverage area.

\subsubsection{$t$ for Temporal Integrity}
\label{subsubsec:t}
% Third, it verifies the freshness of the online broadcasting control communication of SIB1 using the timestamp $t$. 
We use $t$ verification as a third factor of authentication shown in Figure~\ref{fig:logic_diagram} to ensure the freshness of the online broadcasting control communication of the SIB1 message. The user equipment receives the SIB1 generation timestamp $t$ from online SIB1 communication and compares the timestamp with SIB1 reception time, $\bar{t}$, sensed at the user equipment. Similar to $L$ verification, in that case, the user equipment uses another controllable threshold $\tau_t$ for $t$ verification. If $\bar{t} - t$ is lower than $\tau_t$ then the $t$ verification is successful. In conjunction with $L$ verification, $t$ verification prevents wormhole attacks by limiting the SIB1 message validity period.


\subsubsection{Digital Signature Verification Using $K$ for Message Authenticity}
\label{subsubsec:SIB1}
% Fourth, it verifies the message authenticity of the digitally signed SIB1 by using the base station's public key, $K$ to verify the signature. 
At the fourth and final authentication, the user equipment verifies the SIB1 message by authenticating the digital signature using base station public key $K$, accessed from $\mathcal{C}$ after ID verification. As described in Section~\ref{subsec:authentication_factors}, the user equipment receives the SIB1 message with the digital signature $V_K$($S_k$(\emph{SIB1},$n$,$t$)) during online SIB1 communication. The user equipment verifies the digital signature $V_K$($S_k$(\emph{SIB1},$n$,$t$)) to validate the authenticity and integrity of the SIB1 message. It prevents the base station spoofing attack because the digital signature protects the message authenticity and integrity and thus the fake base station cannot modify the radio control parameters to divert the radio connection to itself.

\subsubsection{Verifier if All Factors Verified}
The user equipment authenticates the subject base station if all the factors are authenticated and verified. %, i.e., logical and. 
A successful multi-factor authentication returns the Boolean $A$, where $A = 1$ corresponds to being authenticated and $A = 0$ the authentication failure. 

As illustrated in Figure~\ref{fig:logic_diagram}, the user equipment performs the chronological computations locally as described in the Algorithm~\ref{algo:auth} after receiving the SIB1 message from the base station. It verifies the base station ID using $ID$ verification, get the public key ($K$) and location ($L$) from the certificate database ($\mathcal{C}$), verifies base station location using $L$ verification, verifies the SIB1 generation time using $t$ verification, and finally authenticates SIB1 message using $K$.

%%% Commented out for TDSC
% The online multi-factor authentication \sour{at the user equipment} begins with the base station ID ($ID$) verification. After receiving SIB1 messages the user equipment extracts the $ID_i$ (which is the Cell ID as described in Section~\ref{subsec:background_5G}) from the message and performs a certificate query within $\mathcal{C} = \{ ID_i, K_i, L_i \}_i$. If the user equipment finds a relevant base station certificate from $\mathcal{C}$ then we say it validates the ID of the base station. The base station ID validation helps the user equipment to determine whether the base station is registered within the operator network. A successful query returns with a base station certificate containing the public key ($K_i$) and the location ($L_i$) information of the base station. %Algorithm~\ref{algo:auth_ID} shows the pseudocode for the base station ID authentication.

% Upon successful base station ID verification, the user equipment uses the $L_i$ and $\bar{L}$ for the location ($L$) verification. At first, it calculates the distance ($d$) between itself and the base station using their location information ($L$,$\bar{L}$). We also add a replay attack protection mechanism in location verification. For that, it calculates the time difference ($\Delta t$) between $t$ and $\bar{t}$. The user equipment validates the base station location if the two conditions are satisfied: (a) $d$ is less than or equal to $\tau_d$, and (b) $\Delta t$ is less than or equal to $\tau_t$. Upon successful location verification, the user equipment proceeds to SIB1 message verification.

% As shown in Algorithm~\ref{algo:auth_location} the UE performs location authentication using two functions: calculating the distance($d$) between its own and the base station after retrieving its own location ($\bar{L}[\bar{L_1},\bar{L_2}]$), and validating if the calculated distance is within the received distance threshold($\tau$). The UE uses the Euclidean formula to calculate the distance. If the calculated distance ($d$) is less than or equal to the distance threshold ($\tau$) then the UE authenticates the location of the base station. The UE gets base station location ($L[L_1, L_2]$) information from the base station certificate offline and distance threshold ($\tau$) from SIB1 online. 

%%%%%%%%%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%
% The location authentication prevents the wormhole attack and the replay attack. The base station sets the distance threshold ($\tau_d$) because its coverage range depends on several factors: spectrum, terrain, and transmitting power. As the frequency band increases the coverage range of a base station shrinks. The coverage area decreases in urban areas with more obstacles than in rural areas for a particular frequency band. However, increasing transmitting power expands the coverage range. Typically a 5G base station operating in millimeter wave frequency has $15$ to $600$ meters of coverage range. The base station also sets the SIB1 expiration time threshold ($\tau_t$) based on its transmission characteristics. The rigorous analysis of distance threshold and time threshold calculation is beyond the scope of this research work.

%%%%%%%%%%%%%%%%%%%%%% Option 2 %%%%%%%%%%%%%%%


%\vspace{-12px}
%\subsection{Online Message Authentication at UE} %\subsection{Online Base Station ID and Message Authentication}
%\label{subsec:our_scheme_online_auth}
%\label{sec:online_bs}
%- Describe the authentication process. \\
%- Include design diagram here.
%\syc{The online section should include the following: the authentication of the IDs (including the location authentication) and the message authentication via the digital signature. We may want to split the two subsections}\\
%\souc{Below paragraph deserves an earlier position as it describes base station generating SIB1 message with signature.}
%\sw{Using $\tau$ instead of $d/d$}

%% Moving to an ealier new section
% Fig.~\ref{fig:online} depicts the online RRC communication protocol. Before broadcasting \emph{SIB1} message the base station generates a digital signature $S_k$(\emph{SIB1},$n$,$t$,$\tau$) on \emph{SIB1}, a nonce ($n$), a timestamp ($t$) and a distance threshold ($\tau$) using its private key ($k$). The nonce ($n$) is an arbitrary value and the timestamp ($t$) is the SIB1 generation time at the base station. We use $n$ and $t$ for replay attack protection during each \emph{SIB1} message broadcast. The distance threshold ($\tau$) signifies over-the-air the coverage range of the base station that we use to prevent wormhole attacks. Finally, the base station appends the digital signature along with the other parameters to the \emph{SIB1} message and broadcasts it. The final \emph{SIB1} transmission appends the following: \{\emph{SIB1},$n$,$t$,$\tau$,$S_k$(\emph{SIB1},$n$,$t$,$\tau$)\}.


% The mobile user ensures the availability of its offline blockchain ledger within its local storage prior to initiating the RRC connection. Upon reception of \emph{SIB1}, \sou{we introduce three additional processing along with standardized \emph{SIB1} message handling: (a) get base station certificate (b) verify time and location of \emph{SIB1} (c) verify the digital signature.} At first, the mobile user looks up the \sou{base station certificate} from the blockchain ledger in its local storage using the \emph{ID} received in \emph{SIB1}. \sou{The base station certificate contains the public key ($K$) and the location ($L$) of the base station which are used for authentication and location verification. }

%\syc{Some of these would need to move to the previous section, as it focuses on the location authentication}
%\souc{From here the UE message authentication begins} \\

%%%%%%%%%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%
% Finally, during the message authentication, the UE verifies the digital signature $V_K$($S_k$(\emph{SIB1},$t$,$\tau_t$,$\tau_d$)) using the public key $K$. This validation ensures the authenticity and integrity of the contents of the SIB1 message. After successful verification of the digital signature, we say the base station is authenticated. Then, the UE proceeds to establish an RRC connection with the base station and then the NAS connection with the core network. If the base station is not authenticated then it again starts listening to system information messages from other base stations. 

% In the online phase of our scheme, we add the following four additional data fields in the SIB1 and increase the transmitted Bytes: the digital signature, the timestamp, time threshold, and the distance threshold value. In computations, we add digital signature generation at the base station. At the UE, we add base station ID authentication and certificate reading from the blockchain ledger, location authentication, and message authentication. Algorithm~\ref{algo:auth} depicts the step-by-step procedure of the online base station authentication.

%%%%%%%%%%%%%%%%%%%%%% Option 1 %%%%%%%%%%%%%%%
%\syc{Describe and explain $\mathcal{A}$}
% Finally, during the SIB1 message authentication, the user equipment verifies the digital signature $V_K$($S_k$(\emph{SIB1},$n$,$t$)) to validate the authenticity and integrity of the SIB1 message. Successful verification of the digital signature yields $A = 1$ which means online multi-factor base station authentication at the user equipment is successful. Then, the user equipment proceeds to establish an RRC connection with the base station and the NAS connection with the core network afterward according to the existing standard. If $A = 0$ then user equipment again starts listening to system information messages from other base stations. 

% \syc{Why is this placed here? Isn't the previous paragraph better to end this subsection? Please consider the flow between the paragraphs.}
% In the online phase of our scheme, \sour{we introduce only three additional data fields in the radio control communication and add three additional computations at the user equipment. The three additional data fields in the SIB1 that increase the transmitted bytes are one digital signature ($S_k$), a nonce ($n$), and a timestamp ($t$)}. In computations, we add digital signature generation at the base station. At the user equipment, we add base station ID authentication and certificate reading from the blockchain ledger, location authentication, and message authentication. 

==> Sections/Old_Tex_Files/11142023_Abstract.tex <==
\begin{abstract}
\souc{will update later}
%\syc{Call our scheme blockchain-based key distribution (BBKD)?}
%\sou{Task list:
%\begin{itemize}
%    \item SP: Implement mobile user on other platforms (raspberry pi is preferable) and then power measurement. We'll use ligt-weight computing device. - Completed
%    \item SW/AS: Blockchain offline experiment with remote Cloud
%    \item SP: Online experiment with an improved version of STA Research and our scheme in terms of \textit{signature size} and \textit{public key length}. Goal is to make it close to theoretical value. 
%    Update: 15 May: Signature size is reduced by ~10-15 bytes. Public key (sta research) has been reduced by half (110 bytes to 52 bytes). Yet, ECDSA-224 is the max in sta research. - Done
%    \item SP: Online experiment with varying locations and distance between base station and mobile user. (Base station location. Varying location cannot be done due to signal attenuation but distance experiment (5m, 10m, 15m) is ongoing. 1200 samples for each (our scheme, sta practice, sta research). - Ongoing for 15m distance
%    \item SW: Blockchain offline experiment with local USRP
%    \item SP: Taking large experimental samples with varying algorithms (more specifically, RRC handshake) - Not started yet.
    %\item Post-quantum too ambitious?
%\end{itemize}
%} 
%\syc{20-250 words for abstract for CNS submission}

Malicious or rogue base stations are critical and  well-studied issues in telecommunications networking, %While there are digital security between the user and the backend core network, 
but the current cellular practice remains vulnerable lacking the base station key and authentication. % and the R\&D community only recently proposed to introduce the base station's public key. 
We design and build a blockchain-based key distribution scheme and then use the key to authenticate the base station in 5G radio resource control (RRC) in which the base station transmits a digitally signed broadcast message. The blockchain delivers the base station's public key and builds on its strengths of high integrity (only the core network can write on the blockchain and distribute the keys) and automatic, distributed, and offline synchronization and delivery. %, advancing the start-of-the-art research which distributes the keys in the broadcasting and bandwidth-limited RRC chanenls at the time of the communications. 
Our base station authentication uses the 5G RRC protocol's SIB1 message transmission (regularly broadcasted to the nearby mobile users) and enables the public-key authentication using the digital signature ciphers with greater security levels than the previous research (by offloading the base station's public key distribution in the offline blockchain). We implement and validate our scheme for both offline key distribution and online cellular communications. % (offline is before the telecommunication session and online is during). 
Our implementations simulate the user, base station, and core network and involve radios and computers for both the online 5G communications (srsRAN and SDR) and offline key distribution (Ethereum smart contract with the third-party blockchain transmitter in both the local ad hoc and Internet-remote environments). %For such systems study and implementation, in addition to simulating the telecommunication entities (user, base station, and core network), we implement a third-party node to highlight the distributed delivery of the base station's public key (while only the core network can write, anybody can store and transmit the blockchain). %We use srsRAN and software-defined radio (SDR) for the online base station authentication and RRC communications between the user and the base station, and use Ethereum smart contract for the offline key delivery. % To highlight the automatic and robust blockchain-based key distribution, we also implement the offline key delivery (before the user becomes active for telecommunication networking) in both local and remote experiments and show how the blockchain is appropriate for base station's public key distribution. 
Our experiments show that our scheme can support ECDSA with greater key lengths/security and that the mobile user's computing and energy consumptions are more efficient than the state-of-the-art research due to the blockchain-based offline key distribution. %because the offline key distribution enables the authentication using just one signature verification. 
% \syc{What are the result highlights? Expand with eye-popping numbers for: blockchain is appropriate and its typical issues are non-issues here; online comm. is low in overhead in both duration and energy and the ciphers work}
% \sou{Highlights Online: Low overhead in SIB1 message implies adopting higher elliptic curves signature algorithms, 3.50 times lower signature verification time overhead implies 3.22 times lower energy consumption at the mobile user, cryptographic operation does not incur overhead in RRC connection time}
\end{abstract}

\keywords{Cellular Network, 5G, Blockchain, Rogue Base Station, Base Station Authentication}

==> Sections/Old_Tex_Files/11182023_STA_Research.tex <==
\vspace{-2px}
\subsection{State-of-the-Art Research}
\label{subsec:sta_r}

%\syc{Need confirmation (paragraph):}
Most closely related to our research to authenticate the base station has been conducted by Hussain et al.~\cite{hussain2019insecure}. %and Singla et al.~\cite{singla2021look}, 
%\syc{How does the Singla et al. using identity-based crypto relevant here? Need more info if we want to include.}
Hussain et al.~\cite{hussain2019insecure} use ECDSA-224 cipher algorithm for the digital signature (Singla et al.~\cite{singla2021look} uses the %aggregate signature based on identity-based cryptography using 
Schnorr signature algorithm for identity-based cryptography but we focus on the ECDSA because ECDSA is popularly used in mobile computing and is standardized by NIST (unlike Schnorr)~\cite{niststandard}, although NIST is having preliminary discussions about standardizing Schnorr signature algorithm~\cite{nistschnorr} ). 
This \emph{state-of-the-art research} (STA Research)~\cite{hussain2019insecure} uses the preinstalled public key of the core network in the USIM of the mobile devices (described in Section~\ref{subsec:offline_vs_online}) as the initial anchoring point to generate the certificate chain, and the mobile user verifies the digital signatures of intermediary node (MME/AMF) and base station through the certificate chain (using the public keys of those along the chain). After the verification of the certificate chain, the user can verify the digital signature of the SIB1 message using the base station's public key. In this state-of-the-art research, the mobile user verifies three digital signatures (core network, MME/AMF, SIB1) to authenticate the base station before responding to the base station's SIB1 and making the RRC connection. \sou{Furthermore, both of the recent research works proposed timestamp or location-based solutions for protection against replay/relay attacks. However, in their scheme, the base station sends the threshold values or the location along with the SIB1 message which requires integrity validation of the message before utilizing those parameters which leads to false positive validation.}  %\syc{Is this description applicable to both of the previous research?} 
%There exist two comparable state of the art research ~\cite{hussain2019insecure,singla2021look} that addressed the same key distribution and authentication problem using PKI based and Identity Based schemes respectively. We adapt the core idea of their base station public key distribution and refer it as \emph{state-of-the-art research} in this work. In the state-of-the-art research, the mobile users have preinstalled public key of a trusted node (core network) in their mobile devices using Universal Subscriber Identity Module(USIM) that acts as an anchoring point to verify the public keys of intermediary node (MME/AMF) and base station through certificate chain verification. After successful verification of certificate chain, the mobile user can verify the digital signature of SIB1 message using base station public key. Mobile users get the public keys (MME/AMF, base station) and digital digital signatures (core network, MME/AMF, SIB1) from SIB1 messages broadcast by the base station in RRC layer connection procedure. In the state of the art research, the mobile user needs to verify three digital signatures (core network, MME/AMF, SIB1) to authentic the base station before initiate RRC layer connection setup request. 


\begin{figure}
\includegraphics[width=1\columnwidth]{Figures/horizontal_bar_plot_byte_size_distribution.eps}
    \caption{SIB1 packet size comparison between our scheme and State-of-the-Art research (STA Research) with different signature algorithms. The vertical line shows the SIB1 size limit of 372 Bytes.\vspace{-13px}}
    \label{fig:sib1_packet_size_i}
\end{figure}

\noindent \textbf{Our Scheme vs. STA Research:}
%\syc{Need confirmation (paragraph):}
Our work partly builds on these state-of-the-art works in that we also rely on the core network's public key delivery via USIM, use the ECDSA digital signature, and encode the signature in the RRC SIB1. However, our scheme advances this previous research and differs from them in \sou{three} critical ways. First, our scheme reduces the number of signature verifications by directly sharing the base station's public key, while this previous research requires three digital signature verifications (for the core network, MME/AMF, and SIB1/base station). Second, our scheme delivers the base station's public key offline via blockchain, while the previous research delivers them along with SIB1 online, i.e., appends the public key in SIB1. Our scheme, therefore, enables ECDSA digital signature algorithms of greater security and key length and reduces computation and battery power consumption. \sou{Third, the inclusion of location information in the base station certificate enables our scheme to prevent location spoofing attacks.}
% 
As shown in Fig.~\ref{fig:sib1_packet_size_i}, our scheme can support all the ECDSA ciphers with varying key lengths and security strengths, while the SIB1 size limit of 372 Bytes (as described in Section~\ref{subsec:background_5G}) prohibits the use of ECDSA with greater keys beyond ECDSA-224 in state-of-the-art research. We also experimentally validate and analyze the reduced computation and energy use in Section~\ref{sec:implementation_results}. 

==> Sections/Threat_Model.tex <==
\section{Threat Model and Problem Description}
\label{sec:threat_model}

%\syc{Let's discuss about Threat Model. We would want to establish what we need here and what purposes this section serves.}

\subsection{Threat Model}
%- Describe the capabilities of attackers due to lack of base station authentication.

%- Impersonating a legitimate base station
%- Related work implies this threat Model.

In our threat model, the attacker can have the following capabilities due to the lack of authentication mechanism for the broadcast system information messages:

\subsubsection{Spoofing a legitimate base station} An active attacker is capable of setting up and operating its own malicious base station with the same system parameters (cell id, plmn id, tac, frequency info etc.) as the legitimate base station using SDRs and open-source tools. The adversary can acquire the system information of legitimate base stations by eavesdropping on the public broadcast channels (system information messages). Subsequently, the malicious base station lures the mobile users to camped into it by broadcasting the system information messages with a higher signal strength than the legitimate base station. This enables the adversary to launch bidding down attacks, Authentication and Key Agreement (AKA) bypass, location tracking, traffic monitoring, DNS redirection, and SMS phishing attacks after the mobile user gets connected to the malicious base station. Furthermore, the adversary can launch denial-of-service attack to make the mobile users become unable to attach to or get any network service from the legitimate network.

\subsubsection{Protocol message tempering} In our threat model, we also consider that an adversary has the capabilities to temper the radio resource control (RRC) protocol messages by acting as a man-in-the-middle. In such case, the attacker can modify, drop, or redirect protocol messages transmitted between legitimate participants (base station and mobile user). Modification of the system information messages enables the adversary to configure mobile user device with malicious parameters to establish an RRC connection to the malicious base station. The adversary broadcast these modified system information messages using malicious base station where the mobile users are oblivious to it. %complete ignorant about it.

Additionally, we also consider that the adversary can launch replay attacks to exploit the communication and perform malicious activities. Physical accessibility of the attacker to the base station and core network are out of the scope of our threat model. In the following subsection, we address these vulnerabilities described in our threat model and present our contribution to the problem.

\subsection{Problem Description and Our Contribution}
%- Lack of integrity/authenticity of system information (SI) broadcast messages. \\
%- Design a scheme to verify and validate SI broadcast messages by the mobile user before connection to a network. \\
%- Reduce overhead by breaking down the process into two parts: Offline & Online. \\
%\subsubsection{Problem description} 
In the current 5G standard, due to the lack of authentication mechanism for system information messages, the adversary can lure the benign mobile users to camped into the malicious base station while keeping the mobile users ignorant about the underlying network. Thus, the adversary can launch different privacy and security-related attacks on mobile users. Therefore, the mobile users need to validate the authenticity (legitimacy) of the base station before establishing connection to it and a secure public key distribution of the base station to the mobile users is a prerequisite to achieve this task.

%\subsubsection{Our contribution} 
%To provide authenticity of base station system information messages we design a scheme where cellular network securely distribute its base station public keys to the mobile users and the mobile users use this public key to verify the authenticity of the broadcast messages generated by the base station. 
To provide authenticity of base station system information messages, we design a scheme where cellular network securely distribute its base station public keys to the mobile users in an \emph{offline} phase to use the public keys to verify the authenticity of the broadcast messages generated by the base station in \emph{online} phase.
In our design, we use blockchain-based PKI to securely distribute the base station public key to mobile users. In order to provide the authenticity of base station, we use digital signature scheme on \emph{System information Block Type1 (SIB1)} message since it is cell-specific and carries important network parameters that the mobile users use to initialize RRC connection and acquire other \emph{System information Block (SIB)}s. 

There exist two comparable State-of-the-Art research ~\cite{hussain2019insecure,singla2021look} that addressed the same key distribution and authentication problem using PKI-based and Identity-Based schemes respectively. We adapt the core idea of their base station public key distribution and refer it as \emph{state-of-the-art research} in this work. In the state-of-the-art research, the mobile users have preinstalled public key of a trusted node (core network) in their mobile devices using Universal Subscriber Identity Module (USIM) that acts as an anchoring point to verify the public keys of intermediary node (MME/AMF) and base station through certificate chain verification. After successful verification of the certificate chain, the mobile user can verify the digital signature of SIB1 message using base station public key. Mobile users get the public keys (MME/AMF, base station) and digital digital signatures (core network, MME/AMF, SIB1) from SIB1 messages broadcast by the base station in RRC layer connection procedure. In the State-of-the-Art research, the mobile user needs to verify three digital signatures (core network, MME/AMF, SIB1) to authenticate the base station before initiating RRC layer connection setup request. 

In this work, we also refer \emph{state-of-the-art practice} as the current 3GPP standard where no authentication mechanism broadcast system information of base station exists. Although,~\cite{3gppfbs} propose a recommendation of protecting system information messages but it is yet to be implemented in real-world application.

Our contribution over state-of-the-art research and state-of-the-art practice are: (a) offline distribution of the base station public key to reduce the overhead bytes in SIB1 that enable us to use large-key sized ECDSA algorithms and (b) significantly reduce the signature verification time at the mobile devices which in turns reduce computation and battery power consumption.

\syc{Add high-level comparison against STAP and STAR. This comparison can later be better supported in the Experimental section.} \sou{added}


==> Sections/blockchain_RW.tex <==
\section{More Related Work on Blockchain for Key Management and PKI}
\label{appendix:related}

%\noindent \textbf{Blockchain for Key Management and PKI} \hspace{0.05in} 
%\subsubsection{Blockchain for Key Management and PKI}
%\label{subsubsec:rw_blockchain}
Previous works proposed using blockchain to secure key management and PKI in different scenarios, including smart contract security~\cite{yakubov2018blockchain}, vehicular networking~\cite{sarker2021blockchain}, the digital public-key infrastructure in the web~\cite{matsumoto2017ikp,al2017scpki}, and domain name system (DNS)~\cite{ali2016blockstack}. 
Our work uses the adapted version of the blockchain technology (minimizing the consensus protocol, as described in Section~\ref{subsec:our_scheme_blockchain}) to secure the key management for base stations in the cellular network and take a systems approach for our research.


==> Sections/blockchain_scalability.tex <==
\section{Our Scheme Performance on Blockchain Scalability}
\label{apndx:blockchain_scalability}

\syc{lower priority}

\begin{figure}[t!]
\centering
\includegraphics[width=1\columnwidth]{Figures/bbkdbscalability_Sim.pdf}
\caption{Blockchain scalability in the certificate rate and the block arrival rate.}
\label{fig:bbkdbscalability}
\end{figure}

While blockchain scalability (how many transactions per second can get processed) is a critical challenge in some other blockchain applications, our blockchain used for the base station certificate delivery has a significantly smaller scalability requirement (the required transactions per second) and the ledger growth rate (the ledger Byte per second) than other blockchain applications. 
%
Given the number of base stations $x$ 
and the average lifespan of a base station $y$ (in years), we estimate that the rate of certificate upload on the blockchain is $\frac{x}{y}$ certificates per year or $(60 \cdot 60 \cdot 24 \cdot 365)^{-1} \frac{x}{y} = \frac{x}{3.1536 \cdot 10^7 \cdot y}$ certificates per second. %We use $y=1$ year \syc{Need to justify why this is an aggressive number. As a part of that, include 30-50 years of the steel tower.} 
Assuming that one block includes one certificate/transaction (there can be more efficient schemes including multiple certificates per block), our blockchain requires a scalability rate of $\frac{x}{3.1536 \cdot 10^7 \cdot y}$ certificates per second. 
The ledger size also grows $1417 \frac{1417 \cdot x}{3.1536 \cdot 10^7 \cdot y}$ Bytes per second because one block is $1,417$ Bytes long in our implementation. 
%\syc{Arijet: Fill these in and provide the sources:}\as{addressed}
Fig.~\ref{fig:bbkdbscalability} shows the number of certificates required and the ledger size growth rate, assuming that the number of base stations $x = 4.189 \times 10^5$~\cite{basestationnumber}. % This number is as of Dec 2021
%$1.38 \times  10^6$
%\as 46kB - one transaction
This scalability requirement for our scheme (the certificate rate on the left vertical axis in Fig.~\ref{fig:bbkdbscalability}) is significantly less than both the blockchain scalability capacity recommended by Ethereum smart contract (20 transactions per second~\cite{ethereumtxpersecond}) and the average transactions per second in June 2024 for Ethereum (13.52 transactions per second) and Bitcoin (5.53 transactions per second). %\souc{Simeon: Would you please update the data?} %\syc{Simeon or Arijet: Need help with the transaction scalability with Bitcoin and Ethereum in transactions per second in practice} %\sou{updated as of May}
For example, if the average base station lifespan is 0.5 years (we expect the actual lifespan is likely higher than this, c.f., the physical steel/cell tower hosting the base station has a lifespan of 30-50 years~\cite{celltoweryear}), the certificate rate requirement is 0.0266 certificates/transactions per second, which is three orders of magnitude smaller than the 20 transactions per second as recommended by the Ethereum smart contract for decentralized blockchain applications. 

==> Sections/commented_out_texts.tex <==
%\syc{Sourav: Do you use these acronyms? Let's be consistent with these terms. I would generally recommend reducing the use of acronyms for the description of our work unless it really helps with the spacing in figures and tables. You may still include the well-known acronyms in the Background section, but it's probably worth transforming them to a more generic/descriptive words in our research paper beyond the Background section. I would suggest to call these user or mobile user vs. base station vs. core network and be specific what these are. The Background section should clearly define what these are.}
% transformed all user equipment (UE) to mobile user.
%5G cellular network consists of three main components: 5G core network, Next Generation Radio Access Network (NG-RAN) and mobile users. 5G core network consists of important nodes (such as AMF, AUSF, SMF etc.) for different logical functionality, however in this paper, we abstract \syc{Use present tense} all of these nodes as 5G core network. Next generation radio access network comprise of base stations (which act as the trusted intermediary node between the mobile user and the 5G core network) that are distributed across a wide geographical area for cellular network coverage. A mobile user needs an user equipment with an Universal Subscriber Identity Module (USIM) to access into the cellular network to get services. The mobile user at first establishes Radio Resource Control (RRC) layer radio connection with the base station using the system parameters broadcast by the base station itself. After successful radio connection establishment with the base station, the mobile user then able to establish Non-Access Stratum (NAS) layer control communication connection to the core network to avail the cellular services (voice, data). \syc{Better highlihg the radio/wireless vs. digital backend}
%5G cellular network consists of three main physical entities: core network, base stations and mobile users. As illustrated in figure \ref{fig:overall_arch}.a mobile users are connected to the base station using wireless channels and base stations are connected to the core network through a wired network. The mobile users have to install Universal Subscriber Identity Module (USIM) into its device before initiate connectivity establishment with the network. Prior to avail cellular services the mobile users need to establish Radio Resource Control (RRC) layer connection with the base station and then it able to establish Non-Access Stratum (NAS) layer connection to the core network. Figure \ref{fig:overall_arch}.b shows the RRC and NAS layer connectivity diagram. 


%we are proposing a scheme where the legitimate base station securely disseminate its public key to the mobile users so that the mobile users can authenticate the base station broadcast messages by verifying the digital signature generated by the base station.

%\subsection{Digital Signatures and Certificates}
%In terms of message authentication (or integrity) there are two popular methods: symmetric key based message authentication code  and asymmetric key based digital signature. The drawback of message authentication code is it cannot protect the message from repudiation and a private key needs to be shared magically between communicating parties. On the other hand digital signatures use a private key to sign a message and corresponding public key to verify it. Although it is computationally costly as compared to MAC techniques yet digital signatures are more secure and convenient in several ways: convenient key distribution and management, publicly verifiable signatures and more importantly it has non-repudiation property. 

%While the verifier needs the public key of signer to verify a digital signature, a trusted authority (whom the signer and verifier can trust) can signs the public key of the signer in a digital certificate and it can be share with the verifier through an authentic channel. The trusted party, in this case called the Certificate Authority (CA), plays an important role for public key distribution in the digital signature based message authentication scheme. The certificate itself must contains some mandatory information field so that the verifier can retrieve public key for a specific signer. 

%\noindent \textbf{In our research} \hspace{0.05in}

%- What digital signature algorithms we are considering and why? We are going to implement ECDSA, RSA, PQC consecutively.

%- For digital signatures what type of certificate we are going to use and why? We are going to use X.509 V1 with mandatory fields.

%
%\subsection{Commit-and-Reveal Scheme}
%The commit and reveal scheme in cryptography allows the sender to a commit a message by generating hash of it and %send it to the receiver and reveal the committed message later on so that receiver can verify the hash it received %from the sender after generating the hash from the reveal message. This idea can be utilized in message integrity %protection in data communication where any sender wants to send multiple consecutive messages to the receiver. The %commit-and-reveal method is less costly as compared to digital signature since only hash functions are used.
%



%\begin{figure}
%    \centering
%    \includegraphics[scale=0.35]{Images/Overall_architecture}
%    \caption{Overall architecture of 5G cellular network \syc{Make these two separate subfigures; split them to two figures. Add "Fig. 1(a) shows the physical topology between the user, base station, and core network, including the router switches forwarding the packets between the base station and core network. Fig. 1(b) shows the protocol interactions of RRC vs. NAS between the participating logical entities, while ignoring the geogrpahical distance." It would be good if the text supplements this and emphasizes the base station being closer to the user and reinforce that "for one core network, there are multiple base stations." Such argument may later reap its fruit when we discuss the scalability of the blockchain.}}
%    \label{fig:overall_arch}
%\end{figure}

%In the area of telecommunication, user registration, Universal Subscriber Identity Module (USIM) data storage are the offline process that does not require active communication between the mobile user and the network. On the other hand, after powering on the mobile user device, it starts the online process to get connected to the network to avail the service. 

%PKI based Digital signature schemes consists of three stages: key generation, signing and verification. Key pair (private and public) generation and distribution is a single time activity within a certain period of time. The public key can be distributed through digital certificates with a certain validity period. On the other hand, digital signature generation by sender and verification by the receiver is a multiple time activity as long as the digital certificate is valid. Thus, to reduce computation overhead and faster execution, the whole process can be divided into two phases: 1) Offline key generation and distribution 2) Online signature generation and verification. Likewise, key generation and digital certificate distribution of a base station can be done in offline prior to initiate communication to the users whereas signing and verifying can be done online during communication.

%- How we divided our scheme into online and offline parts with example.
%- Can include some references regarding offline and online aspects of PKI. How it enhanced efficiency.

%\noindent \textbf{In our research} \hspace{0.05in} we merge the offline and online concept of cryptography and telecommunication to bring the efficiency of our scheme. Base station public key can be generated and distributed to the mobile users during offline phase. We use blockchain based PKI to distributed base station public key in this phase. So, in offline phase before initiate the radio connection to the base station the mobile users avail the public key of the base station. During the bootstrapping of radio connectivity the online phase starts and the mobile user use the public key got from offline phase to authenticate the base station.

%\subsection{State of the art Research and Practice} In this research paper, we define state of art research with respect to authenticate base station broadcast \textit{system information} messages as discussed in ~\cite{hussain2019insecure,singla2021look}. We take the concept of the authors' public key dissemination where the mobile users have preinstalled the public key of the core network in their mobile devices using universal subscriber identity module and this public key acts as an anchoring point to verify the public keys of mobility entity (MME/AMF in this case) and base stations.\textit{System information} message of the base station contains public keys (MME/AMF, base station) and digital signatures (core network, MME/AMF and \textit{system information}). In the state of the art research concept the mobile user needs to verify three digital signatures (core network, MME/AMF, \textit{system information}). 

%We consider state of the art practice as the current 3GPP standard where no authentication mechanism of base station \textit{system information} exists. Although, \cite{3gppfbs} propose a recommendation of protecting \textit{system information} messages but it is yet to be implemented in real world application. 

%\subsection{Performance Analysis}
Figure \ref{fig:online_performance} illustrates the performance of our scheme vs the state of the art research. We use 5 different curves of ECDSA digital signature algorithm while measuring the performance of the systems. 
\subsubsection{SIB1 message overhead} In our scheme the message overhead is lower than the state of the art research (in figure \ref{fig:SIB1_overhead}). For ECDSA-224 our SIB1 overhead is only $95$ bytes whereas the state of the art research has $259$ bytes, because, in state of the art researchm, SIB1 message include public keys of three entities (base station, mobility entity (MME/AMF) and the core network) and three digital signatures (SIB1, Mobility Entity and the core network). \\
- Our scheme supports higher ECDSA curves (longer key length) which may implies greater security \\
- Due to size limitation of SIB1 message state of the art research does not support higher ECDSA curves.

\subsubsection{Signature verification time} Signature verification time at the mobile user has greater impact on overall RRC connection setup time. Figure \ref{fig:sign_verification} shows the comparison of signature verification time between our scheme and state of the art research. \\
- Our scheme has lower signature verification time as compared to state of the art research because, in our scheme we need to verify only the SIB1 digital signature whereas in state of the art research, the mobile user verifies three digital signatures (core network signature, MME signature and SIB1 message signature).
- Average signature verification time increases as the ECDSA cruve size increases which is expected.

\subsubsection{Key reading time} Upon reception of SIB1 message the mobile user get the public key of the base station from the blockchain ledger using the ID. The key reading time is significantly low as compared to signature verification or RRC connection time. So, only the signature verification time adds the computational time overhead in RRC connection time.


% \subsection{Experimental Setup}
% \begin{figure}
% \begin{subfigure}{0.32\columnwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/algsPubkeySize.pdf}
%     \caption{Public key size}
%     \label{fig:handshakesize}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.32\columnwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/algsPrivkeySize.pdf}
%     \caption{Private key size}
%     \label{fig:handshakesize}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.32\columnwidth}
%     \centering
%     \includegraphics[width=1\textwidth]{Figures/algsSigSize.pdf}
%     \caption{Signature key size}
%     \label{fig:handshakesize}
% \end{subfigure}
% \caption{Size of public key, private key, and signature. \syc{If this is deterministic, it would be better off to just give the number in tables. Tables with the actual numbers is easier to see.}}
% \label{fig:sizes}
% \end{figure}

==> Sections/digital_signature_primer.tex <==
\vspace{-2px}
\section{Crypto. Primer: Digital Signature Security Assumptions and Algorithms}
\label{appendix:background_public_key}
\syc{Becomes higher priority for ToN (less so for the security venues)}
Public-key cryptography provides the standard and widely used cryptographic techniques for the digital signature (providing sender authenticity and message authenticity) and public-key infrastructure or PKI (providing the digital certificate binding the public key to the subject's identity and serving as the root of trust). 
For digital signature, the subject/prover generates a public-private-key pair ($K$ is the public key while $k$ is the private key) and digitally signs a message $m$ using its private key $k$ to generate the digital signature $S_k(m)$, which involves the public-key cipher algorithm using the private key $k$ on the hash of the message $m$. The verifier receives the message $m$ and the signature $S_k(m)$, which are the two inputs for the verification $V_K(m,S_k(m))$. The verification i) computes the hash of $m$ and ii) applies the public-key cipher algorithm using the public key $K$ on $S_k(m)$. If the two results in the same, then the signature is verified; if not, the verification fails. The verification $V_K(m,S_k(m))$ results in the Boolean. The key inputs for signing $S$ and verification $V$ are in subscripts while the message inputs are in parentheses because the key inputs are fixed while the messages change, i.e., key refreshes are significantly less frequent than the message changes. While any entity involved in networking can generate the public-private key pair and digitally sign, we focus on the base station as our goal is to authenticate the base station using its public key, i.e., $K$ and $k$, respectively, are the base station's public key and private key in our work. %\syc{Let's use these notations throughout the paper. There should be minor adaptations in Our Scheme section.}

% The digital signature security relies on the secrecy of private key $k$ but not on the public key $K$ (i.e., the security and the signature integrity hold even if the public key $K$ is known) and on the cipher design based on the one-way trapdoor function so that it is computationally difficult and impractical to derive $k$ from $K$. Rivest-Shamir-Adleman (RSA) or elliptic curve digital signature algorithm (ECDSA) provides the cipher algorithms for digital signature. Since ECDSA is popularly used in mobile computing due to its efficiency (i.e., smaller keys for comparable security levels), we focus on ECDSA in our scheme and implementation. Furthermore, in many secure applications (including in our scheme as well as the state-of-the-art research), the private key $k$ stays locally and does not get communicated/networked beyond the local machine, significantly reducing the vulnerability and risk of its compromise by the unauthorized entities. 

% Public-key infrastructure (PKI) involves the trusted certificate authority to generate the digital certificate binding the public key $K$ and its subject's identifier. The digital certificates ensure that $K$ belongs to the subject holding the identifier. In our scheme, we use the standardized X.509 digital certificate and the cell ID for the base station ID, described in Section~\ref{subsec:background_5G}. 


% \vspace{-2px}
% \subsection{Digital Signature and Digital Certificate Variable Notations}
% \label{subsec:background_public_key}

% Public-key cryptography provides the standard and widely used cryptographic techniques for the digital signature (providing sender authenticity and message authenticity) and public-key infrastructure or PKI (providing the digital certificate binding the public key to the subject's identity and serving as the root of trust). 
% For digital signature, the subject/prover generates a public-private-key pair ($K$ is the public key while $k$ is the private key) and digitally signs a message $m$ using its private key $k$ to generate the digital signature $S_k(m)$, which involves the public-key cipher algorithm using the private key $k$ on the hash of the message $m$. The verifier receives the message $m$ and the signature $S_k(m)$, which are the two inputs for the verification $V_K(m,S_k(m))$. The verification i) computes the hash of $m$ and ii) applies the public-key cipher algorithm using the public key $K$ on $S_k(m)$. If the two results in the same, then the signature is verified; if not, the verification fails. The verification $V_K(m,S_k(m))$ results in the Boolean. The key inputs for signing $S$ and verification $V$ are in subscripts while the message inputs are in parentheses because the key inputs are fixed while the messages change, i.e., key refreshes are significantly less frequent than the message changes. While any entity involved in networking can generate the public-private key pair and digitally sign, we focus on the base station as our goal is to authenticate the base station using its public key, i.e., $K$ and $k$, respectively, are the base station's public key and private key in our work. 


==> Sections/motivation_RRC.tex <==
\subsection{Motivation: RRC is Heavy}
\label{subsec:RRC_anlaysis}

==> Sections/related_wormhole.tex <==
\section{More Related Work: Wormhole Defense}
\label{appendix:related}

\syc{If included back in the main-body text, better highlight why we single out wormhole defense. "Our work defends against wormhole threat, while the SOTA combining multiple research literature does not."}
% % \newline
% \noindent \textbf{Wormhole Defense} \hspace{0.05in} 
% %\subsubsection{Wormhole Defense}
% %\label{subsubsec:rw_wormhole}
% % \syc{Draft this in the WSN and other contexts beyond 5G/base station}
% % % Hu et. al~\cite{hu2003packet} introduced the wormhole attack that is specific to wireless ad hoc networks (such as wireless sensor networks, IoT) and provided a packet leash-based (geographical and temporal information) defense against the attack. In a wormhole attack, the attackers can record packets (or bits) from the network at one location, tunnel the packets (or bits) to another location, and retransmit them to the network.
\sour{Although wormhole attacks can apply to any wireless network, the research community has taken different approaches in the last two decades to defend against wormhole attacks in wireless ad hoc networks such as wireless sensor networks since routing in such networks is vulnerable to wormhole attacks. The approaches can be divided into two categories based on whether spatial or temporal information of the sender is required or not. Hu et. al~\cite{hu2003packet} provide a packet-leash-based defense mechanism for wireless ad hoc networks, where the packet leash is the geographical and the temporal information of the packet that limits the distance from the sender and lifespan of the packet. On the other hand, there are research works that do not use geographical location or time synchronization information to thwart wormhole attacks. Such research prevents wormhole attacks by estimating the physical distance using distance-bounding protocol~\cite{vcapkun2003sector}, using directional antennas with an accurate set of neighbors~\cite{hu2004using}, monitoring neighbor node behavior~\cite{choi2008wap}, a cryptography-based approach~\cite{lazos2005preventing}. The recent approaches for detecting and preventing wormhole attacks at the network layer routing in mobile ad-hoc networks include machine learning-based~\cite{tahboush2021hybrid,abdan2022machine}, enhancing routing protocol~\cite{sankara2020modified}. Whereas these research works focus on decentralized ad-hoc wireless networks, to the best of our knowledge there is no defense research against wormhole attacks in the cellular networking context which is centralized. We include the wormhole attack in our threat model because of its sophistication in malicious base station attack which is discussed in Section~\ref{subsec:threat_analyses}}.


%\sou{Maybe it would be better if we could give a strong reason why we are using location for a wormhole in our context as compared to the research works mentioned above. Although, I do not have any arguable reason.}
